Actuator-Lag-Aligned Composite Learning for Adaptive Quadrotor Control Under a Rotor-Command Activity Budget

Composite-learning model reference adaptive control (MRAC) adds a prediction error to the tracking-error update. In a quadrotor cascade, the target can use commanded or realized inputs. The two are compared with every controller selected to keep its rotor-command activity in a noisy step within 1.05 times that of a linear-quadratic regulator (LQR). In a radialbasis-function (RBF) neural MRAC, the realized-input target needs only a nominal motor model and the measured attitude, not acceleration or rotor-speed sensing. Ablations and a one-axis analysis trace the benefit to delaying the commanded thrust and torques through a first-order actuator model. A linear filter with the motor time constant matches the nonlinear motor model, equal filtering of both sides of the target does not, and removing the RBF neurons changes the errors of the lag-aligned profiles by less than 1mm. With lag-aligned targets in both loops and a multi-seed guard, the mean error over six evaluation scenarios (Eval6) is 45.6mm with the linear filter and 46.4mm with the motor model; the best guarded non-neural comparator reaches 72.2mm. The advantage is conditional. If maneuver activity must also stay at LQR level, geometric control with a disturbance observer has the lowest design cost, and the activity benefit disappears at twice the modeled motor constant. In PX4 softwarein-the-loop simulation, the lag-aligned controller tracks better than LQR on every tested seed, but no tested gain keeps hover activity within the threshold on all seeds.

==> generated/results_macros.tex <==
% Numerical results generated by the analysis scripts (see the code repository). Do not edit by hand.
% Usage in the text: \val{group}{profile}{quantity}.
\makeatletter
\newcommand{\val}[3]{\csname v@#1@#2@#3\endcsname}
\expandafter\def\csname v@rR@gd@ncand\endcsname{55}
\expandafter\def\csname v@rR@gd@nchange\endcsname{0}
\expandafter\def\csname v@rR@gd@selo\endcsname{0.01}
\expandafter\def\csname v@rR@gd@sehi\endcsname{0.04}
\expandafter\def\csname v@rR@gd@passmargin\endcsname{0.05}
\expandafter\def\csname v@rR@gd@passnse\endcsname{1.8}
\expandafter\def\csname v@rR@gd@failmin\endcsname{0.04}
\expandafter\def\csname v@rR@Lonea@b20\endcsname{13.117}
\expandafter\def\csname v@rR@Lonea@b40\endcsname{13.116}
\expandafter\def\csname v@rR@Loneb@b20\endcsname{13.078}
\expandafter\def\csname v@rR@Loneb@b40\endcsname{13.078}
\expandafter\def\csname v@rR@Lonea@J\endcsname{100.8}
\expandafter\def\csname v@rR@Lonea@eval6\endcsname{111.3}
\expandafter\def\csname v@rR@Lonea@pass\endcsname{95}
\expandafter\def\csname v@rR@Lonea@incS2\endcsname{6}
\expandafter\def\csname v@rR@Lonea@incS4\endcsname{3}
\expandafter\def\csname v@rR@tm@lpfkeep\endcsname{60}
\expandafter\def\csname v@rR@tm@lpfJmax\endcsname{37.7}
\expandafter\def\csname v@rR@tm@lpfdiv\endcsname{80}
\expandafter\def\csname v@rR@tm@lpfact40\endcsname{1.33}
\expandafter\def\csname v@rR@tm@bothkeep\endcsname{80}
\expandafter\def\csname v@rR@tm@bothJmax\endcsname{39.8}
\expandafter\def\csname v@rR@tm@bothdiv\endcsname{100}
\expandafter\def\csname v@rR@tm@bothact40\endcsname{1.32}
\expandafter\def\csname v@rR@tm@attkeep\endcsname{100}
\expandafter\def\csname v@rR@tm@attJmax\endcsname{56.4}
\expandafter\def\csname v@rR@tm@attact40\endcsname{1.07}
\expandafter\def\csname v@rR@lin@gcmd\endcsname{3200}
\expandafter\def\csname v@rR@lin@glag\endcsname{51200}
\expandafter\def\csname v@rR@lin@gratio\endcsname{16}
\expandafter\def\csname v@rR@lin@elag\endcsname{2.20}
\expandafter\def\csname v@rR@lin@ecmd\endcsname{3.20}
\expandafter\def\csname v@rR@lin@esym\endcsname{2.55}
\expandafter\def\csname v@rR@sitl@hovlo\endcsname{0.80}
\expandafter\def\csname v@rR@sitl@hovhi\endcsname{1.12}
\expandafter\def\csname v@rR@sitl@cleanlo\endcsname{0.91}
\expandafter\def\csname v@rR@sitl@cleanhi\endcsname{1.12}
\expandafter\def\csname v@rR@sitl@lqrclean\endcsname{0.59}
\expandafter\def\csname v@rR@sitl@lqrto\endcsname{0.87}
\expandafter\def\csname v@rR@sitl@nto\endcsname{23}
\expandafter\def\csname v@rR@sitl@nhov\endcsname{40}
\expandafter\def\csname v@rR@sitl@med0\endcsname{1.14}
\expandafter\def\csname v@rR@sitl@rel0\endcsname{1.16}
\expandafter\def\csname v@rR@sitl@med20\endcsname{1.04}
\expandafter\def\csname v@rR@sitl@rel20\endcsname{1.05}
\expandafter\def\csname v@rR@sitl@med50\endcsname{1.07}
\expandafter\def\csname v@rR@sitl@rel50\endcsname{1.03}
\expandafter\def\csname v@rR@sitl@swins\endcsname{5}
\expandafter\def\csname v@rR@sitl@sn\endcsname{5}
\expandafter\def\csname v@rR@sitl@scl\endcsname{483}
\expandafter\def\csname v@rR@sitl@slqr\endcsname{619}
\expandafter\def\csname v@rR@sitl@snofilt\endcsname{488}
\expandafter\def\csname v@rR@sitl@smed0\endcsname{1.33}
\expandafter\def\csname v@rR@sitl@smed20\endcsname{1.54}
\expandafter\def\csname v@rR@geo@kp\endcsname{1}
\expandafter\def\csname v@rR@geo@ka\endcsname{0.5}
\expandafter\def\csname v@rR@geo@otau\endcsname{200}
\expandafter\def\csname v@rR@geo@beta\endcsname{1}
\expandafter\def\csname v@rR@geo@rtau\endcsname{400}
\expandafter\def\csname v@rR@geo@srtau\endcsname{200}
\expandafter\def\csname v@rR@base@budget\endcsname{13.0267}
\expandafter\def\csname v@rR@base@gsel\endcsname{80/80/320/1280}
\expandafter\def\csname v@rR@base@bothpass\endcsname{92}
\expandafter\def\csname v@rR@base@innerpass\endcsname{63}
\expandafter\def\csname v@rR@base@cilo\endcsname{96.38}
\expandafter\def\csname v@rB@n1@budget\endcsname{12.64}
\expandafter\def\csname v@rB@n1@attcand\endcsname{80}
\expandafter\def\csname v@rB@n1@attJ\endcsname{50.6}
\expandafter\def\csname v@rB@n1@attnpass\endcsname{3/3}
\expandafter\def\csname v@rB@n1@innercand\endcsname{160}
\expandafter\def\csname v@rB@n1@innerJ\endcsname{46.4}
\expandafter\def\csname v@rB@n1@innernpass\endcsname{3/3}
\expandafter\def\csname v@rB@n1@bothcand\endcsname{160}
\expandafter\def\csname v@rB@n1@bothJ\endcsname{46.5}
\expandafter\def\csname v@rB@n1@bothnpass\endcsname{2/3}
\expandafter\def\csname v@rB@n1@lpfcand\endcsname{160}
\expandafter\def\csname v@rB@n1@lpfJ\endcsname{46.5}
\expandafter\def\csname v@rB@n1@lpfnpass\endcsname{2/3}
\expandafter\def\csname v@rB@n1@geocand\endcsname{924}
\expandafter\def\csname v@rB@n1@geoJ\endcsname{73.0}
\expandafter\def\csname v@rB@n1@geonpass\endcsname{9/10}
\expandafter\def\csname v@rB@n1@indicand\endcsname{71}
\expandafter\def\csname v@rB@n1@indiJ\endcsname{113.7}
\expandafter\def\csname v@rB@n1@indinpass\endcsname{9/10}
\expandafter\def\csname v@rB@n1@attsone\endcsname{80}
\expandafter\def\csname v@rB@n1@attadm\endcsname{4/10}
\expandafter\def\csname v@rB@n1@innersone\endcsname{160}
\expandafter\def\csname v@rB@n1@inneradm\endcsname{5/10}
\expandafter\def\csname v@rB@n1@bothsone\endcsname{320}
\expandafter\def\csname v@rB@n1@bothadm\endcsname{6/10}
\expandafter\def\csname v@rB@n1@lpfsone\endcsname{320}
\expandafter\def\csname v@rB@n1@lpfadm\endcsname{6/10}
\expandafter\def\csname v@rB@n1@geosone\endcsname{924}
\expandafter\def\csname v@rB@n1@geoadm\endcsname{463/1074}
\expandafter\def\csname v@rB@n1@indisone\endcsname{71}
\expandafter\def\csname v@rB@n1@indiadm\endcsname{24/107}
\expandafter\def\csname v@rB@n1@atteval\endcsname{59.2}
\expandafter\def\csname v@rB@n1@attJev\endcsname{50.6}
\expandafter\def\csname v@rB@n1@attact\endcsname{1.028}
\expandafter\def\csname v@rB@n1@innereval\endcsname{54.2}
\expandafter\def\csname v@rB@n1@innerJev\endcsname{46.4}
\expandafter\def\csname v@rB@n1@inneract\endcsname{1.034}
\expandafter\def\csname v@rB@n1@botheval\endcsname{54.4}
\expandafter\def\csname v@rB@n1@bothJev\endcsname{46.5}
\expandafter\def\csname v@rB@n1@bothact\endcsname{1.025}
\expandafter\def\csname v@rB@n1@lpfeval\endcsname{54.3}
\expandafter\def\csname v@rB@n1@lpfJev\endcsname{46.5}
\expandafter\def\csname v@rB@n1@lpfact\endcsname{1.025}
\expandafter\def\csname v@rB@n1@geoeval\endcsname{158.9}
\expandafter\def\csname v@rB@n1@geoJev\endcsname{73.0}
\expandafter\def\csname v@rB@n1@geoact\endcsname{0.894}
\expandafter\def\csname v@rB@n1@indieval\endcsname{275.1}
\expandafter\def\csname v@rB@n1@indiJev\endcsname{113.7}
\expandafter\def\csname v@rB@n1@indiact\endcsname{0.943}
\expandafter\def\csname v@rB@n1@lqreval\endcsname{473.8}
\expandafter\def\csname v@rB@n1@lqrJev\endcsname{326.0}
\expandafter\def\csname v@rB@n1@lqract\endcsname{1.000}
\expandafter\def\csname v@rB@n1@compspread\endcsname{0.2}
\expandafter\def\csname v@rB@n1@actmax\endcsname{1.034}
\expandafter\def\csname v@rB@n1@actmaxfam\endcsname{CL-Inner}
\expandafter\def\csname v@rB@n2@atteval\endcsname{60.7}
\expandafter\def\csname v@rB@n2@attJev\endcsname{57.0}
\expandafter\def\csname v@rB@n2@attact\endcsname{1.041}
\expandafter\def\csname v@rB@n2@innereval\endcsname{56.3}
\expandafter\def\csname v@rB@n2@innerJev\endcsname{53.7}
\expandafter\def\csname v@rB@n2@inneract\endcsname{1.055}
\expandafter\def\csname v@rB@n2@botheval\endcsname{56.5}
\expandafter\def\csname v@rB@n2@bothJev\endcsname{53.9}
\expandafter\def\csname v@rB@n2@bothact\endcsname{1.039}
\expandafter\def\csname v@rB@n2@lpfeval\endcsname{56.4}
\expandafter\def\csname v@rB@n2@lpfJev\endcsname{53.9}
\expandafter\def\csname v@rB@n2@lpfact\endcsname{1.039}
\expandafter\def\csname v@rB@n2@geoeval\endcsname{237.8}
\expandafter\def\csname v@rB@n2@geoJev\endcsname{103.4}
\expandafter\def\csname v@rB@n2@geoact\endcsname{0.895}
\expandafter\def\csname v@rB@n2@indieval\endcsname{347.9}
\expandafter\def\csname v@rB@n2@indiJev\endcsname{151.7}
\expandafter\def\csname v@rB@n2@indiact\endcsname{0.943}
\expandafter\def\csname v@rB@n2@lqreval\endcsname{465.0}
\expandafter\def\csname v@rB@n2@lqrJev\endcsname{312.4}
\expandafter\def\csname v@rB@n2@lqract\endcsname{1.000}
\expandafter\def\csname v@rB@n2@compspread\endcsname{0.2}
\expandafter\def\csname v@rB@n2@actmax\endcsname{1.055}
\expandafter\def\csname v@rB@n2@actmaxfam\endcsname{CL-Inner}
\expandafter\def\csname v@rB@indi2@J\endcsname{70.7}
\expandafter\def\csname v@rB@indi2@eval6\endcsname{72.2}
\expandafter\def\csname v@rB@indi2@bound\endcsname{9.22}
\expandafter\def\csname v@rB@indi2@adm\endcsname{52}
\expandafter\def\csname v@rB@indi2@grid\endcsname{96}
\expandafter\def\csname v@rB@indi2@npass\endcsname{10/10}
\expandafter\def\csname v@rB@indi2@vpass\endcsname{100}
\expandafter\def\csname v@rB@indi2@vpair\endcsname{100}
\expandafter\def\csname v@rB@indi2@fc\endcsname{16}
\expandafter\def\csname v@rB@indi2@po\endcsname{2}
\expandafter\def\csname v@rB@indi2@pi\endcsname{0.5}
\expandafter\def\csname v@rB@indi2@S1\endcsname{29.2}
\expandafter\def\csname v@rB@indi2@S2\endcsname{76.9}
\expandafter\def\csname v@rB@indi2@S3\endcsname{48.1}
\expandafter\def\csname v@rB@indi2@S4\endcsname{87.2}
\expandafter\def\csname v@rB@indi2@S5\endcsname{217.2}
\expandafter\def\csname v@rB@indi2@S6\endcsname{1.4}
\expandafter\def\csname v@rB@indi2@S7\endcsname{1.8}
\expandafter\def\csname v@rB@indi2@S8\endcsname{41.0}
\expandafter\def\csname v@rB@indi2@S9\endcsname{91.5}
\expandafter\def\csname v@rB@indi2@S10\endcsname{52.7}
\expandafter\def\csname v@rB@indi2@Siiw\endcsname{50}
\expandafter\def\csname v@rB@indi2@Siin\endcsname{50}
\expandafter\def\csname v@rB@indi2@Siifail\endcsname{0}
\expandafter\def\csname v@rB@indi2@Siip95\endcsname{97.5}
\expandafter\def\csname v@rB@indi2@Siimed\endcsname{80.3}
\expandafter\def\csname v@rB@indi2@Sivw\endcsname{50}
\expandafter\def\csname v@rB@indi2@Sivn\endcsname{50}
\expandafter\def\csname v@rB@indi2@Sivfail\endcsname{0}
\expandafter\def\csname v@rB@indi2@Sivp95\endcsname{112.5}
\expandafter\def\csname v@rB@indi2@Sivmed\endcsname{90.1}
\expandafter\def\csname v@S1@LQR@RMSE\endcsname{221.6}
\expandafter\def\csname v@S1@LQR@RMSE5\endcsname{161.2}
\expandafter\def\csname v@S1@LQR@MAXE5\endcsname{161.2}
\expandafter\def\csname v@S1@LQR@IAE\endcsname{5.570}
\expandafter\def\csname v@S1@LQR@PSIE\endcsname{0.25}
\expandafter\def\csname v@S1@LQR@TV\endcsname{20}
\expandafter\def\csname v@S1@LQR@DW\endcsname{0.04}
\expandafter\def\csname v@S1@LQR@WSAT\endcsname{0.0}
\expandafter\def\csname v@S1@LQR@DHAT\endcsname{0.651}
\expandafter\def\csname v@S1@LQR@DHATP\endcsname{0.736}
\expandafter\def\csname v@S1@MRAC@RMSE\endcsname{153.2}
\expandafter\def\csname v@S1@MRAC@RMSE5\endcsname{31.3}
\expandafter\def\csname v@S1@MRAC@MAXE5\endcsname{48.1}
\expandafter\def\csname v@S1@MRAC@IAE\endcsname{1.860}
\expandafter\def\csname v@S1@MRAC@PSIE\endcsname{0.36}
\expandafter\def\csname v@S1@MRAC@TV\endcsname{34}
\expandafter\def\csname v@S1@MRAC@DW\endcsname{0.04}
\expandafter\def\csname v@S1@MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S1@MRAC@DHAT\endcsname{0.129}
\expandafter\def\csname v@S1@MRAC@DHATP\endcsname{0.273}
\expandafter\def\csname v@S1@B1@RMSE\endcsname{149.2}
\expandafter\def\csname v@S1@B1@RMSE5\endcsname{36.2}
\expandafter\def\csname v@S1@B1@MAXE5\endcsname{58.5}
\expandafter\def\csname v@S1@B1@IAE\endcsname{1.885}
\expandafter\def\csname v@S1@B1@PSIE\endcsname{0.59}
\expandafter\def\csname v@S1@B1@TV\endcsname{151}
\expandafter\def\csname v@S1@B1@DW\endcsname{0.28}
\expandafter\def\csname v@S1@B1@WSAT\endcsname{0.0}
\expandafter\def\csname v@S1@B1@DHAT\endcsname{0.379}
\expandafter\def\csname v@S1@B1@DHATP\endcsname{0.377}
\expandafter\def\csname v@S1@NN-MRAC@RMSE\endcsname{155.0}
\expandafter\def\csname v@S1@NN-MRAC@RMSE5\endcsname{37.0}
\expandafter\def\csname v@S1@NN-MRAC@MAXE5\endcsname{56.1}
\expandafter\def\csname v@S1@NN-MRAC@IAE\endcsname{2.010}
\expandafter\def\csname v@S1@NN-MRAC@PSIE\endcsname{0.31}
\expandafter\def\csname v@S1@NN-MRAC@TV\endcsname{26}
\expandafter\def\csname v@S1@NN-MRAC@DW\endcsname{0.04}
\expandafter\def\csname v@S1@NN-MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S1@NN-MRAC@DHAT\endcsname{0.147}
\expandafter\def\csname v@S1@NN-MRAC@DHATP\endcsname{0.272}
\expandafter\def\csname v@S1@CL-ucmd@RMSE\endcsname{153.3}
\expandafter\def\csname v@S1@CL-ucmd@RMSE5\endcsname{21.8}
\expandafter\def\csname v@S1@CL-ucmd@MAXE5\endcsname{71.1}
\expandafter\def\csname v@S1@CL-ucmd@IAE\endcsname{1.481}
\expandafter\def\csname v@S1@CL-ucmd@PSIE\endcsname{0.34}
\expandafter\def\csname v@S1@CL-ucmd@TV\endcsname{27}
\expandafter\def\csname v@S1@CL-ucmd@DW\endcsname{0.04}
\expandafter\def\csname v@S1@CL-ucmd@WSAT\endcsname{0.0}
\expandafter\def\csname v@S1@CL-ucmd@DHAT\endcsname{0.074}
\expandafter\def\csname v@S1@CL-ucmd@DHATP\endcsname{0.205}
\expandafter\def\csname v@S1@CL-att@RMSE\endcsname{148.4}
\expandafter\def\csname v@S1@CL-att@RMSE5\endcsname{25.4}
\expandafter\def\csname v@S1@CL-att@MAXE5\endcsname{26.6}
\expandafter\def\csname v@S1@CL-att@IAE\endcsname{1.603}
\expandafter\def\csname v@S1@CL-att@PSIE\endcsname{0.31}
\expandafter\def\csname v@S1@CL-att@TV\endcsname{31}
\expandafter\def\csname v@S1@CL-att@DW\endcsname{0.06}
\expandafter\def\csname v@S1@CL-att@WSAT\endcsname{0.0}
\expandafter\def\csname v@S1@CL-att@DHAT\endcsname{0.105}
\expandafter\def\csname v@S1@CL-att@DHATP\endcsname{0.059}
\expandafter\def\csname v@S1@PROPOSED@RMSE\endcsname{145.4}
\expandafter\def\csname v@S1@PROPOSED@RMSE5\endcsname{21.4}
\expandafter\def\csname v@S1@PROPOSED@MAXE5\endcsname{22.3}
\expandafter\def\csname v@S1@PROPOSED@IAE\endcsname{1.469}
\expandafter\def\csname v@S1@PROPOSED@PSIE\endcsname{0.36}
\expandafter\def\csname v@S1@PROPOSED@TV\endcsname{85}
\expandafter\def\csname v@S1@PROPOSED@DW\endcsname{0.16}
\expandafter\def\csname v@S1@PROPOSED@WSAT\endcsname{0.0}
\expandafter\def\csname v@S1@PROPOSED@DHAT\endcsname{0.088}
\expandafter\def\csname v@S1@PROPOSED@DHATP\endcsname{0.076}
\expandafter\def\csname v@S1@LQR@IMP\endcsname{87}
\expandafter\def\csname v@S1@MRAC@IMP\endcsname{31}
\expandafter\def\csname v@S1@B1@IMP\endcsname{41}
\expandafter\def\csname v@S1@NN-MRAC@IMP\endcsname{42}
\expandafter\def\csname v@S1@CL-ucmd@IMP\endcsname{1}
\expandafter\def\csname v@S1@CL-att@IMP\endcsname{16}
\expandafter\def\csname v@S2@LQR@RMSE\endcsname{231.3}
\expandafter\def\csname v@S2@LQR@RMSE5\endcsname{230.9}
\expandafter\def\csname v@S2@LQR@MAXE5\endcsname{267.3}
\expandafter\def\csname v@S2@LQR@IAE\endcsname{13.284}
\expandafter\def\csname v@S2@LQR@PSIE\endcsname{0.83}
\expandafter\def\csname v@S2@LQR@TV\endcsname{168}
\expandafter\def\csname v@S2@LQR@DW\endcsname{1.10}
\expandafter\def\csname v@S2@LQR@WSAT\endcsname{0.0}
\expandafter\def\csname v@S2@LQR@DHAT\endcsname{1.062}
\expandafter\def\csname v@S2@LQR@DHATP\endcsname{1.030}
\expandafter\def\csname v@S2@MRAC@RMSE\endcsname{74.0}
\expandafter\def\csname v@S2@MRAC@RMSE5\endcsname{76.6}
\expandafter\def\csname v@S2@MRAC@MAXE5\endcsname{235.5}
\expandafter\def\csname v@S2@MRAC@IAE\endcsname{3.533}
\expandafter\def\csname v@S2@MRAC@PSIE\endcsname{1.41}
\expandafter\def\csname v@S2@MRAC@TV\endcsname{800}
\expandafter\def\csname v@S2@MRAC@DW\endcsname{2.97}
\expandafter\def\csname v@S2@MRAC@WSAT\endcsname{0.1}
\expandafter\def\csname v@S2@MRAC@DHAT\endcsname{1.672}
\expandafter\def\csname v@S2@MRAC@DHATP\endcsname{1.662}
\expandafter\def\csname v@S2@B1@RMSE\endcsname{87.5}
\expandafter\def\csname v@S2@B1@RMSE5\endcsname{85.6}
\expandafter\def\csname v@S2@B1@MAXE5\endcsname{309.9}
\expandafter\def\csname v@S2@B1@IAE\endcsname{4.366}
\expandafter\def\csname v@S2@B1@PSIE\endcsname{1.39}
\expandafter\def\csname v@S2@B1@TV\endcsname{1195}
\expandafter\def\csname v@S2@B1@DW\endcsname{2.31}
\expandafter\def\csname v@S2@B1@WSAT\endcsname{0.0}
\expandafter\def\csname v@S2@B1@DHAT\endcsname{1.922}
\expandafter\def\csname v@S2@B1@DHATP\endcsname{1.583}
\expandafter\def\csname v@S2@NN-MRAC@RMSE\endcsname{54.6}
\expandafter\def\csname v@S2@NN-MRAC@RMSE5\endcsname{55.5}
\expandafter\def\csname v@S2@NN-MRAC@MAXE5\endcsname{122.2}
\expandafter\def\csname v@S2@NN-MRAC@IAE\endcsname{2.613}
\expandafter\def\csname v@S2@NN-MRAC@PSIE\endcsname{0.94}
\expandafter\def\csname v@S2@NN-MRAC@TV\endcsname{290}
\expandafter\def\csname v@S2@NN-MRAC@DW\endcsname{1.45}
\expandafter\def\csname v@S2@NN-MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S2@NN-MRAC@DHAT\endcsname{0.869}
\expandafter\def\csname v@S2@NN-MRAC@DHATP\endcsname{0.675}
\expandafter\def\csname v@S2@CL-ucmd@RMSE\endcsname{72.7}
\expandafter\def\csname v@S2@CL-ucmd@RMSE5\endcsname{74.0}
\expandafter\def\csname v@S2@CL-ucmd@MAXE5\endcsname{122.2}
\expandafter\def\csname v@S2@CL-ucmd@IAE\endcsname{3.994}
\expandafter\def\csname v@S2@CL-ucmd@PSIE\endcsname{0.85}
\expandafter\def\csname v@S2@CL-ucmd@TV\endcsname{296}
\expandafter\def\csname v@S2@CL-ucmd@DW\endcsname{1.66}
\expandafter\def\csname v@S2@CL-ucmd@WSAT\endcsname{0.0}
\expandafter\def\csname v@S2@CL-ucmd@DHAT\endcsname{0.878}
\expandafter\def\csname v@S2@CL-ucmd@DHATP\endcsname{0.725}
\expandafter\def\csname v@S2@CL-att@RMSE\endcsname{40.1}
\expandafter\def\csname v@S2@CL-att@RMSE5\endcsname{41.5}
\expandafter\def\csname v@S2@CL-att@MAXE5\endcsname{113.2}
\expandafter\def\csname v@S2@CL-att@IAE\endcsname{1.609}
\expandafter\def\csname v@S2@CL-att@PSIE\endcsname{0.95}
\expandafter\def\csname v@S2@CL-att@TV\endcsname{201}
\expandafter\def\csname v@S2@CL-att@DW\endcsname{1.13}
\expandafter\def\csname v@S2@CL-att@WSAT\endcsname{0.0}
\expandafter\def\csname v@S2@CL-att@DHAT\endcsname{0.665}
\expandafter\def\csname v@S2@CL-att@DHATP\endcsname{0.312}
\expandafter\def\csname v@S2@PROPOSED@RMSE\endcsname{26.4}
\expandafter\def\csname v@S2@PROPOSED@RMSE5\endcsname{27.5}
\expandafter\def\csname v@S2@PROPOSED@MAXE5\endcsname{74.3}
\expandafter\def\csname v@S2@PROPOSED@IAE\endcsname{1.117}
\expandafter\def\csname v@S2@PROPOSED@PSIE\endcsname{1.01}
\expandafter\def\csname v@S2@PROPOSED@TV\endcsname{350}
\expandafter\def\csname v@S2@PROPOSED@DW\endcsname{1.01}
\expandafter\def\csname v@S2@PROPOSED@WSAT\endcsname{0.0}
\expandafter\def\csname v@S2@PROPOSED@DHAT\endcsname{0.820}
\expandafter\def\csname v@S2@PROPOSED@DHATP\endcsname{0.604}
\expandafter\def\csname v@S2@LQR@IMP\endcsname{88}
\expandafter\def\csname v@S2@MRAC@IMP\endcsname{64}
\expandafter\def\csname v@S2@B1@IMP\endcsname{68}
\expandafter\def\csname v@S2@NN-MRAC@IMP\endcsname{50}
\expandafter\def\csname v@S2@CL-ucmd@IMP\endcsname{63}
\expandafter\def\csname v@S2@CL-att@IMP\endcsname{34}
\expandafter\def\csname v@S3@LQR@RMSE\endcsname{446.1}
\expandafter\def\csname v@S3@LQR@RMSE5\endcsname{450.2}
\expandafter\def\csname v@S3@LQR@MAXE5\endcsname{628.8}
\expandafter\def\csname v@S3@LQR@IAE\endcsname{12.608}
\expandafter\def\csname v@S3@LQR@PSIE\endcsname{0.37}
\expandafter\def\csname v@S3@LQR@TV\endcsname{37}
\expandafter\def\csname v@S3@LQR@DW\endcsname{0.04}
\expandafter\def\csname v@S3@LQR@WSAT\endcsname{0.0}
\expandafter\def\csname v@S3@LQR@DHAT\endcsname{1.865}
\expandafter\def\csname v@S3@LQR@DHATP\endcsname{1.936}
\expandafter\def\csname v@S3@MRAC@RMSE\endcsname{175.6}
\expandafter\def\csname v@S3@MRAC@RMSE5\endcsname{88.8}
\expandafter\def\csname v@S3@MRAC@MAXE5\endcsname{117.4}
\expandafter\def\csname v@S3@MRAC@IAE\endcsname{3.460}
\expandafter\def\csname v@S3@MRAC@PSIE\endcsname{0.79}
\expandafter\def\csname v@S3@MRAC@TV\endcsname{255}
\expandafter\def\csname v@S3@MRAC@DW\endcsname{0.15}
\expandafter\def\csname v@S3@MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S3@MRAC@DHAT\endcsname{0.606}
\expandafter\def\csname v@S3@MRAC@DHATP\endcsname{0.603}
\expandafter\def\csname v@S3@B1@RMSE\endcsname{21910.1}
\expandafter\def\csname v@S3@B1@RMSE5\endcsname{36818.0}
\expandafter\def\csname v@S3@B1@MAXE5\endcsname{49897.9}
\expandafter\def\csname v@S3@B1@IAE\endcsname{112.450}
\expandafter\def\csname v@S3@B1@PSIE\endcsname{72.05}
\expandafter\def\csname v@S3@B1@TV\endcsname{4475}
\expandafter\def\csname v@S3@B1@DW\endcsname{6.38}
\expandafter\def\csname v@S3@B1@WSAT\endcsname{65.1}
\expandafter\def\csname v@S3@B1@DHAT\endcsname{200.096}
\expandafter\def\csname v@S3@B1@DHATP\endcsname{237.435}
\expandafter\def\csname v@S3@NN-MRAC@RMSE\endcsname{187.1}
\expandafter\def\csname v@S3@NN-MRAC@RMSE5\endcsname{113.6}
\expandafter\def\csname v@S3@NN-MRAC@MAXE5\endcsname{129.9}
\expandafter\def\csname v@S3@NN-MRAC@IAE\endcsname{4.066}
\expandafter\def\csname v@S3@NN-MRAC@PSIE\endcsname{0.63}
\expandafter\def\csname v@S3@NN-MRAC@TV\endcsname{129}
\expandafter\def\csname v@S3@NN-MRAC@DW\endcsname{0.09}
\expandafter\def\csname v@S3@NN-MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S3@NN-MRAC@DHAT\endcsname{0.499}
\expandafter\def\csname v@S3@NN-MRAC@DHATP\endcsname{0.547}
\expandafter\def\csname v@S3@CL-ucmd@RMSE\endcsname{166.3}
\expandafter\def\csname v@S3@CL-ucmd@RMSE5\endcsname{63.3}
\expandafter\def\csname v@S3@CL-ucmd@MAXE5\endcsname{119.2}
\expandafter\def\csname v@S3@CL-ucmd@IAE\endcsname{2.841}
\expandafter\def\csname v@S3@CL-ucmd@PSIE\endcsname{0.62}
\expandafter\def\csname v@S3@CL-ucmd@TV\endcsname{78}
\expandafter\def\csname v@S3@CL-ucmd@DW\endcsname{0.07}
\expandafter\def\csname v@S3@CL-ucmd@WSAT\endcsname{0.0}
\expandafter\def\csname v@S3@CL-ucmd@DHAT\endcsname{0.250}
\expandafter\def\csname v@S3@CL-ucmd@DHATP\endcsname{0.383}
\expandafter\def\csname v@S3@CL-att@RMSE\endcsname{154.1}
\expandafter\def\csname v@S3@CL-att@RMSE5\endcsname{46.1}
\expandafter\def\csname v@S3@CL-att@MAXE5\endcsname{59.8}
\expandafter\def\csname v@S3@CL-att@IAE\endcsname{2.150}
\expandafter\def\csname v@S3@CL-att@PSIE\endcsname{0.59}
\expandafter\def\csname v@S3@CL-att@TV\endcsname{75}
\expandafter\def\csname v@S3@CL-att@DW\endcsname{0.11}
\expandafter\def\csname v@S3@CL-att@WSAT\endcsname{0.0}
\expandafter\def\csname v@S3@CL-att@DHAT\endcsname{0.193}
\expandafter\def\csname v@S3@CL-att@DHATP\endcsname{0.097}
\expandafter\def\csname v@S3@PROPOSED@RMSE\endcsname{151.0}
\expandafter\def\csname v@S3@PROPOSED@RMSE5\endcsname{35.8}
\expandafter\def\csname v@S3@PROPOSED@MAXE5\endcsname{46.8}
\expandafter\def\csname v@S3@PROPOSED@IAE\endcsname{1.876}
\expandafter\def\csname v@S3@PROPOSED@PSIE\endcsname{0.61}
\expandafter\def\csname v@S3@PROPOSED@TV\endcsname{246}
\expandafter\def\csname v@S3@PROPOSED@DW\endcsname{0.38}
\expandafter\def\csname v@S3@PROPOSED@WSAT\endcsname{0.0}
\expandafter\def\csname v@S3@PROPOSED@DHAT\endcsname{0.150}
\expandafter\def\csname v@S3@PROPOSED@DHATP\endcsname{0.114}
\expandafter\def\csname v@S3@LQR@IMP\endcsname{92}
\expandafter\def\csname v@S3@MRAC@IMP\endcsname{60}
\expandafter\def\csname v@S3@B1@IMP\endcsname{100}
\expandafter\def\csname v@S3@NN-MRAC@IMP\endcsname{69}
\expandafter\def\csname v@S3@CL-ucmd@IMP\endcsname{43}
\expandafter\def\csname v@S3@CL-att@IMP\endcsname{22}
\expandafter\def\csname v@S4@LQR@RMSE\endcsname{332.3}
\expandafter\def\csname v@S4@LQR@RMSE5\endcsname{339.0}
\expandafter\def\csname v@S4@LQR@MAXE5\endcsname{620.9}
\expandafter\def\csname v@S4@LQR@IAE\endcsname{16.458}
\expandafter\def\csname v@S4@LQR@PSIE\endcsname{1.10}
\expandafter\def\csname v@S4@LQR@TV\endcsname{255}
\expandafter\def\csname v@S4@LQR@DW\endcsname{1.40}
\expandafter\def\csname v@S4@LQR@WSAT\endcsname{0.0}
\expandafter\def\csname v@S4@LQR@DHAT\endcsname{1.567}
\expandafter\def\csname v@S4@LQR@DHATP\endcsname{1.503}
\expandafter\def\csname v@S4@MRAC@RMSE\endcsname{92.1}
\expandafter\def\csname v@S4@MRAC@RMSE5\endcsname{93.9}
\expandafter\def\csname v@S4@MRAC@MAXE5\endcsname{270.6}
\expandafter\def\csname v@S4@MRAC@IAE\endcsname{4.613}
\expandafter\def\csname v@S4@MRAC@PSIE\endcsname{2.14}
\expandafter\def\csname v@S4@MRAC@TV\endcsname{1259}
\expandafter\def\csname v@S4@MRAC@DW\endcsname{4.08}
\expandafter\def\csname v@S4@MRAC@WSAT\endcsname{0.4}
\expandafter\def\csname v@S4@MRAC@DHAT\endcsname{1.934}
\expandafter\def\csname v@S4@MRAC@DHATP\endcsname{2.111}
\expandafter\def\csname v@S4@B1@RMSE\endcsname{135.4}
\expandafter\def\csname v@S4@B1@RMSE5\endcsname{136.4}
\expandafter\def\csname v@S4@B1@MAXE5\endcsname{591.8}
\expandafter\def\csname v@S4@B1@IAE\endcsname{5.946}
\expandafter\def\csname v@S4@B1@PSIE\endcsname{2.07}
\expandafter\def\csname v@S4@B1@TV\endcsname{1591}
\expandafter\def\csname v@S4@B1@DW\endcsname{4.16}
\expandafter\def\csname v@S4@B1@WSAT\endcsname{0.2}
\expandafter\def\csname v@S4@B1@DHAT\endcsname{1.832}
\expandafter\def\csname v@S4@B1@DHATP\endcsname{1.564}
\expandafter\def\csname v@S4@NN-MRAC@RMSE\endcsname{77.9}
\expandafter\def\csname v@S4@NN-MRAC@RMSE5\endcsname{78.6}
\expandafter\def\csname v@S4@NN-MRAC@MAXE5\endcsname{193.3}
\expandafter\def\csname v@S4@NN-MRAC@IAE\endcsname{4.145}
\expandafter\def\csname v@S4@NN-MRAC@PSIE\endcsname{1.36}
\expandafter\def\csname v@S4@NN-MRAC@TV\endcsname{436}
\expandafter\def\csname v@S4@NN-MRAC@DW\endcsname{2.21}
\expandafter\def\csname v@S4@NN-MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S4@NN-MRAC@DHAT\endcsname{0.996}
\expandafter\def\csname v@S4@NN-MRAC@DHATP\endcsname{0.763}
\expandafter\def\csname v@S4@CL-ucmd@RMSE\endcsname{94.8}
\expandafter\def\csname v@S4@CL-ucmd@RMSE5\endcsname{96.1}
\expandafter\def\csname v@S4@CL-ucmd@MAXE5\endcsname{217.9}
\expandafter\def\csname v@S4@CL-ucmd@IAE\endcsname{5.206}
\expandafter\def\csname v@S4@CL-ucmd@PSIE\endcsname{1.18}
\expandafter\def\csname v@S4@CL-ucmd@TV\endcsname{461}
\expandafter\def\csname v@S4@CL-ucmd@DW\endcsname{2.51}
\expandafter\def\csname v@S4@CL-ucmd@WSAT\endcsname{0.0}
\expandafter\def\csname v@S4@CL-ucmd@DHAT\endcsname{0.947}
\expandafter\def\csname v@S4@CL-ucmd@DHATP\endcsname{0.788}
\expandafter\def\csname v@S4@CL-att@RMSE\endcsname{50.8}
\expandafter\def\csname v@S4@CL-att@RMSE5\endcsname{50.9}
\expandafter\def\csname v@S4@CL-att@MAXE5\endcsname{110.1}
\expandafter\def\csname v@S4@CL-att@IAE\endcsname{2.806}
\expandafter\def\csname v@S4@CL-att@PSIE\endcsname{1.24}
\expandafter\def\csname v@S4@CL-att@TV\endcsname{451}
\expandafter\def\csname v@S4@CL-att@DW\endcsname{2.53}
\expandafter\def\csname v@S4@CL-att@WSAT\endcsname{0.0}
\expandafter\def\csname v@S4@CL-att@DHAT\endcsname{0.679}
\expandafter\def\csname v@S4@CL-att@DHATP\endcsname{0.416}
\expandafter\def\csname v@S4@PROPOSED@RMSE\endcsname{43.0}
\expandafter\def\csname v@S4@PROPOSED@RMSE5\endcsname{44.0}
\expandafter\def\csname v@S4@PROPOSED@MAXE5\endcsname{100.7}
\expandafter\def\csname v@S4@PROPOSED@IAE\endcsname{2.295}
\expandafter\def\csname v@S4@PROPOSED@PSIE\endcsname{1.47}
\expandafter\def\csname v@S4@PROPOSED@TV\endcsname{838}
\expandafter\def\csname v@S4@PROPOSED@DW\endcsname{3.40}
\expandafter\def\csname v@S4@PROPOSED@WSAT\endcsname{0.2}
\expandafter\def\csname v@S4@PROPOSED@DHAT\endcsname{0.925}
\expandafter\def\csname v@S4@PROPOSED@DHATP\endcsname{0.852}
\expandafter\def\csname v@S4@LQR@IMP\endcsname{87}
\expandafter\def\csname v@S4@MRAC@IMP\endcsname{53}
\expandafter\def\csname v@S4@B1@IMP\endcsname{68}
\expandafter\def\csname v@S4@NN-MRAC@IMP\endcsname{44}
\expandafter\def\csname v@S4@CL-ucmd@IMP\endcsname{54}
\expandafter\def\csname v@S4@CL-att@IMP\endcsname{14}
\expandafter\def\csname v@S5@LQR@RMSE\endcsname{1099.7}
\expandafter\def\csname v@S5@LQR@RMSE5\endcsname{1126.5}
\expandafter\def\csname v@S5@LQR@MAXE5\endcsname{1907.0}
\expandafter\def\csname v@S5@LQR@IAE\endcsname{62.351}
\expandafter\def\csname v@S5@LQR@PSIE\endcsname{2.15}
\expandafter\def\csname v@S5@LQR@TV\endcsname{36294}
\expandafter\def\csname v@S5@LQR@DW\endcsname{11.51}
\expandafter\def\csname v@S5@LQR@WSAT\endcsname{0.0}
\expandafter\def\csname v@S5@LQR@DHAT\endcsname{4.637}
\expandafter\def\csname v@S5@LQR@DHATP\endcsname{4.644}
\expandafter\def\csname v@S5@MRAC@RMSE\endcsname{139.9}
\expandafter\def\csname v@S5@MRAC@RMSE5\endcsname{138.4}
\expandafter\def\csname v@S5@MRAC@MAXE5\endcsname{439.5}
\expandafter\def\csname v@S5@MRAC@IAE\endcsname{7.462}
\expandafter\def\csname v@S5@MRAC@PSIE\endcsname{3.56}
\expandafter\def\csname v@S5@MRAC@TV\endcsname{72263}
\expandafter\def\csname v@S5@MRAC@DW\endcsname{26.62}
\expandafter\def\csname v@S5@MRAC@WSAT\endcsname{2.7}
\expandafter\def\csname v@S5@MRAC@DHAT\endcsname{1.795}
\expandafter\def\csname v@S5@MRAC@DHATP\endcsname{2.362}
\expandafter\def\csname v@S5@B1@RMSE\endcsname{24604.5}
\expandafter\def\csname v@S5@B1@RMSE5\endcsname{31541.3}
\expandafter\def\csname v@S5@B1@MAXE5\endcsname{49955.5}
\expandafter\def\csname v@S5@B1@IAE\endcsname{231.219}
\expandafter\def\csname v@S5@B1@PSIE\endcsname{80.03}
\expandafter\def\csname v@S5@B1@TV\endcsname{22884}
\expandafter\def\csname v@S5@B1@DW\endcsname{23.21}
\expandafter\def\csname v@S5@B1@WSAT\endcsname{68.6}
\expandafter\def\csname v@S5@B1@DHAT\endcsname{193.720}
\expandafter\def\csname v@S5@B1@DHATP\endcsname{384.309}
\expandafter\def\csname v@S5@NN-MRAC@RMSE\endcsname{153.2}
\expandafter\def\csname v@S5@NN-MRAC@RMSE5\endcsname{153.8}
\expandafter\def\csname v@S5@NN-MRAC@MAXE5\endcsname{446.0}
\expandafter\def\csname v@S5@NN-MRAC@IAE\endcsname{7.683}
\expandafter\def\csname v@S5@NN-MRAC@PSIE\endcsname{3.39}
\expandafter\def\csname v@S5@NN-MRAC@TV\endcsname{45459}
\expandafter\def\csname v@S5@NN-MRAC@DW\endcsname{15.41}
\expandafter\def\csname v@S5@NN-MRAC@WSAT\endcsname{0.6}
\expandafter\def\csname v@S5@NN-MRAC@DHAT\endcsname{1.270}
\expandafter\def\csname v@S5@NN-MRAC@DHATP\endcsname{1.327}
\expandafter\def\csname v@S5@CL-ucmd@RMSE\endcsname{133.7}
\expandafter\def\csname v@S5@CL-ucmd@RMSE5\endcsname{132.7}
\expandafter\def\csname v@S5@CL-ucmd@MAXE5\endcsname{452.8}
\expandafter\def\csname v@S5@CL-ucmd@IAE\endcsname{7.184}
\expandafter\def\csname v@S5@CL-ucmd@PSIE\endcsname{2.91}
\expandafter\def\csname v@S5@CL-ucmd@TV\endcsname{65080}
\expandafter\def\csname v@S5@CL-ucmd@DW\endcsname{22.15}
\expandafter\def\csname v@S5@CL-ucmd@WSAT\endcsname{1.0}
\expandafter\def\csname v@S5@CL-ucmd@DHAT\endcsname{0.832}
\expandafter\def\csname v@S5@CL-ucmd@DHATP\endcsname{0.985}
\expandafter\def\csname v@S5@CL-att@RMSE\endcsname{137.4}
\expandafter\def\csname v@S5@CL-att@RMSE5\endcsname{142.2}
\expandafter\def\csname v@S5@CL-att@MAXE5\endcsname{736.0}
\expandafter\def\csname v@S5@CL-att@IAE\endcsname{5.521}
\expandafter\def\csname v@S5@CL-att@PSIE\endcsname{3.16}
\expandafter\def\csname v@S5@CL-att@TV\endcsname{62118}
\expandafter\def\csname v@S5@CL-att@DW\endcsname{20.47}
\expandafter\def\csname v@S5@CL-att@WSAT\endcsname{0.4}
\expandafter\def\csname v@S5@CL-att@DHAT\endcsname{0.746}
\expandafter\def\csname v@S5@CL-att@DHATP\endcsname{0.522}
\expandafter\def\csname v@S5@PROPOSED@RMSE\endcsname{109.2}
\expandafter\def\csname v@S5@PROPOSED@RMSE5\endcsname{113.6}
\expandafter\def\csname v@S5@PROPOSED@MAXE5\endcsname{686.7}
\expandafter\def\csname v@S5@PROPOSED@IAE\endcsname{3.936}
\expandafter\def\csname v@S5@PROPOSED@PSIE\endcsname{3.18}
\expandafter\def\csname v@S5@PROPOSED@TV\endcsname{68993}
\expandafter\def\csname v@S5@PROPOSED@DW\endcsname{22.92}
\expandafter\def\csname v@S5@PROPOSED@WSAT\endcsname{0.7}
\expandafter\def\csname v@S5@PROPOSED@DHAT\endcsname{0.820}
\expandafter\def\csname v@S5@PROPOSED@DHATP\endcsname{0.874}
\expandafter\def\csname v@S5@LQR@IMP\endcsname{90}
\expandafter\def\csname v@S5@MRAC@IMP\endcsname{18}
\expandafter\def\csname v@S5@B1@IMP\endcsname{100}
\expandafter\def\csname v@S5@NN-MRAC@IMP\endcsname{26}
\expandafter\def\csname v@S5@CL-ucmd@IMP\endcsname{14}
\expandafter\def\csname v@S5@CL-att@IMP\endcsname{20}
\expandafter\def\csname v@S6@LQR@RMSE\endcsname{433.4}
\expandafter\def\csname v@S6@LQR@RMSE5\endcsname{0.0}
\expandafter\def\csname v@S6@LQR@MAXE5\endcsname{0.1}
\expandafter\def\csname v@S6@LQR@IAE\endcsname{1.534}
\expandafter\def\csname v@S6@LQR@PSIE\endcsname{0.67}
\expandafter\def\csname v@S6@LQR@TV\endcsname{88}
\expandafter\def\csname v@S6@LQR@DW\endcsname{0.11}
\expandafter\def\csname v@S6@LQR@WSAT\endcsname{0.0}
\expandafter\def\csname v@S6@LQR@DHAT\endcsname{0.000}
\expandafter\def\csname v@S6@LQR@DHATP\endcsname{0.000}
\expandafter\def\csname v@S6@LQR@Trx\endcsname{1.08}
\expandafter\def\csname v@S6@LQR@Tsx\endcsname{1.96}
\expandafter\def\csname v@S6@LQR@OSx\endcsname{0.05}
\expandafter\def\csname v@S6@LQR@SSEx\endcsname{0.00}
\expandafter\def\csname v@S6@LQR@Trz\endcsname{1.35}
\expandafter\def\csname v@S6@LQR@Tsz\endcsname{2.13}
\expandafter\def\csname v@S6@LQR@OSz\endcsname{0.55}
\expandafter\def\csname v@S6@LQR@SSEz\endcsname{0.00}
\expandafter\def\csname v@S6@MRAC@RMSE\endcsname{418.2}
\expandafter\def\csname v@S6@MRAC@RMSE5\endcsname{5.5}
\expandafter\def\csname v@S6@MRAC@MAXE5\endcsname{10.0}
\expandafter\def\csname v@S6@MRAC@IAE\endcsname{1.577}
\expandafter\def\csname v@S6@MRAC@PSIE\endcsname{1.17}
\expandafter\def\csname v@S6@MRAC@TV\endcsname{159}
\expandafter\def\csname v@S6@MRAC@DW\endcsname{0.12}
\expandafter\def\csname v@S6@MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S6@MRAC@DHAT\endcsname{0.020}
\expandafter\def\csname v@S6@MRAC@DHATP\endcsname{0.019}
\expandafter\def\csname v@S6@MRAC@Trx\endcsname{1.23}
\expandafter\def\csname v@S6@MRAC@Tsx\endcsname{3.76}
\expandafter\def\csname v@S6@MRAC@OSx\endcsname{6.84}
\expandafter\def\csname v@S6@MRAC@SSEx\endcsname{1.35}
\expandafter\def\csname v@S6@MRAC@Trz\endcsname{1.14}
\expandafter\def\csname v@S6@MRAC@Tsz\endcsname{3.26}
\expandafter\def\csname v@S6@MRAC@OSz\endcsname{6.31}
\expandafter\def\csname v@S6@MRAC@SSEz\endcsname{0.66}
\expandafter\def\csname v@S6@B1@RMSE\endcsname{411.2}
\expandafter\def\csname v@S6@B1@RMSE5\endcsname{15.2}
\expandafter\def\csname v@S6@B1@MAXE5\endcsname{32.2}
\expandafter\def\csname v@S6@B1@IAE\endcsname{1.550}
\expandafter\def\csname v@S6@B1@PSIE\endcsname{1.22}
\expandafter\def\csname v@S6@B1@TV\endcsname{555}
\expandafter\def\csname v@S6@B1@DW\endcsname{0.66}
\expandafter\def\csname v@S6@B1@WSAT\endcsname{0.0}
\expandafter\def\csname v@S6@B1@DHAT\endcsname{0.520}
\expandafter\def\csname v@S6@B1@DHATP\endcsname{0.375}
\expandafter\def\csname v@S6@B1@Trx\endcsname{1.02}
\expandafter\def\csname v@S6@B1@Tsx\endcsname{7.05}
\expandafter\def\csname v@S6@B1@OSx\endcsname{7.37}
\expandafter\def\csname v@S6@B1@SSEx\endcsname{3.83}
\expandafter\def\csname v@S6@B1@Trz\endcsname{1.32}
\expandafter\def\csname v@S6@B1@Tsz\endcsname{1.81}
\expandafter\def\csname v@S6@B1@OSz\endcsname{1.58}
\expandafter\def\csname v@S6@B1@SSEz\endcsname{1.93}
\expandafter\def\csname v@S6@NN-MRAC@RMSE\endcsname{421.1}
\expandafter\def\csname v@S6@NN-MRAC@RMSE5\endcsname{1.7}
\expandafter\def\csname v@S6@NN-MRAC@MAXE5\endcsname{5.2}
\expandafter\def\csname v@S6@NN-MRAC@IAE\endcsname{1.587}
\expandafter\def\csname v@S6@NN-MRAC@PSIE\endcsname{1.00}
\expandafter\def\csname v@S6@NN-MRAC@TV\endcsname{124}
\expandafter\def\csname v@S6@NN-MRAC@DW\endcsname{0.12}
\expandafter\def\csname v@S6@NN-MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S6@NN-MRAC@DHAT\endcsname{0.003}
\expandafter\def\csname v@S6@NN-MRAC@DHATP\endcsname{0.004}
\expandafter\def\csname v@S6@NN-MRAC@Trx\endcsname{1.03}
\expandafter\def\csname v@S6@NN-MRAC@Tsx\endcsname{4.02}
\expandafter\def\csname v@S6@NN-MRAC@OSx\endcsname{5.54}
\expandafter\def\csname v@S6@NN-MRAC@SSEx\endcsname{0.01}
\expandafter\def\csname v@S6@NN-MRAC@Trz\endcsname{1.16}
\expandafter\def\csname v@S6@NN-MRAC@Tsz\endcsname{3.74}
\expandafter\def\csname v@S6@NN-MRAC@OSz\endcsname{7.05}
\expandafter\def\csname v@S6@NN-MRAC@SSEz\endcsname{0.03}
\expandafter\def\csname v@S6@CL-ucmd@RMSE\endcsname{421.3}
\expandafter\def\csname v@S6@CL-ucmd@RMSE5\endcsname{25.5}
\expandafter\def\csname v@S6@CL-ucmd@MAXE5\endcsname{51.7}
\expandafter\def\csname v@S6@CL-ucmd@IAE\endcsname{1.758}
\expandafter\def\csname v@S6@CL-ucmd@PSIE\endcsname{1.05}
\expandafter\def\csname v@S6@CL-ucmd@TV\endcsname{134}
\expandafter\def\csname v@S6@CL-ucmd@DW\endcsname{0.11}
\expandafter\def\csname v@S6@CL-ucmd@WSAT\endcsname{0.0}
\expandafter\def\csname v@S6@CL-ucmd@DHAT\endcsname{0.076}
\expandafter\def\csname v@S6@CL-ucmd@DHATP\endcsname{0.075}
\expandafter\def\csname v@S6@CL-ucmd@Trx\endcsname{1.00}
\expandafter\def\csname v@S6@CL-ucmd@Tsx\endcsname{6.44}
\expandafter\def\csname v@S6@CL-ucmd@OSx\endcsname{5.87}
\expandafter\def\csname v@S6@CL-ucmd@SSEx\endcsname{5.41}
\expandafter\def\csname v@S6@CL-ucmd@Trz\endcsname{1.14}
\expandafter\def\csname v@S6@CL-ucmd@Tsz\endcsname{4.33}
\expandafter\def\csname v@S6@CL-ucmd@OSz\endcsname{7.03}
\expandafter\def\csname v@S6@CL-ucmd@SSEz\endcsname{0.64}
\expandafter\def\csname v@S6@CL-att@RMSE\endcsname{413.3}
\expandafter\def\csname v@S6@CL-att@RMSE5\endcsname{0.3}
\expandafter\def\csname v@S6@CL-att@MAXE5\endcsname{1.4}
\expandafter\def\csname v@S6@CL-att@IAE\endcsname{1.455}
\expandafter\def\csname v@S6@CL-att@PSIE\endcsname{1.00}
\expandafter\def\csname v@S6@CL-att@TV\endcsname{141}
\expandafter\def\csname v@S6@CL-att@DW\endcsname{0.16}
\expandafter\def\csname v@S6@CL-att@WSAT\endcsname{0.0}
\expandafter\def\csname v@S6@CL-att@DHAT\endcsname{0.000}
\expandafter\def\csname v@S6@CL-att@DHATP\endcsname{0.000}
\expandafter\def\csname v@S6@CL-att@Trx\endcsname{0.87}
\expandafter\def\csname v@S6@CL-att@Tsx\endcsname{2.84}
\expandafter\def\csname v@S6@CL-att@OSx\endcsname{5.27}
\expandafter\def\csname v@S6@CL-att@SSEx\endcsname{0.00}
\expandafter\def\csname v@S6@CL-att@Trz\endcsname{1.15}
\expandafter\def\csname v@S6@CL-att@Tsz\endcsname{3.34}
\expandafter\def\csname v@S6@CL-att@OSz\endcsname{5.01}
\expandafter\def\csname v@S6@CL-att@SSEz\endcsname{0.00}
\expandafter\def\csname v@S6@PROPOSED@RMSE\endcsname{406.6}
\expandafter\def\csname v@S6@PROPOSED@RMSE5\endcsname{0.4}
\expandafter\def\csname v@S6@PROPOSED@MAXE5\endcsname{1.7}
\expandafter\def\csname v@S6@PROPOSED@IAE\endcsname{1.402}
\expandafter\def\csname v@S6@PROPOSED@PSIE\endcsname{1.66}
\expandafter\def\csname v@S6@PROPOSED@TV\endcsname{447}
\expandafter\def\csname v@S6@PROPOSED@DW\endcsname{0.58}
\expandafter\def\csname v@S6@PROPOSED@WSAT\endcsname{0.0}
\expandafter\def\csname v@S6@PROPOSED@DHAT\endcsname{0.000}
\expandafter\def\csname v@S6@PROPOSED@DHATP\endcsname{0.000}
\expandafter\def\csname v@S6@PROPOSED@Trx\endcsname{0.97}
\expandafter\def\csname v@S6@PROPOSED@Tsx\endcsname{2.76}
\expandafter\def\csname v@S6@PROPOSED@OSx\endcsname{3.14}
\expandafter\def\csname v@S6@PROPOSED@SSEx\endcsname{0.00}
\expandafter\def\csname v@S6@PROPOSED@Trz\endcsname{1.15}
\expandafter\def\csname v@S6@PROPOSED@Tsz\endcsname{2.92}
\expandafter\def\csname v@S6@PROPOSED@OSz\endcsname{3.83}
\expandafter\def\csname v@S6@PROPOSED@SSEz\endcsname{0.00}
\expandafter\def\csname v@S6@LQR@IMP\endcsname{-1531}
\expandafter\def\csname v@S6@MRAC@IMP\endcsname{93}
\expandafter\def\csname v@S6@B1@IMP\endcsname{98}
\expandafter\def\csname v@S6@NN-MRAC@IMP\endcsname{78}
\expandafter\def\csname v@S6@CL-ucmd@IMP\endcsname{99}
\expandafter\def\csname v@S6@CL-att@IMP\endcsname{-16}
\expandafter\def\csname v@S7@LQR@RMSE\endcsname{306.5}
\expandafter\def\csname v@S7@LQR@RMSE5\endcsname{1.2}
\expandafter\def\csname v@S7@LQR@MAXE5\endcsname{1.9}
\expandafter\def\csname v@S7@LQR@IAE\endcsname{1.551}
\expandafter\def\csname v@S7@LQR@PSIE\endcsname{0.48}
\expandafter\def\csname v@S7@LQR@TV\endcsname{39516}
\expandafter\def\csname v@S7@LQR@DW\endcsname{12.41}
\expandafter\def\csname v@S7@LQR@WSAT\endcsname{0.0}
\expandafter\def\csname v@S7@LQR@DHAT\endcsname{0.120}
\expandafter\def\csname v@S7@LQR@DHATP\endcsname{0.001}
\expandafter\def\csname v@S7@LQR@Trx\endcsname{1.08}
\expandafter\def\csname v@S7@LQR@Tsx\endcsname{1.96}
\expandafter\def\csname v@S7@LQR@OSx\endcsname{0.17}
\expandafter\def\csname v@S7@LQR@SSEx\endcsname{0.25}
\expandafter\def\csname v@S7@LQR@Trz\endcsname{1.35}
\expandafter\def\csname v@S7@LQR@Tsz\endcsname{2.15}
\expandafter\def\csname v@S7@LQR@OSz\endcsname{0.41}
\expandafter\def\csname v@S7@LQR@SSEz\endcsname{0.83}
\expandafter\def\csname v@S7@MRAC@RMSE\endcsname{295.8}
\expandafter\def\csname v@S7@MRAC@RMSE5\endcsname{3.6}
\expandafter\def\csname v@S7@MRAC@MAXE5\endcsname{11.1}
\expandafter\def\csname v@S7@MRAC@IAE\endcsname{1.591}
\expandafter\def\csname v@S7@MRAC@PSIE\endcsname{0.83}
\expandafter\def\csname v@S7@MRAC@TV\endcsname{40368}
\expandafter\def\csname v@S7@MRAC@DW\endcsname{12.68}
\expandafter\def\csname v@S7@MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S7@MRAC@DHAT\endcsname{0.122}
\expandafter\def\csname v@S7@MRAC@DHATP\endcsname{0.039}
\expandafter\def\csname v@S7@MRAC@Trx\endcsname{1.23}
\expandafter\def\csname v@S7@MRAC@Tsx\endcsname{3.78}
\expandafter\def\csname v@S7@MRAC@OSx\endcsname{6.91}
\expandafter\def\csname v@S7@MRAC@SSEx\endcsname{0.90}
\expandafter\def\csname v@S7@MRAC@Trz\endcsname{1.14}
\expandafter\def\csname v@S7@MRAC@Tsz\endcsname{3.23}
\expandafter\def\csname v@S7@MRAC@OSz\endcsname{6.19}
\expandafter\def\csname v@S7@MRAC@SSEz\endcsname{0.57}
\expandafter\def\csname v@S7@B1@RMSE\endcsname{290.7}
\expandafter\def\csname v@S7@B1@RMSE5\endcsname{8.7}
\expandafter\def\csname v@S7@B1@MAXE5\endcsname{23.0}
\expandafter\def\csname v@S7@B1@IAE\endcsname{1.590}
\expandafter\def\csname v@S7@B1@PSIE\endcsname{0.87}
\expandafter\def\csname v@S7@B1@TV\endcsname{32797}
\expandafter\def\csname v@S7@B1@DW\endcsname{10.76}
\expandafter\def\csname v@S7@B1@WSAT\endcsname{0.0}
\expandafter\def\csname v@S7@B1@DHAT\endcsname{0.321}
\expandafter\def\csname v@S7@B1@DHATP\endcsname{0.350}
\expandafter\def\csname v@S7@B1@Trx\endcsname{1.01}
\expandafter\def\csname v@S7@B1@Tsx\endcsname{5.87}
\expandafter\def\csname v@S7@B1@OSx\endcsname{7.48}
\expandafter\def\csname v@S7@B1@SSEx\endcsname{2.09}
\expandafter\def\csname v@S7@B1@Trz\endcsname{1.32}
\expandafter\def\csname v@S7@B1@Tsz\endcsname{1.82}
\expandafter\def\csname v@S7@B1@OSz\endcsname{1.45}
\expandafter\def\csname v@S7@B1@SSEz\endcsname{0.47}
\expandafter\def\csname v@S7@NN-MRAC@RMSE\endcsname{297.8}
\expandafter\def\csname v@S7@NN-MRAC@RMSE5\endcsname{1.6}
\expandafter\def\csname v@S7@NN-MRAC@MAXE5\endcsname{6.0}
\expandafter\def\csname v@S7@NN-MRAC@IAE\endcsname{1.599}
\expandafter\def\csname v@S7@NN-MRAC@PSIE\endcsname{0.71}
\expandafter\def\csname v@S7@NN-MRAC@TV\endcsname{39839}
\expandafter\def\csname v@S7@NN-MRAC@DW\endcsname{12.51}
\expandafter\def\csname v@S7@NN-MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S7@NN-MRAC@DHAT\endcsname{0.121}
\expandafter\def\csname v@S7@NN-MRAC@DHATP\endcsname{0.016}
\expandafter\def\csname v@S7@NN-MRAC@Trx\endcsname{1.04}
\expandafter\def\csname v@S7@NN-MRAC@Tsx\endcsname{3.99}
\expandafter\def\csname v@S7@NN-MRAC@OSx\endcsname{5.56}
\expandafter\def\csname v@S7@NN-MRAC@SSEx\endcsname{0.36}
\expandafter\def\csname v@S7@NN-MRAC@Trz\endcsname{1.16}
\expandafter\def\csname v@S7@NN-MRAC@Tsz\endcsname{3.73}
\expandafter\def\csname v@S7@NN-MRAC@OSz\endcsname{6.92}
\expandafter\def\csname v@S7@NN-MRAC@SSEz\endcsname{0.27}
\expandafter\def\csname v@S7@CL-ucmd@RMSE\endcsname{297.9}
\expandafter\def\csname v@S7@CL-ucmd@RMSE5\endcsname{15.0}
\expandafter\def\csname v@S7@CL-ucmd@MAXE5\endcsname{52.0}
\expandafter\def\csname v@S7@CL-ucmd@IAE\endcsname{1.776}
\expandafter\def\csname v@S7@CL-ucmd@PSIE\endcsname{0.75}
\expandafter\def\csname v@S7@CL-ucmd@TV\endcsname{40440}
\expandafter\def\csname v@S7@CL-ucmd@DW\endcsname{12.70}
\expandafter\def\csname v@S7@CL-ucmd@WSAT\endcsname{0.0}
\expandafter\def\csname v@S7@CL-ucmd@DHAT\endcsname{0.129}
\expandafter\def\csname v@S7@CL-ucmd@DHATP\endcsname{0.054}
\expandafter\def\csname v@S7@CL-ucmd@Trx\endcsname{1.00}
\expandafter\def\csname v@S7@CL-ucmd@Tsx\endcsname{6.42}
\expandafter\def\csname v@S7@CL-ucmd@OSx\endcsname{5.98}
\expandafter\def\csname v@S7@CL-ucmd@SSEx\endcsname{0.40}
\expandafter\def\csname v@S7@CL-ucmd@Trz\endcsname{1.14}
\expandafter\def\csname v@S7@CL-ucmd@Tsz\endcsname{4.29}
\expandafter\def\csname v@S7@CL-ucmd@OSz\endcsname{6.91}
\expandafter\def\csname v@S7@CL-ucmd@SSEz\endcsname{0.33}
\expandafter\def\csname v@S7@CL-att@RMSE\endcsname{292.2}
\expandafter\def\csname v@S7@CL-att@RMSE5\endcsname{1.2}
\expandafter\def\csname v@S7@CL-att@MAXE5\endcsname{2.0}
\expandafter\def\csname v@S7@CL-att@IAE\endcsname{1.468}
\expandafter\def\csname v@S7@CL-att@PSIE\endcsname{0.71}
\expandafter\def\csname v@S7@CL-att@TV\endcsname{41160}
\expandafter\def\csname v@S7@CL-att@DW\endcsname{12.93}
\expandafter\def\csname v@S7@CL-att@WSAT\endcsname{0.0}
\expandafter\def\csname v@S7@CL-att@DHAT\endcsname{0.121}
\expandafter\def\csname v@S7@CL-att@DHATP\endcsname{0.018}
\expandafter\def\csname v@S7@CL-att@Trx\endcsname{0.87}
\expandafter\def\csname v@S7@CL-att@Tsx\endcsname{2.84}
\expandafter\def\csname v@S7@CL-att@OSx\endcsname{5.31}
\expandafter\def\csname v@S7@CL-att@SSEx\endcsname{0.43}
\expandafter\def\csname v@S7@CL-att@Trz\endcsname{1.15}
\expandafter\def\csname v@S7@CL-att@Tsz\endcsname{3.32}
\expandafter\def\csname v@S7@CL-att@OSz\endcsname{4.90}
\expandafter\def\csname v@S7@CL-att@SSEz\endcsname{0.41}
\expandafter\def\csname v@S7@PROPOSED@RMSE\endcsname{287.5}
\expandafter\def\csname v@S7@PROPOSED@RMSE5\endcsname{1.3}
\expandafter\def\csname v@S7@PROPOSED@MAXE5\endcsname{2.5}
\expandafter\def\csname v@S7@PROPOSED@IAE\endcsname{1.419}
\expandafter\def\csname v@S7@PROPOSED@PSIE\endcsname{1.16}
\expandafter\def\csname v@S7@PROPOSED@TV\endcsname{41253}
\expandafter\def\csname v@S7@PROPOSED@DW\endcsname{12.98}
\expandafter\def\csname v@S7@PROPOSED@WSAT\endcsname{0.0}
\expandafter\def\csname v@S7@PROPOSED@DHAT\endcsname{0.122}
\expandafter\def\csname v@S7@PROPOSED@DHATP\endcsname{0.050}
\expandafter\def\csname v@S7@PROPOSED@Trx\endcsname{0.96}
\expandafter\def\csname v@S7@PROPOSED@Tsx\endcsname{2.77}
\expandafter\def\csname v@S7@PROPOSED@OSx\endcsname{3.00}
\expandafter\def\csname v@S7@PROPOSED@SSEx\endcsname{0.58}
\expandafter\def\csname v@S7@PROPOSED@Trz\endcsname{1.16}
\expandafter\def\csname v@S7@PROPOSED@Tsz\endcsname{2.88}
\expandafter\def\csname v@S7@PROPOSED@OSz\endcsname{3.68}
\expandafter\def\csname v@S7@PROPOSED@SSEz\endcsname{0.92}
\expandafter\def\csname v@S7@LQR@IMP\endcsname{-11}
\expandafter\def\csname v@S7@MRAC@IMP\endcsname{63}
\expandafter\def\csname v@S7@B1@IMP\endcsname{85}
\expandafter\def\csname v@S7@NN-MRAC@IMP\endcsname{15}
\expandafter\def\csname v@S7@CL-ucmd@IMP\endcsname{91}
\expandafter\def\csname v@S7@CL-att@IMP\endcsname{-16}
\expandafter\def\csname v@S8@LQR@RMSE\endcsname{445.6}
\expandafter\def\csname v@S8@LQR@RMSE5\endcsname{465.8}
\expandafter\def\csname v@S8@LQR@MAXE5\endcsname{743.8}
\expandafter\def\csname v@S8@LQR@IAE\endcsname{16.943}
\expandafter\def\csname v@S8@LQR@PSIE\endcsname{0.76}
\expandafter\def\csname v@S8@LQR@TV\endcsname{37476}
\expandafter\def\csname v@S8@LQR@DW\endcsname{11.76}
\expandafter\def\csname v@S8@LQR@WSAT\endcsname{0.0}
\expandafter\def\csname v@S8@LQR@DHAT\endcsname{1.947}
\expandafter\def\csname v@S8@LQR@DHATP\endcsname{1.812}
\expandafter\def\csname v@S8@MRAC@RMSE\endcsname{69.0}
\expandafter\def\csname v@S8@MRAC@RMSE5\endcsname{68.0}
\expandafter\def\csname v@S8@MRAC@MAXE5\endcsname{156.7}
\expandafter\def\csname v@S8@MRAC@IAE\endcsname{2.494}
\expandafter\def\csname v@S8@MRAC@PSIE\endcsname{0.78}
\expandafter\def\csname v@S8@MRAC@TV\endcsname{38517}
\expandafter\def\csname v@S8@MRAC@DW\endcsname{12.09}
\expandafter\def\csname v@S8@MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S8@MRAC@DHAT\endcsname{0.410}
\expandafter\def\csname v@S8@MRAC@DHATP\endcsname{0.401}
\expandafter\def\csname v@S8@B1@RMSE\endcsname{18889.7}
\expandafter\def\csname v@S8@B1@RMSE5\endcsname{23549.2}
\expandafter\def\csname v@S8@B1@MAXE5\endcsname{49975.9}
\expandafter\def\csname v@S8@B1@IAE\endcsname{158.282}
\expandafter\def\csname v@S8@B1@PSIE\endcsname{77.78}
\expandafter\def\csname v@S8@B1@TV\endcsname{22148}
\expandafter\def\csname v@S8@B1@DW\endcsname{16.32}
\expandafter\def\csname v@S8@B1@WSAT\endcsname{46.5}
\expandafter\def\csname v@S8@B1@DHAT\endcsname{115.598}
\expandafter\def\csname v@S8@B1@DHATP\endcsname{187.147}
\expandafter\def\csname v@S8@NN-MRAC@RMSE\endcsname{93.1}
\expandafter\def\csname v@S8@NN-MRAC@RMSE5\endcsname{92.6}
\expandafter\def\csname v@S8@NN-MRAC@MAXE5\endcsname{171.5}
\expandafter\def\csname v@S8@NN-MRAC@IAE\endcsname{3.436}
\expandafter\def\csname v@S8@NN-MRAC@PSIE\endcsname{0.77}
\expandafter\def\csname v@S8@NN-MRAC@TV\endcsname{38535}
\expandafter\def\csname v@S8@NN-MRAC@DW\endcsname{12.10}
\expandafter\def\csname v@S8@NN-MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S8@NN-MRAC@DHAT\endcsname{0.506}
\expandafter\def\csname v@S8@NN-MRAC@DHATP\endcsname{0.318}
\expandafter\def\csname v@S8@CL-ucmd@RMSE\endcsname{97.1}
\expandafter\def\csname v@S8@CL-ucmd@RMSE5\endcsname{97.7}
\expandafter\def\csname v@S8@CL-ucmd@MAXE5\endcsname{197.1}
\expandafter\def\csname v@S8@CL-ucmd@IAE\endcsname{3.513}
\expandafter\def\csname v@S8@CL-ucmd@PSIE\endcsname{0.74}
\expandafter\def\csname v@S8@CL-ucmd@TV\endcsname{53934}
\expandafter\def\csname v@S8@CL-ucmd@DW\endcsname{17.43}
\expandafter\def\csname v@S8@CL-ucmd@WSAT\endcsname{0.0}
\expandafter\def\csname v@S8@CL-ucmd@DHAT\endcsname{0.488}
\expandafter\def\csname v@S8@CL-ucmd@DHATP\endcsname{0.407}
\expandafter\def\csname v@S8@CL-att@RMSE\endcsname{71.2}
\expandafter\def\csname v@S8@CL-att@RMSE5\endcsname{69.5}
\expandafter\def\csname v@S8@CL-att@MAXE5\endcsname{124.7}
\expandafter\def\csname v@S8@CL-att@IAE\endcsname{2.641}
\expandafter\def\csname v@S8@CL-att@PSIE\endcsname{0.75}
\expandafter\def\csname v@S8@CL-att@TV\endcsname{58711}
\expandafter\def\csname v@S8@CL-att@DW\endcsname{19.02}
\expandafter\def\csname v@S8@CL-att@WSAT\endcsname{0.0}
\expandafter\def\csname v@S8@CL-att@DHAT\endcsname{0.394}
\expandafter\def\csname v@S8@CL-att@DHATP\endcsname{0.251}
\expandafter\def\csname v@S8@PROPOSED@RMSE\endcsname{51.0}
\expandafter\def\csname v@S8@PROPOSED@RMSE5\endcsname{51.2}
\expandafter\def\csname v@S8@PROPOSED@MAXE5\endcsname{115.5}
\expandafter\def\csname v@S8@PROPOSED@IAE\endcsname{1.866}
\expandafter\def\csname v@S8@PROPOSED@PSIE\endcsname{0.72}
\expandafter\def\csname v@S8@PROPOSED@TV\endcsname{66759}
\expandafter\def\csname v@S8@PROPOSED@DW\endcsname{21.87}
\expandafter\def\csname v@S8@PROPOSED@WSAT\endcsname{0.0}
\expandafter\def\csname v@S8@PROPOSED@DHAT\endcsname{0.327}
\expandafter\def\csname v@S8@PROPOSED@DHATP\endcsname{0.259}
\expandafter\def\csname v@S8@LQR@IMP\endcsname{89}
\expandafter\def\csname v@S8@MRAC@IMP\endcsname{25}
\expandafter\def\csname v@S8@B1@IMP\endcsname{100}
\expandafter\def\csname v@S8@NN-MRAC@IMP\endcsname{45}
\expandafter\def\csname v@S8@CL-ucmd@IMP\endcsname{48}
\expandafter\def\csname v@S8@CL-att@IMP\endcsname{26}
\expandafter\def\csname v@S9@LQR@RMSE\endcsname{535.6}
\expandafter\def\csname v@S9@LQR@RMSE5\endcsname{552.7}
\expandafter\def\csname v@S9@LQR@MAXE5\endcsname{840.1}
\expandafter\def\csname v@S9@LQR@IAE\endcsname{29.889}
\expandafter\def\csname v@S9@LQR@PSIE\endcsname{2.07}
\expandafter\def\csname v@S9@LQR@TV\endcsname{42744}
\expandafter\def\csname v@S9@LQR@DW\endcsname{13.67}
\expandafter\def\csname v@S9@LQR@WSAT\endcsname{0.0}
\expandafter\def\csname v@S9@LQR@DHAT\endcsname{2.598}
\expandafter\def\csname v@S9@LQR@DHATP\endcsname{2.338}
\expandafter\def\csname v@S9@MRAC@RMSE\endcsname{146.9}
\expandafter\def\csname v@S9@MRAC@RMSE5\endcsname{147.6}
\expandafter\def\csname v@S9@MRAC@MAXE5\endcsname{341.0}
\expandafter\def\csname v@S9@MRAC@IAE\endcsname{7.320}
\expandafter\def\csname v@S9@MRAC@PSIE\endcsname{2.94}
\expandafter\def\csname v@S9@MRAC@TV\endcsname{100375}
\expandafter\def\csname v@S9@MRAC@DW\endcsname{38.36}
\expandafter\def\csname v@S9@MRAC@WSAT\endcsname{5.3}
\expandafter\def\csname v@S9@MRAC@DHAT\endcsname{2.312}
\expandafter\def\csname v@S9@MRAC@DHATP\endcsname{2.857}
\expandafter\def\csname v@S9@B1@RMSE\endcsname{20693.6}
\expandafter\def\csname v@S9@B1@RMSE5\endcsname{23526.0}
\expandafter\def\csname v@S9@B1@MAXE5\endcsname{49996.8}
\expandafter\def\csname v@S9@B1@IAE\endcsname{361.961}
\expandafter\def\csname v@S9@B1@PSIE\endcsname{95.51}
\expandafter\def\csname v@S9@B1@TV\endcsname{27150}
\expandafter\def\csname v@S9@B1@DW\endcsname{31.31}
\expandafter\def\csname v@S9@B1@WSAT\endcsname{82.7}
\expandafter\def\csname v@S9@B1@DHAT\endcsname{228.527}
\expandafter\def\csname v@S9@B1@DHATP\endcsname{583.141}
\expandafter\def\csname v@S9@NN-MRAC@RMSE\endcsname{124.7}
\expandafter\def\csname v@S9@NN-MRAC@RMSE5\endcsname{125.9}
\expandafter\def\csname v@S9@NN-MRAC@MAXE5\endcsname{291.0}
\expandafter\def\csname v@S9@NN-MRAC@IAE\endcsname{6.343}
\expandafter\def\csname v@S9@NN-MRAC@PSIE\endcsname{2.66}
\expandafter\def\csname v@S9@NN-MRAC@TV\endcsname{54798}
\expandafter\def\csname v@S9@NN-MRAC@DW\endcsname{18.80}
\expandafter\def\csname v@S9@NN-MRAC@WSAT\endcsname{0.8}
\expandafter\def\csname v@S9@NN-MRAC@DHAT\endcsname{1.660}
\expandafter\def\csname v@S9@NN-MRAC@DHATP\endcsname{1.363}
\expandafter\def\csname v@S9@CL-ucmd@RMSE\endcsname{137.2}
\expandafter\def\csname v@S9@CL-ucmd@RMSE5\endcsname{137.8}
\expandafter\def\csname v@S9@CL-ucmd@MAXE5\endcsname{295.4}
\expandafter\def\csname v@S9@CL-ucmd@IAE\endcsname{7.499}
\expandafter\def\csname v@S9@CL-ucmd@PSIE\endcsname{2.18}
\expandafter\def\csname v@S9@CL-ucmd@TV\endcsname{71023}
\expandafter\def\csname v@S9@CL-ucmd@DW\endcsname{23.76}
\expandafter\def\csname v@S9@CL-ucmd@WSAT\endcsname{0.6}
\expandafter\def\csname v@S9@CL-ucmd@DHAT\endcsname{1.330}
\expandafter\def\csname v@S9@CL-ucmd@DHATP\endcsname{1.137}
\expandafter\def\csname v@S9@CL-att@RMSE\endcsname{67.6}
\expandafter\def\csname v@S9@CL-att@RMSE5\endcsname{67.7}
\expandafter\def\csname v@S9@CL-att@MAXE5\endcsname{157.1}
\expandafter\def\csname v@S9@CL-att@IAE\endcsname{3.556}
\expandafter\def\csname v@S9@CL-att@PSIE\endcsname{2.36}
\expandafter\def\csname v@S9@CL-att@TV\endcsname{73213}
\expandafter\def\csname v@S9@CL-att@DW\endcsname{24.21}
\expandafter\def\csname v@S9@CL-att@WSAT\endcsname{0.5}
\expandafter\def\csname v@S9@CL-att@DHAT\endcsname{1.044}
\expandafter\def\csname v@S9@CL-att@DHATP\endcsname{0.673}
\expandafter\def\csname v@S9@PROPOSED@RMSE\endcsname{55.5}
\expandafter\def\csname v@S9@PROPOSED@RMSE5\endcsname{57.0}
\expandafter\def\csname v@S9@PROPOSED@MAXE5\endcsname{140.4}
\expandafter\def\csname v@S9@PROPOSED@IAE\endcsname{2.932}
\expandafter\def\csname v@S9@PROPOSED@PSIE\endcsname{2.47}
\expandafter\def\csname v@S9@PROPOSED@TV\endcsname{82824}
\expandafter\def\csname v@S9@PROPOSED@DW\endcsname{27.66}
\expandafter\def\csname v@S9@PROPOSED@WSAT\endcsname{0.9}
\expandafter\def\csname v@S9@PROPOSED@DHAT\endcsname{1.137}
\expandafter\def\csname v@S9@PROPOSED@DHATP\endcsname{0.971}
\expandafter\def\csname v@S9@LQR@IMP\endcsname{90}
\expandafter\def\csname v@S9@MRAC@IMP\endcsname{61}
\expandafter\def\csname v@S9@B1@IMP\endcsname{100}
\expandafter\def\csname v@S9@NN-MRAC@IMP\endcsname{55}
\expandafter\def\csname v@S9@CL-ucmd@IMP\endcsname{59}
\expandafter\def\csname v@S9@CL-att@IMP\endcsname{16}
\expandafter\def\csname v@S10@LQR@RMSE\endcsname{576.6}
\expandafter\def\csname v@S10@LQR@RMSE5\endcsname{591.1}
\expandafter\def\csname v@S10@LQR@MAXE5\endcsname{756.2}
\expandafter\def\csname v@S10@LQR@IAE\endcsname{17.099}
\expandafter\def\csname v@S10@LQR@PSIE\endcsname{0.52}
\expandafter\def\csname v@S10@LQR@TV\endcsname{35905}
\expandafter\def\csname v@S10@LQR@DW\endcsname{11.27}
\expandafter\def\csname v@S10@LQR@WSAT\endcsname{0.0}
\expandafter\def\csname v@S10@LQR@DHAT\endcsname{2.459}
\expandafter\def\csname v@S10@LQR@DHATP\endcsname{2.389}
\expandafter\def\csname v@S10@MRAC@RMSE\endcsname{139.9}
\expandafter\def\csname v@S10@MRAC@RMSE5\endcsname{112.2}
\expandafter\def\csname v@S10@MRAC@MAXE5\endcsname{158.6}
\expandafter\def\csname v@S10@MRAC@IAE\endcsname{3.808}
\expandafter\def\csname v@S10@MRAC@PSIE\endcsname{1.32}
\expandafter\def\csname v@S10@MRAC@TV\endcsname{51260}
\expandafter\def\csname v@S10@MRAC@DW\endcsname{16.38}
\expandafter\def\csname v@S10@MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S10@MRAC@DHAT\endcsname{1.214}
\expandafter\def\csname v@S10@MRAC@DHATP\endcsname{1.056}
\expandafter\def\csname v@S10@B1@RMSE\endcsname{23706.3}
\expandafter\def\csname v@S10@B1@RMSE5\endcsname{34132.4}
\expandafter\def\csname v@S10@B1@MAXE5\endcsname{49956.6}
\expandafter\def\csname v@S10@B1@IAE\endcsname{161.173}
\expandafter\def\csname v@S10@B1@PSIE\endcsname{79.04}
\expandafter\def\csname v@S10@B1@TV\endcsname{18419}
\expandafter\def\csname v@S10@B1@DW\endcsname{15.24}
\expandafter\def\csname v@S10@B1@WSAT\endcsname{68.0}
\expandafter\def\csname v@S10@B1@DHAT\endcsname{161.805}
\expandafter\def\csname v@S10@B1@DHATP\endcsname{243.222}
\expandafter\def\csname v@S10@NN-MRAC@RMSE\endcsname{126.7}
\expandafter\def\csname v@S10@NN-MRAC@RMSE5\endcsname{96.3}
\expandafter\def\csname v@S10@NN-MRAC@MAXE5\endcsname{149.8}
\expandafter\def\csname v@S10@NN-MRAC@IAE\endcsname{3.232}
\expandafter\def\csname v@S10@NN-MRAC@PSIE\endcsname{0.79}
\expandafter\def\csname v@S10@NN-MRAC@TV\endcsname{38123}
\expandafter\def\csname v@S10@NN-MRAC@DW\endcsname{11.99}
\expandafter\def\csname v@S10@NN-MRAC@WSAT\endcsname{0.0}
\expandafter\def\csname v@S10@NN-MRAC@DHAT\endcsname{0.798}
\expandafter\def\csname v@S10@NN-MRAC@DHATP\endcsname{0.483}
\expandafter\def\csname v@S10@CL-ucmd@RMSE\endcsname{112.2}
\expandafter\def\csname v@S10@CL-ucmd@RMSE5\endcsname{77.3}
\expandafter\def\csname v@S10@CL-ucmd@MAXE5\endcsname{202.4}
\expandafter\def\csname v@S10@CL-ucmd@IAE\endcsname{2.514}
\expandafter\def\csname v@S10@CL-ucmd@PSIE\endcsname{0.53}
\expandafter\def\csname v@S10@CL-ucmd@TV\endcsname{45806}
\expandafter\def\csname v@S10@CL-ucmd@DW\endcsname{14.47}
\expandafter\def\csname v@S10@CL-ucmd@WSAT\endcsname{0.0}
\expandafter\def\csname v@S10@CL-ucmd@DHAT\endcsname{0.471}
\expandafter\def\csname v@S10@CL-ucmd@DHATP\endcsname{0.324}
\expandafter\def\csname v@S10@CL-att@RMSE\endcsname{74.1}
\expandafter\def\csname v@S10@CL-att@RMSE5\endcsname{36.7}
\expandafter\def\csname v@S10@CL-att@MAXE5\endcsname{62.7}
\expandafter\def\csname v@S10@CL-att@IAE\endcsname{1.464}
\expandafter\def\csname v@S10@CL-att@PSIE\endcsname{0.50}
\expandafter\def\csname v@S10@CL-att@TV\endcsname{54114}
\expandafter\def\csname v@S10@CL-att@DW\endcsname{17.19}
\expandafter\def\csname v@S10@CL-att@WSAT\endcsname{0.0}
\expandafter\def\csname v@S10@CL-att@DHAT\endcsname{0.360}
\expandafter\def\csname v@S10@CL-att@DHATP\endcsname{0.122}
\expandafter\def\csname v@S10@PROPOSED@RMSE\endcsname{64.4}
\expandafter\def\csname v@S10@PROPOSED@RMSE5\endcsname{27.3}
\expandafter\def\csname v@S10@PROPOSED@MAXE5\endcsname{43.9}
\expandafter\def\csname v@S10@PROPOSED@IAE\endcsname{1.142}
\expandafter\def\csname v@S10@PROPOSED@PSIE\endcsname{0.55}
\expandafter\def\csname v@S10@PROPOSED@TV\endcsname{72849}
\expandafter\def\csname v@S10@PROPOSED@DW\endcsname{23.33}
\expandafter\def\csname v@S10@PROPOSED@WSAT\endcsname{0.0}
\expandafter\def\csname v@S10@PROPOSED@DHAT\endcsname{0.437}
\expandafter\def\csname v@S10@PROPOSED@DHATP\endcsname{0.310}
\expandafter\def\csname v@S10@LQR@IMP\endcsname{95}
\expandafter\def\csname v@S10@MRAC@IMP\endcsname{76}
\expandafter\def\csname v@S10@B1@IMP\endcsname{100}
\expandafter\def\csname v@S10@NN-MRAC@IMP\endcsname{72}
\expandafter\def\csname v@S10@CL-ucmd@IMP\endcsname{65}
\expandafter\def\csname v@S10@CL-att@IMP\endcsname{26}
\expandafter\def\csname v@S234@LQR@IMPmin\endcsname{87}
\expandafter\def\csname v@S234@LQR@IMPmax\endcsname{92}
\expandafter\def\csname v@S234@MRAC@IMPmin\endcsname{53}
\expandafter\def\csname v@S234@MRAC@IMPmax\endcsname{64}
\expandafter\def\csname v@S234@B1@IMPmin\endcsname{68}
\expandafter\def\csname v@S234@B1@IMPmax\endcsname{100}
\expandafter\def\csname v@S234@NN-MRAC@IMPmin\endcsname{44}
\expandafter\def\csname v@S234@NN-MRAC@IMPmax\endcsname{69}
\expandafter\def\csname v@S234@CL-ucmd@IMPmin\endcsname{43}
\expandafter\def\csname v@S234@CL-ucmd@IMPmax\endcsname{63}
\expandafter\def\csname v@S234@CL-att@IMPmin\endcsname{14}
\expandafter\def\csname v@S234@CL-att@IMPmax\endcsname{34}
\expandafter\def\csname v@tune@LQR@go\endcsname{0}
\expandafter\def\csname v@tune@LQR@gi\endcsname{0}
\expandafter\def\csname v@tune@LQR@lo\endcsname{0}
\expandafter\def\csname v@tune@LQR@li\endcsname{0}
\expandafter\def\csname v@tune@LQR@kc\endcsname{0}
\expandafter\def\csname v@tune@LQR@lam\endcsname{0.5}
\expandafter\def\csname v@tune@LQR@mu\endcsname{0}
\expandafter\def\csname v@tune@MRAC@go\endcsname{40}
\expandafter\def\csname v@tune@MRAC@gi\endcsname{400}
\expandafter\def\csname v@tune@MRAC@lo\endcsname{0}
\expandafter\def\csname v@tune@MRAC@li\endcsname{0}
\expandafter\def\csname v@tune@MRAC@kc\endcsname{0}
\expandafter\def\csname v@tune@MRAC@lam\endcsname{0.5}
\expandafter\def\csname v@tune@MRAC@mu\endcsname{0}
\expandafter\def\csname v@tune@MRAC@J\endcsname{86.5}
\expandafter\def\csname v@tune@MRAC@n\endcsname{11}
\expandafter\def\csname v@tune@B1@go\endcsname{0}
\expandafter\def\csname v@tune@B1@gi\endcsname{0}
\expandafter\def\csname v@tune@B1@lo\endcsname{0}
\expandafter\def\csname v@tune@B1@li\endcsname{0}
\expandafter\def\csname v@tune@B1@kc\endcsname{0}
\expandafter\def\csname v@tune@B1@lam\endcsname{0.5}
\expandafter\def\csname v@tune@B1@mu\endcsname{0.2}
\expandafter\def\csname v@tune@B1@J\endcsname{Inf}
\expandafter\def\csname v@tune@B1@n\endcsname{5}
\expandafter\def\csname v@tune@NN-MRAC@go\endcsname{40}
\expandafter\def\csname v@tune@NN-MRAC@gi\endcsname{400}
\expandafter\def\csname v@tune@NN-MRAC@lo\endcsname{5}
\expandafter\def\csname v@tune@NN-MRAC@li\endcsname{25}
\expandafter\def\csname v@tune@NN-MRAC@kc\endcsname{0}
\expandafter\def\csname v@tune@NN-MRAC@lam\endcsname{0.5}
\expandafter\def\csname v@tune@NN-MRAC@mu\endcsname{0}
\expandafter\def\csname v@tune@NN-MRAC@J\endcsname{82.6}
\expandafter\def\csname v@tune@NN-MRAC@n\endcsname{22}
\expandafter\def\csname v@tune@CL-ucmd@go\endcsname{20}
\expandafter\def\csname v@tune@CL-ucmd@gi\endcsname{200}
\expandafter\def\csname v@tune@CL-ucmd@lo\endcsname{0}
\expandafter\def\csname v@tune@CL-ucmd@li\endcsname{0}
\expandafter\def\csname v@tune@CL-ucmd@kc\endcsname{0.25}
\expandafter\def\csname v@tune@CL-ucmd@lam\endcsname{0.5}
\expandafter\def\csname v@tune@CL-ucmd@mu\endcsname{0}
\expandafter\def\csname v@tune@CL-ucmd@J\endcsname{77.8}
\expandafter\def\csname v@tune@CL-ucmd@n\endcsname{132}
\expandafter\def\csname v@tune@CL-att@go\endcsname{160}
\expandafter\def\csname v@tune@CL-att@gi\endcsname{1600}
\expandafter\def\csname v@tune@CL-att@lo\endcsname{0}
\expandafter\def\csname v@tune@CL-att@li\endcsname{0}
\expandafter\def\csname v@tune@CL-att@kc\endcsname{0.25}
\expandafter\def\csname v@tune@CL-att@lam\endcsname{2}
\expandafter\def\csname v@tune@CL-att@mu\endcsname{0}
\expandafter\def\csname v@tune@CL-att@J\endcsname{46.2}
\expandafter\def\csname v@tune@CL-att@n\endcsname{132}
\expandafter\def\csname v@tune@PROPOSED@go\endcsname{2560}
\expandafter\def\csname v@tune@PROPOSED@gi\endcsname{25600}
\expandafter\def\csname v@tune@PROPOSED@lo\endcsname{0}
\expandafter\def\csname v@tune@PROPOSED@li\endcsname{0}
\expandafter\def\csname v@tune@PROPOSED@kc\endcsname{0.25}
\expandafter\def\csname v@tune@PROPOSED@lam\endcsname{2}
\expandafter\def\csname v@tune@PROPOSED@mu\endcsname{0}
\expandafter\def\csname v@tune@PROPOSED@J\endcsname{35.8}
\expandafter\def\csname v@tune@PROPOSED@n\endcsname{132}
\expandafter\def\csname v@tune@all@budget\endcsname{13.03}
\expandafter\def\csname v@tune@all@lqrdw\endcsname{12.41}
\expandafter\def\csname v@avg@LQR@des\endcsname{340.0}
\expandafter\def\csname v@avg@LQR@val\endcsname{536.6}
\expandafter\def\csname v@avg@LQR@valall\endcsname{482.9}
\expandafter\def\csname v@avg@MRAC@des\endcsname{86.5}
\expandafter\def\csname v@avg@MRAC@val\endcsname{109.2}
\expandafter\def\csname v@avg@MRAC@valall\endcsname{83.8}
\expandafter\def\csname v@avg@B1@des\endcsname{12346.7}
\expandafter\def\csname v@avg@B1@val\endcsname{div.}
\expandafter\def\csname v@avg@B1@valall\endcsname{div.}
\expandafter\def\csname v@avg@NN-MRAC@des\endcsname{82.6}
\expandafter\def\csname v@avg@NN-MRAC@val\endcsname{104.9}
\expandafter\def\csname v@avg@NN-MRAC@valall\endcsname{84.5}
\expandafter\def\csname v@avg@CL-ucmd@des\endcsname{77.8}
\expandafter\def\csname v@avg@CL-ucmd@val\endcsname{104.3}
\expandafter\def\csname v@avg@CL-ucmd@valall\endcsname{82.1}
\expandafter\def\csname v@avg@CL-att@des\endcsname{46.2}
\expandafter\def\csname v@avg@CL-att@val\endcsname{57.9}
\expandafter\def\csname v@avg@CL-att@valall\endcsname{57.0}
\expandafter\def\csname v@avg@PROPOSED@des\endcsname{35.8}
\expandafter\def\csname v@avg@PROPOSED@val\endcsname{45.1}
\expandafter\def\csname v@avg@PROPOSED@valall\endcsname{45.1}
\expandafter\def\csname v@S8910@LQR@IMPmin\endcsname{89}
\expandafter\def\csname v@S8910@LQR@IMPmax\endcsname{95}
\expandafter\def\csname v@S8910@MRAC@IMPmin\endcsname{25}
\expandafter\def\csname v@S8910@MRAC@IMPmax\endcsname{76}
\expandafter\def\csname v@S8910@B1@IMPmin\endcsname{100}
\expandafter\def\csname v@S8910@B1@IMPmax\endcsname{100}
\expandafter\def\csname v@S8910@NN-MRAC@IMPmin\endcsname{45}
\expandafter\def\csname v@S8910@NN-MRAC@IMPmax\endcsname{72}
\expandafter\def\csname v@S8910@CL-ucmd@IMPmin\endcsname{48}
\expandafter\def\csname v@S8910@CL-ucmd@IMPmax\endcsname{65}
\expandafter\def\csname v@S8910@CL-att@IMPmin\endcsname{16}
\expandafter\def\csname v@S8910@CL-att@IMPmax\endcsname{26}
\expandafter\def\csname v@MCS2@LQR@med\endcsname{330.2}
\expandafter\def\csname v@MCS2@LQR@mean\endcsname{343.1}
\expandafter\def\csname v@MCS2@LQR@std\endcsname{99.4}
\expandafter\def\csname v@MCS2@LQR@max\endcsname{435.9}
\expandafter\def\csname v@MCS2@LQR@dw\endcsname{12.21}
\expandafter\def\csname v@MCS2@LQR@fail\endcsname{0}
\expandafter\def\csname v@MCS2@LQR@wins\endcsname{50}
\expandafter\def\csname v@MCS2@LQR@p\endcsname{<\!10^{-3}}
\expandafter\def\csname v@MCS2@LQR@r\endcsname{1.00}
\expandafter\def\csname v@MCS2@MRAC@med\endcsname{91.8}
\expandafter\def\csname v@MCS2@MRAC@mean\endcsname{93.0}
\expandafter\def\csname v@MCS2@MRAC@std\endcsname{19.4}
\expandafter\def\csname v@MCS2@MRAC@max\endcsname{255.5}
\expandafter\def\csname v@MCS2@MRAC@dw\endcsname{21.56}
\expandafter\def\csname v@MCS2@MRAC@fail\endcsname{0}
\expandafter\def\csname v@MCS2@MRAC@wins\endcsname{50}
\expandafter\def\csname v@MCS2@MRAC@p\endcsname{<\!10^{-3}}
\expandafter\def\csname v@MCS2@MRAC@r\endcsname{1.00}
\expandafter\def\csname v@MCS2@B1@med\endcsname{400.5}
\expandafter\def\csname v@MCS2@B1@mean\endcsname{345.2}
\expandafter\def\csname v@MCS2@B1@std\endcsname{267.8}
\expandafter\def\csname v@MCS2@B1@max\endcsname{1299.5}
\expandafter\def\csname v@MCS2@B1@dw\endcsname{21.80}
\expandafter\def\csname v@MCS2@B1@fail\endcsname{43}
\expandafter\def\csname v@MCS2@B1@wins\endcsname{7}
\expandafter\def\csname v@MCS2@B1@p\endcsname{=0.016}
\expandafter\def\csname v@MCS2@B1@r\endcsname{1.00}
\expandafter\def\csname v@MCS2@NN-MRAC@med\endcsname{67.4}
\expandafter\def\csname v@MCS2@NN-MRAC@mean\endcsname{68.6}
\expandafter\def\csname v@MCS2@NN-MRAC@std\endcsname{10.4}
\expandafter\def\csname v@MCS2@NN-MRAC@max\endcsname{158.1}
\expandafter\def\csname v@MCS2@NN-MRAC@dw\endcsname{13.72}
\expandafter\def\csname v@MCS2@NN-MRAC@fail\endcsname{0}
\expandafter\def\csname v@MCS2@NN-MRAC@wins\endcsname{50}
\expandafter\def\csname v@MCS2@NN-MRAC@p\endcsname{<\!10^{-3}}
\expandafter\def\csname v@MCS2@NN-MRAC@r\endcsname{1.00}
\expandafter\def\csname v@MCS2@CL-ucmd@med\endcsname{76.0}
\expandafter\def\csname v@MCS2@CL-ucmd@mean\endcsname{75.6}
\expandafter\def\csname v@MCS2@CL-ucmd@std\endcsname{2.5}
\expandafter\def\csname v@MCS2@CL-ucmd@max\endcsname{141.6}
\expandafter\def\csname v@MCS2@CL-ucmd@dw\endcsname{16.76}
\expandafter\def\csname v@MCS2@CL-ucmd@fail\endcsname{0}
\expandafter\def\csname v@MCS2@CL-ucmd@wins\endcsname{50}
\expandafter\def\csname v@MCS2@CL-ucmd@p\endcsname{<\!10^{-3}}
\expandafter\def\csname v@MCS2@CL-ucmd@r\endcsname{1.00}
\expandafter\def\csname v@MCS2@CL-att@med\endcsname{45.7}
\expandafter\def\csname v@MCS2@CL-att@mean\endcsname{47.1}
\expandafter\def\csname v@MCS2@CL-att@std\endcsname{4.9}
\expandafter\def\csname v@MCS2@CL-att@max\endcsname{125.3}
\expandafter\def\csname v@MCS2@CL-att@dw\endcsname{16.70}
\expandafter\def\csname v@MCS2@CL-att@fail\endcsname{0}
\expandafter\def\csname v@MCS2@CL-att@wins\endcsname{50}
\expandafter\def\csname v@MCS2@CL-att@p\endcsname{<\!10^{-3}}
\expandafter\def\csname v@MCS2@CL-att@r\endcsname{1.00}
\expandafter\def\csname v@MCS2@PROPOSED@med\endcsname{29.4}
\expandafter\def\csname v@MCS2@PROPOSED@mean\endcsname{29.8}
\expandafter\def\csname v@MCS2@PROPOSED@std\endcsname{2.1}
\expandafter\def\csname v@MCS2@PROPOSED@max\endcsname{74.6}
\expandafter\def\csname v@MCS2@PROPOSED@dw\endcsname{19.49}
\expandafter\def\csname v@MCS2@PROPOSED@fail\endcsname{0}
\expandafter\def\csname v@MCS2@PROPOSED@wins\endcsname{--}
\expandafter\def\csname v@MCS2@PROPOSED@p\endcsname{--}
\expandafter\def\csname v@MCS2@PROPOSED@r\endcsname{--}
\expandafter\def\csname v@MCS4@LQR@med\endcsname{404.1}
\expandafter\def\csname v@MCS4@LQR@mean\endcsname{396.3}
\expandafter\def\csname v@MCS4@LQR@std\endcsname{104.5}
\expandafter\def\csname v@MCS4@LQR@max\endcsname{617.8}
\expandafter\def\csname v@MCS4@LQR@dw\endcsname{12.26}
\expandafter\def\csname v@MCS4@LQR@fail\endcsname{0}
\expandafter\def\csname v@MCS4@LQR@wins\endcsname{50}
\expandafter\def\csname v@MCS4@LQR@p\endcsname{<\!10^{-3}}
\expandafter\def\csname v@MCS4@LQR@r\endcsname{1.00}
\expandafter\def\csname v@MCS4@MRAC@med\endcsname{111.9}
\expandafter\def\csname v@MCS4@MRAC@mean\endcsname{116.6}
\expandafter\def\csname v@MCS4@MRAC@std\endcsname{27.9}
\expandafter\def\csname v@MCS4@MRAC@max\endcsname{323.0}
\expandafter\def\csname v@MCS4@MRAC@dw\endcsname{25.27}
\expandafter\def\csname v@MCS4@MRAC@fail\endcsname{2}
\expandafter\def\csname v@MCS4@MRAC@wins\endcsname{44}
\expandafter\def\csname v@MCS4@MRAC@p\endcsname{<\!10^{-3}}
\expandafter\def\csname v@MCS4@MRAC@r\endcsname{0.91}
\expandafter\def\csname v@MCS4@B1@med\endcsname{162.4}
\expandafter\def\csname v@MCS4@B1@mean\endcsname{214.3}
\expandafter\def\csname v@MCS4@B1@std\endcsname{114.7}
\expandafter\def\csname v@MCS4@B1@max\endcsname{974.5}
\expandafter\def\csname v@MCS4@B1@dw\endcsname{18.67}
\expandafter\def\csname v@MCS4@B1@fail\endcsname{40}
\expandafter\def\csname v@MCS4@B1@wins\endcsname{10}
\expandafter\def\csname v@MCS4@B1@p\endcsname{=0.002}
\expandafter\def\csname v@MCS4@B1@r\endcsname{1.00}
\expandafter\def\csname v@MCS4@NN-MRAC@med\endcsname{84.4}
\expandafter\def\csname v@MCS4@NN-MRAC@mean\endcsname{86.3}
\expandafter\def\csname v@MCS4@NN-MRAC@std\endcsname{10.9}
\expandafter\def\csname v@MCS4@NN-MRAC@max\endcsname{204.6}
\expandafter\def\csname v@MCS4@NN-MRAC@dw\endcsname{15.01}
\expandafter\def\csname v@MCS4@NN-MRAC@fail\endcsname{0}
\expandafter\def\csname v@MCS4@NN-MRAC@wins\endcsname{44}
\expandafter\def\csname v@MCS4@NN-MRAC@p\endcsname{<\!10^{-3}}
\expandafter\def\csname v@MCS4@NN-MRAC@r\endcsname{0.62}
\expandafter\def\csname v@MCS4@CL-ucmd@med\endcsname{98.1}
\expandafter\def\csname v@MCS4@CL-ucmd@mean\endcsname{100.3}
\expandafter\def\csname v@MCS4@CL-ucmd@std\endcsname{13.1}
\expandafter\def\csname v@MCS4@CL-ucmd@max\endcsname{200.8}
\expandafter\def\csname v@MCS4@CL-ucmd@dw\endcsname{19.63}
\expandafter\def\csname v@MCS4@CL-ucmd@fail\endcsname{0}
\expandafter\def\csname v@MCS4@CL-ucmd@wins\endcsname{44}
\expandafter\def\csname v@MCS4@CL-ucmd@p\endcsname{<\!10^{-3}}
\expandafter\def\csname v@MCS4@CL-ucmd@r\endcsname{0.77}
\expandafter\def\csname v@MCS4@CL-att@med\endcsname{53.7}
\expandafter\def\csname v@MCS4@CL-att@mean\endcsname{54.8}
\expandafter\def\csname v@MCS4@CL-att@std\endcsname{8.2}
\expandafter\def\csname v@MCS4@CL-att@max\endcsname{131.1}
\expandafter\def\csname v@MCS4@CL-att@dw\endcsname{20.00}
\expandafter\def\csname v@MCS4@CL-att@fail\endcsname{0}
\expandafter\def\csname v@MCS4@CL-att@wins\endcsname{40}
\expandafter\def\csname v@MCS4@CL-att@p\endcsname{=0.020}
\expandafter\def\csname v@MCS4@CL-att@r\endcsname{0.38}
\expandafter\def\csname v@MCS4@PROPOSED@med\endcsname{49.0}
\expandafter\def\csname v@MCS4@PROPOSED@mean\endcsname{62.4}
\expandafter\def\csname v@MCS4@PROPOSED@std\endcsname{45.8}
\expandafter\def\csname v@MCS4@PROPOSED@max\endcsname{208.0}
\expandafter\def\csname v@MCS4@PROPOSED@dw\endcsname{24.24}
\expandafter\def\csname v@MCS4@PROPOSED@fail\endcsname{0}
\expandafter\def\csname v@MCS4@PROPOSED@wins\endcsname{--}
\expandafter\def\csname v@MCS4@PROPOSED@p\endcsname{--}
\expandafter\def\csname v@MCS4@PROPOSED@r\endcsname{--}
\expandafter\def\csname v@MC@all@N\endcsname{50}
\expandafter\def\csname v@MCS2L@all@n\endcsname{23}
\expandafter\def\csname v@MCS2L@PROPOSED@med\endcsname{28.8}
\expandafter\def\csname v@MCS2L@CL-att@med\endcsname{45.5}
\expandafter\def\csname v@MCS2L@NN-MRAC@med\endcsname{70.7}
\expandafter\def\csname v@MCS2L@CL-att@wins\endcsname{23}
\expandafter\def\csname v@MCS2H@all@n\endcsname{27}
\expandafter\def\csname v@MCS2H@PROPOSED@med\endcsname{30.0}
\expandafter\def\csname v@MCS2H@CL-att@med\endcsname{46.3}
\expandafter\def\csname v@MCS2H@NN-MRAC@med\endcsname{66.1}
\expandafter\def\csname v@MCS2H@CL-att@wins\endcsname{27}
\expandafter\def\csname v@MCS4L@all@n\endcsname{23}
\expandafter\def\csname v@MCS4L@PROPOSED@med\endcsname{44.3}
\expandafter\def\csname v@MCS4L@CL-att@med\endcsname{53.2}
\expandafter\def\csname v@MCS4L@NN-MRAC@med\endcsname{88.2}
\expandafter\def\csname v@MCS4L@CL-att@wins\endcsname{23}
\expandafter\def\csname v@MCS4H@all@n\endcsname{27}
\expandafter\def\csname v@MCS4H@PROPOSED@med\endcsname{50.2}
\expandafter\def\csname v@MCS4H@CL-att@med\endcsname{56.1}
\expandafter\def\csname v@MCS4H@NN-MRAC@med\endcsname{82.3}
\expandafter\def\csname v@MCS4H@CL-att@wins\endcsname{17}
\expandafter\def\csname v@tmr@LQR@min\endcsname{338.7}
\expandafter\def\csname v@tmr@LQR@max\endcsname{339.1}
\expandafter\def\csname v@tmr@LQR@dw10\endcsname{1.40}
\expandafter\def\csname v@tmr@LQR@dw80\endcsname{1.42}
\expandafter\def\csname v@tmr@MRAC@min\endcsname{83.1}
\expandafter\def\csname v@tmr@MRAC@max\endcsname{97.2}
\expandafter\def\csname v@tmr@MRAC@dw10\endcsname{4.13}
\expandafter\def\csname v@tmr@MRAC@dw80\endcsname{5.53}
\expandafter\def\csname v@tmr@B1@min\endcsname{125.9}
\expandafter\def\csname v@tmr@B1@max\endcsname{368.1}
\expandafter\def\csname v@tmr@B1@dw10\endcsname{4.12}
\expandafter\def\csname v@tmr@B1@dw80\endcsname{8.65}
\expandafter\def\csname v@tmr@NN-MRAC@min\endcsname{75.1}
\expandafter\def\csname v@tmr@NN-MRAC@max\endcsname{79.5}
\expandafter\def\csname v@tmr@NN-MRAC@dw10\endcsname{2.16}
\expandafter\def\csname v@tmr@NN-MRAC@dw80\endcsname{3.22}
\expandafter\def\csname v@tmr@CL-ucmd@min\endcsname{95.6}
\expandafter\def\csname v@tmr@CL-ucmd@max\endcsname{98.6}
\expandafter\def\csname v@tmr@CL-ucmd@dw10\endcsname{2.42}
\expandafter\def\csname v@tmr@CL-ucmd@dw80\endcsname{4.84}
\expandafter\def\csname v@tmr@CL-att@min\endcsname{50.2}
\expandafter\def\csname v@tmr@CL-att@max\endcsname{58.3}
\expandafter\def\csname v@tmr@CL-att@dw10\endcsname{2.44}
\expandafter\def\csname v@tmr@CL-att@dw80\endcsname{4.89}
\expandafter\def\csname v@tmr@PROPOSED@min\endcsname{42.8}
\expandafter\def\csname v@tmr@PROPOSED@max\endcsname{49.0}
\expandafter\def\csname v@tmr@PROPOSED@dw10\endcsname{3.34}
\expandafter\def\csname v@tmr@PROPOSED@dw80\endcsname{4.04}
\expandafter\def\csname v@tm10@LQR@RMSE5\endcsname{339.1}
\expandafter\def\csname v@tm10@LQR@DW\endcsname{1.40}
\expandafter\def\csname v@tm10@MRAC@RMSE5\endcsname{97.2}
\expandafter\def\csname v@tm10@MRAC@DW\endcsname{4.13}
\expandafter\def\csname v@tm10@B1@RMSE5\endcsname{125.9}
\expandafter\def\csname v@tm10@B1@DW\endcsname{4.12}
\expandafter\def\csname v@tm10@NN-MRAC@RMSE5\endcsname{79.5}
\expandafter\def\csname v@tm10@NN-MRAC@DW\endcsname{2.16}
\expandafter\def\csname v@tm10@CL-ucmd@RMSE5\endcsname{95.9}
\expandafter\def\csname v@tm10@CL-ucmd@DW\endcsname{2.42}
\expandafter\def\csname v@tm10@CL-att@RMSE5\endcsname{50.2}
\expandafter\def\csname v@tm10@CL-att@DW\endcsname{2.44}
\expandafter\def\csname v@tm10@PROPOSED@RMSE5\endcsname{44.5}
\expandafter\def\csname v@tm10@PROPOSED@DW\endcsname{3.34}
\expandafter\def\csname v@tm20@LQR@RMSE5\endcsname{339.0}
\expandafter\def\csname v@tm20@LQR@DW\endcsname{1.40}
\expandafter\def\csname v@tm20@MRAC@RMSE5\endcsname{93.9}
\expandafter\def\csname v@tm20@MRAC@DW\endcsname{4.08}
\expandafter\def\csname v@tm20@B1@RMSE5\endcsname{136.4}
\expandafter\def\csname v@tm20@B1@DW\endcsname{4.16}
\expandafter\def\csname v@tm20@NN-MRAC@RMSE5\endcsname{78.6}
\expandafter\def\csname v@tm20@NN-MRAC@DW\endcsname{2.21}
\expandafter\def\csname v@tm20@CL-ucmd@RMSE5\endcsname{96.1}
\expandafter\def\csname v@tm20@CL-ucmd@DW\endcsname{2.51}
\expandafter\def\csname v@tm20@CL-att@RMSE5\endcsname{50.9}
\expandafter\def\csname v@tm20@CL-att@DW\endcsname{2.53}
\expandafter\def\csname v@tm20@PROPOSED@RMSE5\endcsname{44.0}
\expandafter\def\csname v@tm20@PROPOSED@DW\endcsname{3.40}
\expandafter\def\csname v@tm40@LQR@RMSE5\endcsname{338.8}
\expandafter\def\csname v@tm40@LQR@DW\endcsname{1.40}
\expandafter\def\csname v@tm40@MRAC@RMSE5\endcsname{85.9}
\expandafter\def\csname v@tm40@MRAC@DW\endcsname{4.30}
\expandafter\def\csname v@tm40@B1@RMSE5\endcsname{368.1}
\expandafter\def\csname v@tm40@B1@DW\endcsname{17.13}
\expandafter\def\csname v@tm40@NN-MRAC@RMSE5\endcsname{77.1}
\expandafter\def\csname v@tm40@NN-MRAC@DW\endcsname{2.43}
\expandafter\def\csname v@tm40@CL-ucmd@RMSE5\endcsname{95.9}
\expandafter\def\csname v@tm40@CL-ucmd@DW\endcsname{3.01}
\expandafter\def\csname v@tm40@CL-att@RMSE5\endcsname{53.9}
\expandafter\def\csname v@tm40@CL-att@DW\endcsname{3.34}
\expandafter\def\csname v@tm40@PROPOSED@RMSE5\endcsname{42.8}
\expandafter\def\csname v@tm40@PROPOSED@DW\endcsname{3.55}
\expandafter\def\csname v@tm60@LQR@RMSE5\endcsname{338.7}
\expandafter\def\csname v@tm60@LQR@DW\endcsname{1.40}
\expandafter\def\csname v@tm60@MRAC@RMSE5\endcsname{83.1}
\expandafter\def\csname v@tm60@MRAC@DW\endcsname{4.80}
\expandafter\def\csname v@tm60@B1@RMSE5\endcsname{div.}
\expandafter\def\csname v@tm60@B1@DW\endcsname{5.69}
\expandafter\def\csname v@tm60@NN-MRAC@RMSE5\endcsname{75.9}
\expandafter\def\csname v@tm60@NN-MRAC@DW\endcsname{2.84}
\expandafter\def\csname v@tm60@CL-ucmd@RMSE5\endcsname{95.6}
\expandafter\def\csname v@tm60@CL-ucmd@DW\endcsname{4.30}
\expandafter\def\csname v@tm60@CL-att@RMSE5\endcsname{55.8}
\expandafter\def\csname v@tm60@CL-att@DW\endcsname{4.15}
\expandafter\def\csname v@tm60@PROPOSED@RMSE5\endcsname{45.3}
\expandafter\def\csname v@tm60@PROPOSED@DW\endcsname{3.69}
\expandafter\def\csname v@tm80@LQR@RMSE5\endcsname{338.9}
\expandafter\def\csname v@tm80@LQR@DW\endcsname{1.42}
\expandafter\def\csname v@tm80@MRAC@RMSE5\endcsname{84.9}
\expandafter\def\csname v@tm80@MRAC@DW\endcsname{5.53}
\expandafter\def\csname v@tm80@B1@RMSE5\endcsname{div.}
\expandafter\def\csname v@tm80@B1@DW\endcsname{8.65}
\expandafter\def\csname v@tm80@NN-MRAC@RMSE5\endcsname{75.1}
\expandafter\def\csname v@tm80@NN-MRAC@DW\endcsname{3.22}
\expandafter\def\csname v@tm80@CL-ucmd@RMSE5\endcsname{98.6}
\expandafter\def\csname v@tm80@CL-ucmd@DW\endcsname{4.84}
\expandafter\def\csname v@tm80@CL-att@RMSE5\endcsname{58.3}
\expandafter\def\csname v@tm80@CL-att@DW\endcsname{4.89}
\expandafter\def\csname v@tm80@PROPOSED@RMSE5\endcsname{49.0}
\expandafter\def\csname v@tm80@PROPOSED@DW\endcsname{4.04}
\expandafter\def\csname v@MCS2@LQR@nbig\endcsname{0}
\expandafter\def\csname v@MCS2@LQR@xmax\endcsname{601.5}
\expandafter\def\csname v@MCS2@LQR@nok\endcsname{50}
\expandafter\def\csname v@MCS2@LQR@meanok\endcsname{343.1}
\expandafter\def\csname v@MCS2@LQR@stdok\endcsname{99.4}
\expandafter\def\csname v@MCS4@LQR@nbig\endcsname{0}
\expandafter\def\csname v@MCS4@LQR@xmax\endcsname{602.8}
\expandafter\def\csname v@MCS4@LQR@nok\endcsname{50}
\expandafter\def\csname v@MCS4@LQR@meanok\endcsname{396.3}
\expandafter\def\csname v@MCS4@LQR@stdok\endcsname{104.5}
\expandafter\def\csname v@MCS2@MRAC@nbig\endcsname{0}
\expandafter\def\csname v@MCS2@MRAC@xmax\endcsname{134.4}
\expandafter\def\csname v@MCS2@MRAC@nok\endcsname{50}
\expandafter\def\csname v@MCS2@MRAC@meanok\endcsname{93.0}
\expandafter\def\csname v@MCS2@MRAC@stdok\endcsname{19.4}
\expandafter\def\csname v@MCS4@MRAC@nbig\endcsname{0}
\expandafter\def\csname v@MCS4@MRAC@xmax\endcsname{248.1}
\expandafter\def\csname v@MCS4@MRAC@nok\endcsname{48}
\expandafter\def\csname v@MCS4@MRAC@meanok\endcsname{116.6}
\expandafter\def\csname v@MCS4@MRAC@stdok\endcsname{27.9}
\expandafter\def\csname v@MCS2@B1@nbig\endcsname{0}
\expandafter\def\csname v@MCS2@B1@xmax\endcsname{838.4}
\expandafter\def\csname v@MCS2@B1@nok\endcsname{7}
\expandafter\def\csname v@MCS2@B1@meanok\endcsname{345.2}
\expandafter\def\csname v@MCS2@B1@stdok\endcsname{267.8}
\expandafter\def\csname v@MCS4@B1@nbig\endcsname{0}
\expandafter\def\csname v@MCS4@B1@xmax\endcsname{406.3}
\expandafter\def\csname v@MCS4@B1@nok\endcsname{10}
\expandafter\def\csname v@MCS4@B1@meanok\endcsname{214.3}
\expandafter\def\csname v@MCS4@B1@stdok\endcsname{114.7}
\expandafter\def\csname v@MCS2@NN-MRAC@nbig\endcsname{0}
\expandafter\def\csname v@MCS2@NN-MRAC@xmax\endcsname{95.5}
\expandafter\def\csname v@MCS2@NN-MRAC@nok\endcsname{50}
\expandafter\def\csname v@MCS2@NN-MRAC@meanok\endcsname{68.6}
\expandafter\def\csname v@MCS2@NN-MRAC@stdok\endcsname{10.4}
\expandafter\def\csname v@MCS4@NN-MRAC@nbig\endcsname{0}
\expandafter\def\csname v@MCS4@NN-MRAC@xmax\endcsname{121.5}
\expandafter\def\csname v@MCS4@NN-MRAC@nok\endcsname{50}
\expandafter\def\csname v@MCS4@NN-MRAC@meanok\endcsname{86.3}
\expandafter\def\csname v@MCS4@NN-MRAC@stdok\endcsname{10.9}
\expandafter\def\csname v@MCS2@CL-ucmd@nbig\endcsname{0}
\expandafter\def\csname v@MCS2@CL-ucmd@xmax\endcsname{79.5}
\expandafter\def\csname v@MCS2@CL-ucmd@nok\endcsname{50}
\expandafter\def\csname v@MCS2@CL-ucmd@meanok\endcsname{75.6}
\expandafter\def\csname v@MCS2@CL-ucmd@stdok\endcsname{2.5}
\expandafter\def\csname v@MCS4@CL-ucmd@nbig\endcsname{0}
\expandafter\def\csname v@MCS4@CL-ucmd@xmax\endcsname{128.7}
\expandafter\def\csname v@MCS4@CL-ucmd@nok\endcsname{50}
\expandafter\def\csname v@MCS4@CL-ucmd@meanok\endcsname{100.3}
\expandafter\def\csname v@MCS4@CL-ucmd@stdok\endcsname{13.1}
\expandafter\def\csname v@MCS2@CL-att@nbig\endcsname{0}
\expandafter\def\csname v@MCS2@CL-att@xmax\endcsname{58.5}
\expandafter\def\csname v@MCS2@CL-att@nok\endcsname{50}
\expandafter\def\csname v@MCS2@CL-att@meanok\endcsname{47.1}
\expandafter\def\csname v@MCS2@CL-att@stdok\endcsname{4.9}
\expandafter\def\csname v@MCS4@CL-att@nbig\endcsname{0}
\expandafter\def\csname v@MCS4@CL-att@xmax\endcsname{70.4}
\expandafter\def\csname v@MCS4@CL-att@nok\endcsname{50}
\expandafter\def\csname v@MCS4@CL-att@meanok\endcsname{54.8}
\expandafter\def\csname v@MCS4@CL-att@stdok\endcsname{8.2}
\expandafter\def\csname v@MCS2@PROPOSED@nbig\endcsname{0}
\expandafter\def\csname v@MCS2@PROPOSED@xmax\endcsname{34.4}
\expandafter\def\csname v@MCS2@PROPOSED@nok\endcsname{50}
\expandafter\def\csname v@MCS2@PROPOSED@meanok\endcsname{29.8}
\expandafter\def\csname v@MCS2@PROPOSED@stdok\endcsname{2.1}
\expandafter\def\csname v@MCS4@PROPOSED@nbig\endcsname{0}
\expandafter\def\csname v@MCS4@PROPOSED@xmax\endcsname{270.9}
\expandafter\def\csname v@MCS4@PROPOSED@nok\endcsname{50}
\expandafter\def\csname v@MCS4@PROPOSED@meanok\endcsname{62.4}
\expandafter\def\csname v@MCS4@PROPOSED@stdok\endcsname{45.8}
\expandafter\def\csname v@dwr@NN@lo\endcsname{1.4}
\expandafter\def\csname v@dwr@NN@hi\endcsname{1.6}
\expandafter\def\csname v@gt5@CL-att@RMSE5\endcsname{87.1}
\expandafter\def\csname v@gt5@CL-att@DHATP\endcsname{0.432}
\expandafter\def\csname v@gt5@CL-att@DW\endcsname{12.45}
\expandafter\def\csname v@gt10@CL-att@RMSE5\endcsname{75.1}
\expandafter\def\csname v@gt10@CL-att@DHATP\endcsname{0.384}
\expandafter\def\csname v@gt10@CL-att@DW\endcsname{12.45}
\expandafter\def\csname v@gt20@CL-att@RMSE5\endcsname{66.1}
\expandafter\def\csname v@gt20@CL-att@DHATP\endcsname{0.362}
\expandafter\def\csname v@gt20@CL-att@DW\endcsname{12.44}
\expandafter\def\csname v@gt40@CL-att@RMSE5\endcsname{59.8}
\expandafter\def\csname v@gt40@CL-att@DHATP\endcsname{0.362}
\expandafter\def\csname v@gt40@CL-att@DW\endcsname{12.46}
\expandafter\def\csname v@gt80@CL-att@RMSE5\endcsname{55.0}
\expandafter\def\csname v@gt80@CL-att@DHATP\endcsname{0.380}
\expandafter\def\csname v@gt80@CL-att@DW\endcsname{12.57}
\expandafter\def\csname v@gt160@CL-att@RMSE5\endcsname{50.9}
\expandafter\def\csname v@gt160@CL-att@DHATP\endcsname{0.416}
\expandafter\def\csname v@gt160@CL-att@DW\endcsname{12.93}
\expandafter\def\csname v@gt320@CL-att@RMSE5\endcsname{47.6}
\expandafter\def\csname v@gt320@CL-att@DHATP\endcsname{0.469}
\expandafter\def\csname v@gt320@CL-att@DW\endcsname{13.75}
\expandafter\def\csname v@gt640@CL-att@RMSE5\endcsname{45.1}
\expandafter\def\csname v@gt640@CL-att@DHATP\endcsname{0.542}
\expandafter\def\csname v@gt640@CL-att@DW\endcsname{15.21}
\expandafter\def\csname v@gt1280@CL-att@RMSE5\endcsname{43.3}
\expandafter\def\csname v@gt1280@CL-att@DHATP\endcsname{0.634}
\expandafter\def\csname v@gt1280@CL-att@DW\endcsname{15.95}
\expandafter\def\csname v@gt2560@CL-att@RMSE5\endcsname{41.6}
\expandafter\def\csname v@gt2560@CL-att@DHATP\endcsname{0.735}
\expandafter\def\csname v@gt2560@CL-att@DW\endcsname{16.99}
\expandafter\def\csname v@gt5120@CL-att@RMSE5\endcsname{40.3}
\expandafter\def\csname v@gt5120@CL-att@DHATP\endcsname{0.853}
\expandafter\def\csname v@gt5120@CL-att@DW\endcsname{18.38}
\expandafter\def\csname v@gt5@PROPOSED@RMSE5\endcsname{85.7}
\expandafter\def\csname v@gt5@PROPOSED@DHATP\endcsname{0.429}
\expandafter\def\csname v@gt5@PROPOSED@DW\endcsname{12.41}
\expandafter\def\csname v@gt10@PROPOSED@RMSE5\endcsname{73.5}
\expandafter\def\csname v@gt10@PROPOSED@DHATP\endcsname{0.379}
\expandafter\def\csname v@gt10@PROPOSED@DW\endcsname{12.41}
\expandafter\def\csname v@gt20@PROPOSED@RMSE5\endcsname{64.5}
\expandafter\def\csname v@gt20@PROPOSED@DHATP\endcsname{0.354}
\expandafter\def\csname v@gt20@PROPOSED@DW\endcsname{12.41}
\expandafter\def\csname v@gt40@PROPOSED@RMSE5\endcsname{58.2}
\expandafter\def\csname v@gt40@PROPOSED@DHATP\endcsname{0.353}
\expandafter\def\csname v@gt40@PROPOSED@DW\endcsname{12.41}
\expandafter\def\csname v@gt80@PROPOSED@RMSE5\endcsname{53.3}
\expandafter\def\csname v@gt80@PROPOSED@DHATP\endcsname{0.372}
\expandafter\def\csname v@gt80@PROPOSED@DW\endcsname{12.44}
\expandafter\def\csname v@gt160@PROPOSED@RMSE5\endcsname{49.4}
\expandafter\def\csname v@gt160@PROPOSED@DHATP\endcsname{0.417}
\expandafter\def\csname v@gt160@PROPOSED@DW\endcsname{12.51}
\expandafter\def\csname v@gt320@PROPOSED@RMSE5\endcsname{47.1}
\expandafter\def\csname v@gt320@PROPOSED@DHATP\endcsname{0.495}
\expandafter\def\csname v@gt320@PROPOSED@DW\endcsname{12.59}
\expandafter\def\csname v@gt640@PROPOSED@RMSE5\endcsname{45.7}
\expandafter\def\csname v@gt640@PROPOSED@DHATP\endcsname{0.609}
\expandafter\def\csname v@gt640@PROPOSED@DW\endcsname{12.67}
\expandafter\def\csname v@gt1280@PROPOSED@RMSE5\endcsname{45.2}
\expandafter\def\csname v@gt1280@PROPOSED@DHATP\endcsname{0.735}
\expandafter\def\csname v@gt1280@PROPOSED@DW\endcsname{12.76}
\expandafter\def\csname v@gt2560@PROPOSED@RMSE5\endcsname{44.0}
\expandafter\def\csname v@gt2560@PROPOSED@DHATP\endcsname{0.852}
\expandafter\def\csname v@gt2560@PROPOSED@DW\endcsname{12.98}
\expandafter\def\csname v@gt5120@PROPOSED@RMSE5\endcsname{43.6}
\expandafter\def\csname v@gt5120@PROPOSED@DHATP\endcsname{1.059}
\expandafter\def\csname v@gt5120@PROPOSED@DW\endcsname{13.47}
\expandafter\def\csname v@pb100@MRAC@J\endcsname{--}
\expandafter\def\csname v@pb100@MRAC@go\endcsname{--}
\expandafter\def\csname v@pb100@NN-MRAC@J\endcsname{--}
\expandafter\def\csname v@pb100@NN-MRAC@go\endcsname{--}
\expandafter\def\csname v@pb100@CL-ucmd@J\endcsname{--}
\expandafter\def\csname v@pb100@CL-ucmd@go\endcsname{--}
\expandafter\def\csname v@pb100@CL-att@J\endcsname{--}
\expandafter\def\csname v@pb100@CL-att@go\endcsname{--}
\expandafter\def\csname v@pb100@PROPOSED@J\endcsname{49.7}
\expandafter\def\csname v@pb100@PROPOSED@go\endcsname{5120}
\expandafter\def\csname v@pb105@MRAC@J\endcsname{86.5}
\expandafter\def\csname v@pb105@MRAC@go\endcsname{40}
\expandafter\def\csname v@pb105@NN-MRAC@J\endcsname{82.6}
\expandafter\def\csname v@pb105@NN-MRAC@go\endcsname{40}
\expandafter\def\csname v@pb105@CL-ucmd@J\endcsname{77.8}
\expandafter\def\csname v@pb105@CL-ucmd@go\endcsname{20}
\expandafter\def\csname v@pb105@CL-att@J\endcsname{46.2}
\expandafter\def\csname v@pb105@CL-att@go\endcsname{160}
\expandafter\def\csname v@pb105@PROPOSED@J\endcsname{35.8}
\expandafter\def\csname v@pb105@PROPOSED@go\endcsname{2560}
\expandafter\def\csname v@pb110@MRAC@J\endcsname{86.5}
\expandafter\def\csname v@pb110@MRAC@go\endcsname{40}
\expandafter\def\csname v@pb110@NN-MRAC@J\endcsname{82.6}
\expandafter\def\csname v@pb110@NN-MRAC@go\endcsname{40}
\expandafter\def\csname v@pb110@CL-ucmd@J\endcsname{77.8}
\expandafter\def\csname v@pb110@CL-ucmd@go\endcsname{20}
\expandafter\def\csname v@pb110@CL-att@J\endcsname{44.4}
\expandafter\def\csname v@pb110@CL-att@go\endcsname{160}
\expandafter\def\csname v@pb110@PROPOSED@J\endcsname{35.8}
\expandafter\def\csname v@pb110@PROPOSED@go\endcsname{2560}
\expandafter\def\csname v@pb115@MRAC@J\endcsname{86.5}
\expandafter\def\csname v@pb115@MRAC@go\endcsname{40}
\expandafter\def\csname v@pb115@NN-MRAC@J\endcsname{82.6}
\expandafter\def\csname v@pb115@NN-MRAC@go\endcsname{40}
\expandafter\def\csname v@pb115@CL-ucmd@J\endcsname{77.8}
\expandafter\def\csname v@pb115@CL-ucmd@go\endcsname{20}
\expandafter\def\csname v@pb115@CL-att@J\endcsname{41.1}
\expandafter\def\csname v@pb115@CL-att@go\endcsname{320}
\expandafter\def\csname v@pb115@PROPOSED@J\endcsname{35.8}
\expandafter\def\csname v@pb115@PROPOSED@go\endcsname{2560}
\expandafter\def\csname v@pb120@MRAC@J\endcsname{86.5}
\expandafter\def\csname v@pb120@MRAC@go\endcsname{40}
\expandafter\def\csname v@pb120@NN-MRAC@J\endcsname{82.6}
\expandafter\def\csname v@pb120@NN-MRAC@go\endcsname{40}
\expandafter\def\csname v@pb120@CL-ucmd@J\endcsname{77.8}
\expandafter\def\csname v@pb120@CL-ucmd@go\endcsname{20}
\expandafter\def\csname v@pb120@CL-att@J\endcsname{41.1}
\expandafter\def\csname v@pb120@CL-att@go\endcsname{320}
\expandafter\def\csname v@pb120@PROPOSED@J\endcsname{35.8}
\expandafter\def\csname v@pb120@PROPOSED@go\endcsname{2560}
\expandafter\def\csname v@pb125@MRAC@J\endcsname{86.5}
\expandafter\def\csname v@pb125@MRAC@go\endcsname{40}
\expandafter\def\csname v@pb125@NN-MRAC@J\endcsname{82.6}
\expandafter\def\csname v@pb125@NN-MRAC@go\endcsname{40}
\expandafter\def\csname v@pb125@CL-ucmd@J\endcsname{77.8}
\expandafter\def\csname v@pb125@CL-ucmd@go\endcsname{20}
\expandafter\def\csname v@pb125@CL-att@J\endcsname{39.9}
\expandafter\def\csname v@pb125@CL-att@go\endcsname{640}
\expandafter\def\csname v@pb125@PROPOSED@J\endcsname{35.8}
\expandafter\def\csname v@pb125@PROPOSED@go\endcsname{2560}
\expandafter\def\csname v@pb130@MRAC@J\endcsname{86.5}
\expandafter\def\csname v@pb130@MRAC@go\endcsname{40}
\expandafter\def\csname v@pb130@NN-MRAC@J\endcsname{82.6}
\expandafter\def\csname v@pb130@NN-MRAC@go\endcsname{40}
\expandafter\def\csname v@pb130@CL-ucmd@J\endcsname{77.8}
\expandafter\def\csname v@pb130@CL-ucmd@go\endcsname{20}
\expandafter\def\csname v@pb130@CL-att@J\endcsname{37.3}
\expandafter\def\csname v@pb130@CL-att@go\endcsname{1280}
\expandafter\def\csname v@pb130@PROPOSED@J\endcsname{35.8}
\expandafter\def\csname v@pb130@PROPOSED@go\endcsname{2560}
\expandafter\def\csname v@pb135@MRAC@J\endcsname{86.5}
\expandafter\def\csname v@pb135@MRAC@go\endcsname{40}
\expandafter\def\csname v@pb135@NN-MRAC@J\endcsname{82.6}
\expandafter\def\csname v@pb135@NN-MRAC@go\endcsname{40}
\expandafter\def\csname v@pb135@CL-ucmd@J\endcsname{77.8}
\expandafter\def\csname v@pb135@CL-ucmd@go\endcsname{20}
\expandafter\def\csname v@pb135@CL-att@J\endcsname{37.3}
\expandafter\def\csname v@pb135@CL-att@go\endcsname{1280}
\expandafter\def\csname v@pb135@PROPOSED@J\endcsname{35.8}
\expandafter\def\csname v@pb135@PROPOSED@go\endcsname{2560}
\expandafter\def\csname v@pb140@MRAC@J\endcsname{86.5}
\expandafter\def\csname v@pb140@MRAC@go\endcsname{40}
\expandafter\def\csname v@pb140@NN-MRAC@J\endcsname{82.6}
\expandafter\def\csname v@pb140@NN-MRAC@go\endcsname{40}
\expandafter\def\csname v@pb140@CL-ucmd@J\endcsname{77.8}
\expandafter\def\csname v@pb140@CL-ucmd@go\endcsname{20}
\expandafter\def\csname v@pb140@CL-att@J\endcsname{35.5}
\expandafter\def\csname v@pb140@CL-att@go\endcsname{2560}
\expandafter\def\csname v@pb140@PROPOSED@J\endcsname{35.8}
\expandafter\def\csname v@pb140@PROPOSED@go\endcsname{2560}
\expandafter\def\csname v@pb145@MRAC@J\endcsname{86.5}
\expandafter\def\csname v@pb145@MRAC@go\endcsname{40}
\expandafter\def\csname v@pb145@NN-MRAC@J\endcsname{82.6}
\expandafter\def\csname v@pb145@NN-MRAC@go\endcsname{40}
\expandafter\def\csname v@pb145@CL-ucmd@J\endcsname{77.8}
\expandafter\def\csname v@pb145@CL-ucmd@go\endcsname{20}
\expandafter\def\csname v@pb145@CL-att@J\endcsname{35.5}
\expandafter\def\csname v@pb145@CL-att@go\endcsname{2560}
\expandafter\def\csname v@pb145@PROPOSED@J\endcsname{35.8}
\expandafter\def\csname v@pb145@PROPOSED@go\endcsname{2560}
\expandafter\def\csname v@pb150@MRAC@J\endcsname{86.5}
\expandafter\def\csname v@pb150@MRAC@go\endcsname{40}
\expandafter\def\csname v@pb150@NN-MRAC@J\endcsname{82.6}
\expandafter\def\csname v@pb150@NN-MRAC@go\endcsname{40}
\expandafter\def\csname v@pb150@CL-ucmd@J\endcsname{77.8}
\expandafter\def\csname v@pb150@CL-ucmd@go\endcsname{20}
\expandafter\def\csname v@pb150@CL-att@J\endcsname{34.2}
\expandafter\def\csname v@pb150@CL-att@go\endcsname{5120}
\expandafter\def\csname v@pb150@PROPOSED@J\endcsname{35.8}
\expandafter\def\csname v@pb150@PROPOSED@go\endcsname{2560}
\expandafter\def\csname v@pb100cfg@PROPOSED@go\endcsname{5120}
\expandafter\def\csname v@pb100cfg@PROPOSED@lo\endcsname{0}
\expandafter\def\csname v@pb100cfg@PROPOSED@kc\endcsname{1}
\expandafter\def\csname v@pb100cfg@PROPOSED@lam\endcsname{2}
\expandafter\def\csname v@pb100cfg@PROPOSED@act\endcsname{12.37}
\expandafter\def\csname v@pb100cfg@all@lqr\endcsname{12.41}
\expandafter\def\csname v@fa@tm20@lqr\endcsname{12.41}
\expandafter\def\csname v@fa20@lp0@J105\endcsname{46.2}
\expandafter\def\csname v@fa20@lp0@go105\endcsname{160}
\expandafter\def\csname v@fa20@lp0@J125\endcsname{39.9}
\expandafter\def\csname v@fa20@lp0@go125\endcsname{640}
\expandafter\def\csname v@fa20@lp0@J140\endcsname{35.5}
\expandafter\def\csname v@fa20@lp0@go140\endcsname{2560}
\expandafter\def\csname v@fa20@lp0@Jg\endcsname{35.5}
\expandafter\def\csname v@fa20@lp0@DWg\endcsname{16.99}
\expandafter\def\csname v@fa20@lp0@DW160\endcsname{12.93}
\expandafter\def\csname v@fa20@lp5@J105\endcsname{45.8}
\expandafter\def\csname v@fa20@lp5@go105\endcsname{160}
\expandafter\def\csname v@fa20@lp5@J125\endcsname{36.9}
\expandafter\def\csname v@fa20@lp5@go125\endcsname{1280}
\expandafter\def\csname v@fa20@lp5@J140\endcsname{34.7}
\expandafter\def\csname v@fa20@lp5@go140\endcsname{5120}
\expandafter\def\csname v@fa20@lp5@Jg\endcsname{35.3}
\expandafter\def\csname v@fa20@lp5@DWg\endcsname{16.17}
\expandafter\def\csname v@fa20@lp5@DW160\endcsname{12.87}
\expandafter\def\csname v@fa20@lp10@J105\endcsname{45.4}
\expandafter\def\csname v@fa20@lp10@go105\endcsname{160}
\expandafter\def\csname v@fa20@lp10@J125\endcsname{35.2}
\expandafter\def\csname v@fa20@lp10@go125\endcsname{2560}
\expandafter\def\csname v@fa20@lp10@J140\endcsname{34.8}
\expandafter\def\csname v@fa20@lp10@go140\endcsname{5120}
\expandafter\def\csname v@fa20@lp10@Jg\endcsname{35.2}
\expandafter\def\csname v@fa20@lp10@DWg\endcsname{14.97}
\expandafter\def\csname v@fa20@lp10@DW160\endcsname{12.78}
\expandafter\def\csname v@fa20@lp15@J105\endcsname{42.1}
\expandafter\def\csname v@fa20@lp15@go105\endcsname{320}
\expandafter\def\csname v@fa20@lp15@J125\endcsname{35.1}
\expandafter\def\csname v@fa20@lp15@go125\endcsname{5120}
\expandafter\def\csname v@fa20@lp15@J140\endcsname{35.1}
\expandafter\def\csname v@fa20@lp15@go140\endcsname{5120}
\expandafter\def\csname v@fa20@lp15@Jg\endcsname{35.3}
\expandafter\def\csname v@fa20@lp15@DWg\endcsname{13.87}
\expandafter\def\csname v@fa20@lp15@DW160\endcsname{12.66}
\expandafter\def\csname v@fa20@lp20@J105\endcsname{35.8}
\expandafter\def\csname v@fa20@lp20@go105\endcsname{2560}
\expandafter\def\csname v@fa20@lp20@J125\endcsname{35.8}
\expandafter\def\csname v@fa20@lp20@go125\endcsname{2560}
\expandafter\def\csname v@fa20@lp20@J140\endcsname{35.8}
\expandafter\def\csname v@fa20@lp20@go140\endcsname{2560}
\expandafter\def\csname v@fa20@lp20@Jg\endcsname{35.8}
\expandafter\def\csname v@fa20@lp20@DWg\endcsname{12.98}
\expandafter\def\csname v@fa20@lp20@DW160\endcsname{12.51}
\expandafter\def\csname v@fa20@lp25@J105\endcsname{36.3}
\expandafter\def\csname v@fa20@lp25@go105\endcsname{2560}
\expandafter\def\csname v@fa20@lp25@J125\endcsname{36.3}
\expandafter\def\csname v@fa20@lp25@go125\endcsname{2560}
\expandafter\def\csname v@fa20@lp25@J140\endcsname{36.3}
\expandafter\def\csname v@fa20@lp25@go140\endcsname{2560}
\expandafter\def\csname v@fa20@lp25@Jg\endcsname{36.3}
\expandafter\def\csname v@fa20@lp25@DWg\endcsname{12.28}
\expandafter\def\csname v@fa20@lp25@DW160\endcsname{12.35}
\expandafter\def\csname v@fa20@lp30@J105\endcsname{36.9}
\expandafter\def\csname v@fa20@lp30@go105\endcsname{2560}
\expandafter\def\csname v@fa20@lp30@J125\endcsname{36.9}
\expandafter\def\csname v@fa20@lp30@go125\endcsname{2560}
\expandafter\def\csname v@fa20@lp30@J140\endcsname{36.9}
\expandafter\def\csname v@fa20@lp30@go140\endcsname{2560}
\expandafter\def\csname v@fa20@lp30@Jg\endcsname{36.9}
\expandafter\def\csname v@fa20@lp30@DWg\endcsname{11.74}
\expandafter\def\csname v@fa20@lp30@DW160\endcsname{12.19}
\expandafter\def\csname v@fa20@lp40@J105\endcsname{39.6}
\expandafter\def\csname v@fa20@lp40@go105\endcsname{2560}
\expandafter\def\csname v@fa20@lp40@J125\endcsname{39.6}
\expandafter\def\csname v@fa20@lp40@go125\endcsname{2560}
\expandafter\def\csname v@fa20@lp40@J140\endcsname{39.6}
\expandafter\def\csname v@fa20@lp40@go140\endcsname{2560}
\expandafter\def\csname v@fa20@lp40@Jg\endcsname{39.6}
\expandafter\def\csname v@fa20@lp40@DWg\endcsname{10.95}
\expandafter\def\csname v@fa20@lp40@DW160\endcsname{11.89}
\expandafter\def\csname v@fa20@lp60@J105\endcsname{44.5}
\expandafter\def\csname v@fa20@lp60@go105\endcsname{640}
\expandafter\def\csname v@fa20@lp60@J125\endcsname{44.5}
\expandafter\def\csname v@fa20@lp60@go125\endcsname{640}
\expandafter\def\csname v@fa20@lp60@J140\endcsname{44.5}
\expandafter\def\csname v@fa20@lp60@go140\endcsname{640}
\expandafter\def\csname v@fa20@lp60@Jg\endcsname{112.1}
\expandafter\def\csname v@fa20@lp60@DWg\endcsname{10.20}
\expandafter\def\csname v@fa20@lp60@DW160\endcsname{11.36}
\expandafter\def\csname v@fa20@lp80@J105\endcsname{49.8}
\expandafter\def\csname v@fa20@lp80@go105\endcsname{80}
\expandafter\def\csname v@fa20@lp80@J125\endcsname{49.8}
\expandafter\def\csname v@fa20@lp80@go125\endcsname{80}
\expandafter\def\csname v@fa20@lp80@J140\endcsname{49.8}
\expandafter\def\csname v@fa20@lp80@go140\endcsname{80}
\expandafter\def\csname v@fa20@lp80@Jg\endcsname{374.6}
\expandafter\def\csname v@fa20@lp80@DWg\endcsname{9.80}
\expandafter\def\csname v@fa20@lp80@DW160\endcsname{10.90}
\expandafter\def\csname v@fa@tm60@lqr\endcsname{12.41}
\expandafter\def\csname v@fa60@lp0@J105\endcsname{64.4}
\expandafter\def\csname v@fa60@lp0@go105\endcsname{20}
\expandafter\def\csname v@fa60@lp0@J125\endcsname{52.5}
\expandafter\def\csname v@fa60@lp0@go125\endcsname{80}
\expandafter\def\csname v@fa60@lp0@J140\endcsname{52.5}
\expandafter\def\csname v@fa60@lp0@go140\endcsname{80}
\expandafter\def\csname v@fa60@lp0@Jg\endcsname{38.2}
\expandafter\def\csname v@fa60@lp0@DWg\endcsname{22.45}
\expandafter\def\csname v@fa60@lp0@DW160\endcsname{17.56}
\expandafter\def\csname v@fa60@lp5@J105\endcsname{63.7}
\expandafter\def\csname v@fa60@lp5@go105\endcsname{20}
\expandafter\def\csname v@fa60@lp5@J125\endcsname{51.6}
\expandafter\def\csname v@fa60@lp5@go125\endcsname{80}
\expandafter\def\csname v@fa60@lp5@J140\endcsname{48.4}
\expandafter\def\csname v@fa60@lp5@go140\endcsname{160}
\expandafter\def\csname v@fa60@lp5@Jg\endcsname{37.4}
\expandafter\def\csname v@fa60@lp5@DWg\endcsname{22.49}
\expandafter\def\csname v@fa60@lp5@DW160\endcsname{16.62}
\expandafter\def\csname v@fa60@lp10@J105\endcsname{63.0}
\expandafter\def\csname v@fa60@lp10@go105\endcsname{20}
\expandafter\def\csname v@fa60@lp10@J125\endcsname{50.7}
\expandafter\def\csname v@fa60@lp10@go125\endcsname{80}
\expandafter\def\csname v@fa60@lp10@J140\endcsname{44.3}
\expandafter\def\csname v@fa60@lp10@go140\endcsname{320}
\expandafter\def\csname v@fa60@lp10@Jg\endcsname{36.6}
\expandafter\def\csname v@fa60@lp10@DWg\endcsname{23.83}
\expandafter\def\csname v@fa60@lp10@DW160\endcsname{15.53}
\expandafter\def\csname v@fa60@lp15@J105\endcsname{62.5}
\expandafter\def\csname v@fa60@lp15@go105\endcsname{20}
\expandafter\def\csname v@fa60@lp15@J125\endcsname{46.6}
\expandafter\def\csname v@fa60@lp15@go125\endcsname{160}
\expandafter\def\csname v@fa60@lp15@J140\endcsname{43.6}
\expandafter\def\csname v@fa60@lp15@go140\endcsname{320}
\expandafter\def\csname v@fa60@lp15@Jg\endcsname{36.4}
\expandafter\def\csname v@fa60@lp15@DWg\endcsname{23.54}
\expandafter\def\csname v@fa60@lp15@DW160\endcsname{14.74}
\expandafter\def\csname v@fa60@lp20@J105\endcsname{62.1}
\expandafter\def\csname v@fa60@lp20@go105\endcsname{20}
\expandafter\def\csname v@fa60@lp20@J125\endcsname{42.9}
\expandafter\def\csname v@fa60@lp20@go125\endcsname{320}
\expandafter\def\csname v@fa60@lp20@J140\endcsname{40.0}
\expandafter\def\csname v@fa60@lp20@go140\endcsname{640}
\expandafter\def\csname v@fa60@lp20@Jg\endcsname{36.6}
\expandafter\def\csname v@fa60@lp20@DWg\endcsname{21.92}
\expandafter\def\csname v@fa60@lp20@DW160\endcsname{14.30}
\expandafter\def\csname v@fa60@lp25@J105\endcsname{54.0}
\expandafter\def\csname v@fa60@lp25@go105\endcsname{40}
\expandafter\def\csname v@fa60@lp25@J125\endcsname{42.6}
\expandafter\def\csname v@fa60@lp25@go125\endcsname{320}
\expandafter\def\csname v@fa60@lp25@J140\endcsname{39.8}
\expandafter\def\csname v@fa60@lp25@go140\endcsname{640}
\expandafter\def\csname v@fa60@lp25@Jg\endcsname{37.0}
\expandafter\def\csname v@fa60@lp25@DWg\endcsname{19.38}
\expandafter\def\csname v@fa60@lp25@DW160\endcsname{14.07}
\expandafter\def\csname v@fa60@lp30@J105\endcsname{53.7}
\expandafter\def\csname v@fa60@lp30@go105\endcsname{40}
\expandafter\def\csname v@fa60@lp30@J125\endcsname{42.4}
\expandafter\def\csname v@fa60@lp30@go125\endcsname{320}
\expandafter\def\csname v@fa60@lp30@J140\endcsname{37.2}
\expandafter\def\csname v@fa60@lp30@go140\endcsname{2560}
\expandafter\def\csname v@fa60@lp30@Jg\endcsname{37.2}
\expandafter\def\csname v@fa60@lp30@DWg\endcsname{17.35}
\expandafter\def\csname v@fa60@lp30@DW160\endcsname{13.88}
\expandafter\def\csname v@fa60@lp40@J105\endcsname{48.7}
\expandafter\def\csname v@fa60@lp40@go105\endcsname{80}
\expandafter\def\csname v@fa60@lp40@J125\endcsname{37.8}
\expandafter\def\csname v@fa60@lp40@go125\endcsname{2560}
\expandafter\def\csname v@fa60@lp40@J140\endcsname{37.6}
\expandafter\def\csname v@fa60@lp40@go140\endcsname{5120}
\expandafter\def\csname v@fa60@lp40@Jg\endcsname{37.8}
\expandafter\def\csname v@fa60@lp40@DWg\endcsname{15.36}
\expandafter\def\csname v@fa60@lp40@DW160\endcsname{13.48}
\expandafter\def\csname v@fa60@lp60@J105\endcsname{61.3}
\expandafter\def\csname v@fa60@lp60@go105\endcsname{20}
\expandafter\def\csname v@fa60@lp60@J125\endcsname{61.3}
\expandafter\def\csname v@fa60@lp60@go125\endcsname{20}
\expandafter\def\csname v@fa60@lp60@J140\endcsname{61.3}
\expandafter\def\csname v@fa60@lp60@go140\endcsname{20}
\expandafter\def\csname v@fa60@lp60@Jg\endcsname{Inf}
\expandafter\def\csname v@fa60@lp60@DWg\endcsname{12.89}
\expandafter\def\csname v@fa60@lp60@DW160\endcsname{12.47}
\expandafter\def\csname v@fa60@lp80@J105\endcsname{93.2}
\expandafter\def\csname v@fa60@lp80@go105\endcsname{5}
\expandafter\def\csname v@fa60@lp80@J125\endcsname{93.2}
\expandafter\def\csname v@fa60@lp80@go125\endcsname{5}
\expandafter\def\csname v@fa60@lp80@J140\endcsname{93.2}
\expandafter\def\csname v@fa60@lp80@go140\endcsname{5}
\expandafter\def\csname v@fa60@lp80@Jg\endcsname{Inf}
\expandafter\def\csname v@fa60@lp80@DWg\endcsname{11.45}
\expandafter\def\csname v@fa60@lp80@DW160\endcsname{11.49}
\expandafter\def\csname v@ts1S2@LQR@RMSE5\endcsname{230.9}
\expandafter\def\csname v@ts1S2@LQR@DW\endcsname{1.10}
\expandafter\def\csname v@ts1S2@LQR@TV\endcsname{168}
\expandafter\def\csname v@ts1S2@MRAC@RMSE5\endcsname{76.6}
\expandafter\def\csname v@ts1S2@MRAC@DW\endcsname{2.97}
\expandafter\def\csname v@ts1S2@MRAC@TV\endcsname{800}
\expandafter\def\csname v@ts1S2@B1@RMSE5\endcsname{85.6}
\expandafter\def\csname v@ts1S2@B1@DW\endcsname{2.31}
\expandafter\def\csname v@ts1S2@B1@TV\endcsname{1195}
\expandafter\def\csname v@ts1S2@NN-MRAC@RMSE5\endcsname{55.5}
\expandafter\def\csname v@ts1S2@NN-MRAC@DW\endcsname{1.45}
\expandafter\def\csname v@ts1S2@NN-MRAC@TV\endcsname{290}
\expandafter\def\csname v@ts1S2@CL-ucmd@RMSE5\endcsname{74.0}
\expandafter\def\csname v@ts1S2@CL-ucmd@DW\endcsname{1.66}
\expandafter\def\csname v@ts1S2@CL-ucmd@TV\endcsname{296}
\expandafter\def\csname v@ts1S2@CL-att@RMSE5\endcsname{41.5}
\expandafter\def\csname v@ts1S2@CL-att@DW\endcsname{1.13}
\expandafter\def\csname v@ts1S2@CL-att@TV\endcsname{201}
\expandafter\def\csname v@ts1S2@PROPOSED@RMSE5\endcsname{27.5}
\expandafter\def\csname v@ts1S2@PROPOSED@DW\endcsname{1.01}
\expandafter\def\csname v@ts1S2@PROPOSED@TV\endcsname{350}
\expandafter\def\csname v@ts1S4@LQR@RMSE5\endcsname{339.0}
\expandafter\def\csname v@ts1S4@LQR@DW\endcsname{1.40}
\expandafter\def\csname v@ts1S4@LQR@TV\endcsname{255}
\expandafter\def\csname v@ts1S4@MRAC@RMSE5\endcsname{93.9}
\expandafter\def\csname v@ts1S4@MRAC@DW\endcsname{4.08}
\expandafter\def\csname v@ts1S4@MRAC@TV\endcsname{1259}
\expandafter\def\csname v@ts1S4@B1@RMSE5\endcsname{136.4}
\expandafter\def\csname v@ts1S4@B1@DW\endcsname{4.16}
\expandafter\def\csname v@ts1S4@B1@TV\endcsname{1591}
\expandafter\def\csname v@ts1S4@NN-MRAC@RMSE5\endcsname{78.6}
\expandafter\def\csname v@ts1S4@NN-MRAC@DW\endcsname{2.21}
\expandafter\def\csname v@ts1S4@NN-MRAC@TV\endcsname{436}
\expandafter\def\csname v@ts1S4@CL-ucmd@RMSE5\endcsname{96.1}
\expandafter\def\csname v@ts1S4@CL-ucmd@DW\endcsname{2.51}
\expandafter\def\csname v@ts1S4@CL-ucmd@TV\endcsname{461}
\expandafter\def\csname v@ts1S4@CL-att@RMSE5\endcsname{50.9}
\expandafter\def\csname v@ts1S4@CL-att@DW\endcsname{2.53}
\expandafter\def\csname v@ts1S4@CL-att@TV\endcsname{451}
\expandafter\def\csname v@ts1S4@PROPOSED@RMSE5\endcsname{44.0}
\expandafter\def\csname v@ts1S4@PROPOSED@DW\endcsname{3.40}
\expandafter\def\csname v@ts1S4@PROPOSED@TV\endcsname{838}
\expandafter\def\csname v@ts2S2@LQR@RMSE5\endcsname{230.9}
\expandafter\def\csname v@ts2S2@LQR@DW\endcsname{1.57}
\expandafter\def\csname v@ts2S2@LQR@TV\endcsname{168}
\expandafter\def\csname v@ts2S2@MRAC@RMSE5\endcsname{76.3}
\expandafter\def\csname v@ts2S2@MRAC@DW\endcsname{4.25}
\expandafter\def\csname v@ts2S2@MRAC@TV\endcsname{804}
\expandafter\def\csname v@ts2S2@B1@RMSE5\endcsname{86.1}
\expandafter\def\csname v@ts2S2@B1@DW\endcsname{3.31}
\expandafter\def\csname v@ts2S2@B1@TV\endcsname{1172}
\expandafter\def\csname v@ts2S2@NN-MRAC@RMSE5\endcsname{55.4}
\expandafter\def\csname v@ts2S2@NN-MRAC@DW\endcsname{2.07}
\expandafter\def\csname v@ts2S2@NN-MRAC@TV\endcsname{291}
\expandafter\def\csname v@ts2S2@CL-ucmd@RMSE5\endcsname{73.8}
\expandafter\def\csname v@ts2S2@CL-ucmd@DW\endcsname{2.37}
\expandafter\def\csname v@ts2S2@CL-ucmd@TV\endcsname{297}
\expandafter\def\csname v@ts2S2@CL-att@RMSE5\endcsname{41.7}
\expandafter\def\csname v@ts2S2@CL-att@DW\endcsname{1.62}
\expandafter\def\csname v@ts2S2@CL-att@TV\endcsname{201}
\expandafter\def\csname v@ts2S2@PROPOSED@RMSE5\endcsname{27.6}
\expandafter\def\csname v@ts2S2@PROPOSED@DW\endcsname{1.45}
\expandafter\def\csname v@ts2S2@PROPOSED@TV\endcsname{353}
\expandafter\def\csname v@ts2S4@LQR@RMSE5\endcsname{339.0}
\expandafter\def\csname v@ts2S4@LQR@DW\endcsname{1.99}
\expandafter\def\csname v@ts2S4@LQR@TV\endcsname{256}
\expandafter\def\csname v@ts2S4@MRAC@RMSE5\endcsname{93.7}
\expandafter\def\csname v@ts2S4@MRAC@DW\endcsname{5.92}
\expandafter\def\csname v@ts2S4@MRAC@TV\endcsname{1273}
\expandafter\def\csname v@ts2S4@B1@RMSE5\endcsname{136.7}
\expandafter\def\csname v@ts2S4@B1@DW\endcsname{5.94}
\expandafter\def\csname v@ts2S4@B1@TV\endcsname{1564}
\expandafter\def\csname v@ts2S4@NN-MRAC@RMSE5\endcsname{78.5}
\expandafter\def\csname v@ts2S4@NN-MRAC@DW\endcsname{3.16}
\expandafter\def\csname v@ts2S4@NN-MRAC@TV\endcsname{437}
\expandafter\def\csname v@ts2S4@CL-ucmd@RMSE5\endcsname{96.0}
\expandafter\def\csname v@ts2S4@CL-ucmd@DW\endcsname{3.58}
\expandafter\def\csname v@ts2S4@CL-ucmd@TV\endcsname{462}
\expandafter\def\csname v@ts2S4@CL-att@RMSE5\endcsname{51.1}
\expandafter\def\csname v@ts2S4@CL-att@DW\endcsname{3.63}
\expandafter\def\csname v@ts2S4@CL-att@TV\endcsname{455}
\expandafter\def\csname v@ts2S4@PROPOSED@RMSE5\endcsname{44.3}
\expandafter\def\csname v@ts2S4@PROPOSED@DW\endcsname{4.98}
\expandafter\def\csname v@ts2S4@PROPOSED@TV\endcsname{860}
\expandafter\def\csname v@ts4S2@LQR@RMSE5\endcsname{231.0}
\expandafter\def\csname v@ts4S2@LQR@DW\endcsname{2.26}
\expandafter\def\csname v@ts4S2@LQR@TV\endcsname{169}
\expandafter\def\csname v@ts4S2@MRAC@RMSE5\endcsname{75.9}
\expandafter\def\csname v@ts4S2@MRAC@DW\endcsname{6.16}
\expandafter\def\csname v@ts4S2@MRAC@TV\endcsname{814}
\expandafter\def\csname v@ts4S2@B1@RMSE5\endcsname{91.7}
\expandafter\def\csname v@ts4S2@B1@DW\endcsname{5.20}
\expandafter\def\csname v@ts4S2@B1@TV\endcsname{1265}
\expandafter\def\csname v@ts4S2@NN-MRAC@RMSE5\endcsname{55.2}
\expandafter\def\csname v@ts4S2@NN-MRAC@DW\endcsname{2.98}
\expandafter\def\csname v@ts4S2@NN-MRAC@TV\endcsname{292}
\expandafter\def\csname v@ts4S2@CL-ucmd@RMSE5\endcsname{73.3}
\expandafter\def\csname v@ts4S2@CL-ucmd@DW\endcsname{3.40}
\expandafter\def\csname v@ts4S2@CL-ucmd@TV\endcsname{297}
\expandafter\def\csname v@ts4S2@CL-att@RMSE5\endcsname{42.4}
\expandafter\def\csname v@ts4S2@CL-att@DW\endcsname{2.32}
\expandafter\def\csname v@ts4S2@CL-att@TV\endcsname{202}
\expandafter\def\csname v@ts4S2@PROPOSED@RMSE5\endcsname{27.9}
\expandafter\def\csname v@ts4S2@PROPOSED@DW\endcsname{2.13}
\expandafter\def\csname v@ts4S2@PROPOSED@TV\endcsname{361}
\expandafter\def\csname v@ts4S4@LQR@RMSE5\endcsname{339.0}
\expandafter\def\csname v@ts4S4@LQR@DW\endcsname{2.87}
\expandafter\def\csname v@ts4S4@LQR@TV\endcsname{258}
\expandafter\def\csname v@ts4S4@MRAC@RMSE5\endcsname{93.4}
\expandafter\def\csname v@ts4S4@MRAC@DW\endcsname{8.71}
\expandafter\def\csname v@ts4S4@MRAC@TV\endcsname{1298}
\expandafter\def\csname v@ts4S4@B1@RMSE5\endcsname{174.6}
\expandafter\def\csname v@ts4S4@B1@DW\endcsname{10.30}
\expandafter\def\csname v@ts4S4@B1@TV\endcsname{2518}
\expandafter\def\csname v@ts4S4@NN-MRAC@RMSE5\endcsname{78.4}
\expandafter\def\csname v@ts4S4@NN-MRAC@DW\endcsname{4.57}
\expandafter\def\csname v@ts4S4@NN-MRAC@TV\endcsname{439}
\expandafter\def\csname v@ts4S4@CL-ucmd@RMSE5\endcsname{95.7}
\expandafter\def\csname v@ts4S4@CL-ucmd@DW\endcsname{5.15}
\expandafter\def\csname v@ts4S4@CL-ucmd@TV\endcsname{465}
\expandafter\def\csname v@ts4S4@CL-att@RMSE5\endcsname{51.5}
\expandafter\def\csname v@ts4S4@CL-att@DW\endcsname{5.17}
\expandafter\def\csname v@ts4S4@CL-att@TV\endcsname{461}
\expandafter\def\csname v@ts4S4@PROPOSED@RMSE5\endcsname{44.8}
\expandafter\def\csname v@ts4S4@PROPOSED@DW\endcsname{7.49}
\expandafter\def\csname v@ts4S4@PROPOSED@TV\endcsname{910}
\expandafter\def\csname v@tsmc1@MRAC@med\endcsname{111.9}
\expandafter\def\csname v@tsmc1@MRAC@fail\endcsname{2}
\expandafter\def\csname v@tsmc2@MRAC@med\endcsname{111.2}
\expandafter\def\csname v@tsmc2@MRAC@fail\endcsname{2}
\expandafter\def\csname v@tsmc2@MRAC@wins\endcsname{44}
\expandafter\def\csname v@tsmc4@MRAC@med\endcsname{110.9}
\expandafter\def\csname v@tsmc4@MRAC@fail\endcsname{1}
\expandafter\def\csname v@tsmc4@MRAC@wins\endcsname{45}
\expandafter\def\csname v@tsmc1@NN-MRAC@med\endcsname{84.4}
\expandafter\def\csname v@tsmc1@NN-MRAC@fail\endcsname{0}
\expandafter\def\csname v@tsmc2@NN-MRAC@med\endcsname{84.4}
\expandafter\def\csname v@tsmc2@NN-MRAC@fail\endcsname{0}
\expandafter\def\csname v@tsmc2@NN-MRAC@wins\endcsname{44}
\expandafter\def\csname v@tsmc4@NN-MRAC@med\endcsname{84.1}
\expandafter\def\csname v@tsmc4@NN-MRAC@fail\endcsname{0}
\expandafter\def\csname v@tsmc4@NN-MRAC@wins\endcsname{43}
\expandafter\def\csname v@tsmc1@CL-ucmd@med\endcsname{98.1}
\expandafter\def\csname v@tsmc1@CL-ucmd@fail\endcsname{0}
\expandafter\def\csname v@tsmc2@CL-ucmd@med\endcsname{98.1}
\expandafter\def\csname v@tsmc2@CL-ucmd@fail\endcsname{0}
\expandafter\def\csname v@tsmc2@CL-ucmd@wins\endcsname{44}
\expandafter\def\csname v@tsmc4@CL-ucmd@med\endcsname{98.1}
\expandafter\def\csname v@tsmc4@CL-ucmd@fail\endcsname{0}
\expandafter\def\csname v@tsmc4@CL-ucmd@wins\endcsname{43}
\expandafter\def\csname v@tsmc1@CL-att@med\endcsname{53.7}
\expandafter\def\csname v@tsmc1@CL-att@fail\endcsname{0}
\expandafter\def\csname v@tsmc2@CL-att@med\endcsname{53.9}
\expandafter\def\csname v@tsmc2@CL-att@fail\endcsname{0}
\expandafter\def\csname v@tsmc2@CL-att@wins\endcsname{39}
\expandafter\def\csname v@tsmc4@CL-att@med\endcsname{54.2}
\expandafter\def\csname v@tsmc4@CL-att@fail\endcsname{0}
\expandafter\def\csname v@tsmc4@CL-att@wins\endcsname{37}
\expandafter\def\csname v@tsmc1@PROPOSED@med\endcsname{49.0}
\expandafter\def\csname v@tsmc1@PROPOSED@fail\endcsname{0}
\expandafter\def\csname v@tsmc2@PROPOSED@med\endcsname{50.0}
\expandafter\def\csname v@tsmc2@PROPOSED@fail\endcsname{0}
\expandafter\def\csname v@tsmc4@PROPOSED@med\endcsname{52.0}
\expandafter\def\csname v@tsmc4@PROPOSED@fail\endcsname{0}
\expandafter\def\csname v@time@LQR@mat\endcsname{20}
\expandafter\def\csname v@time@LQR@mex\endcsname{0.3}
\expandafter\def\csname v@time@MRAC@mat\endcsname{32}
\expandafter\def\csname v@time@MRAC@mex\endcsname{0.5}
\expandafter\def\csname v@time@B1@mat\endcsname{30}
\expandafter\def\csname v@time@B1@mex\endcsname{--}
\expandafter\def\csname v@time@NN-MRAC@mat\endcsname{29}
\expandafter\def\csname v@time@NN-MRAC@mex\endcsname{0.5}
\expandafter\def\csname v@time@CL-ucmd@mat\endcsname{45}
\expandafter\def\csname v@time@CL-ucmd@mex\endcsname{4.5}
\expandafter\def\csname v@time@CL-att@mat\endcsname{43}
\expandafter\def\csname v@time@CL-att@mex\endcsname{4.4}
\expandafter\def\csname v@time@PROPOSED@mat\endcsname{46}
\expandafter\def\csname v@time@PROPOSED@mex\endcsname{4.5}
\expandafter\def\csname v@an@in@GM\endcsname{Inf}
\expandafter\def\csname v@an@in@PM\endcsname{48.1}
\expandafter\def\csname v@an@in@wc\endcsname{14.98}
\expandafter\def\csname v@an@in@DM\endcsname{56.0}
\expandafter\def\csname v@an@out@GM\endcsname{11.8}
\expandafter\def\csname v@an@out@PM\endcsname{49.9}
\expandafter\def\csname v@an@out@wc\endcsname{3.06}
\expandafter\def\csname v@an@out@DM\endcsname{284.0}
\expandafter\def\csname v@an@in@Ms\endcsname{1.33}
\expandafter\def\csname v@an@out@Ms\endcsname{1.56}
\expandafter\def\csname v@an@rob@jmin\endcsname{0.20}
\expandafter\def\csname v@an@rob@jmax\endcsname{3.80}
\expandafter\def\csname v@an@rob@tmax\endcsname{115}
\expandafter\def\csname v@an@step@dev\endcsname{36.0}
\expandafter\def\csname v@an@lin@tr\endcsname{1.04}
\expandafter\def\csname v@an@lin@ts\endcsname{1.91}
\expandafter\def\csname v@an@lin@OS\endcsname{0.1}
\expandafter\def\csname v@an@nl@tr\endcsname{1.08}
\expandafter\def\csname v@an@nl@ts\endcsname{1.95}
\expandafter\def\csname v@an@nl@OS\endcsname{0.1}
\expandafter\def\csname v@an@rmo@tr\endcsname{1.08}
\expandafter\def\csname v@an@rmo@ts\endcsname{2.98}
\expandafter\def\csname v@an@rmo@OS\endcsname{4.3}
\expandafter\def\csname v@an@rmi@tr\endcsname{0.21}
\expandafter\def\csname v@an@rmi@ts\endcsname{0.60}
\expandafter\def\csname v@an@rmi@OS\endcsname{4.3}
\expandafter\def\csname v@sl@all@maxdp\endcsname{1.6\times10^{-7}}
\expandafter\def\csname v@sl@all@maxdr\endcsname{1.1\times10^{-8}}
\expandafter\def\csname v@sl@all@n\endcsname{14}
\expandafter\def\csname v@sitlSii@LQR@RMSE5\endcsname{671}
\expandafter\def\csname v@sitlSii@LQR@RMSE5sd\endcsname{96}
\expandafter\def\csname v@sitlSii@LQR@RMSEest\endcsname{329}
\expandafter\def\csname v@sitlSii@LQR@RMSEestsd\endcsname{18}
\expandafter\def\csname v@sitlSii@LQR@esterr\endcsname{414}
\expandafter\def\csname v@sitlSii@LQR@esterrsd\endcsname{119}
\expandafter\def\csname v@sitlSii@LQR@DW\endcsname{1.50}
\expandafter\def\csname v@sitlSii@LQR@DWsd\endcsname{0.13}
\expandafter\def\csname v@sitlSii@LQR@DWfive\endcsname{1.47}
\expandafter\def\csname v@sitlSii@LQR@DWfivesd\endcsname{0.06}
\expandafter\def\csname v@sitlSii@LQR@TV\endcsname{2527}
\expandafter\def\csname v@sitlSii@LQR@TVsd\endcsname{15}
\expandafter\def\csname v@sitlSii@LQR@cpu\endcsname{0.7}
\expandafter\def\csname v@sitlSii@LQR@cpusd\endcsname{0.1}
\expandafter\def\csname v@sitlSii@LQR@cpuP\endcsname{1.8}
\expandafter\def\csname v@sitlSii@LQR@cpuPsd\endcsname{0.6}
\expandafter\def\csname v@sitlSii@LQR@N\endcsname{5}
\expandafter\def\csname v@sitlSii@PROPOSED@RMSE5\endcsname{438}
\expandafter\def\csname v@sitlSii@PROPOSED@RMSE5sd\endcsname{83}
\expandafter\def\csname v@sitlSii@PROPOSED@RMSEest\endcsname{184}
\expandafter\def\csname v@sitlSii@PROPOSED@RMSEestsd\endcsname{27}
\expandafter\def\csname v@sitlSii@PROPOSED@esterr\endcsname{338}
\expandafter\def\csname v@sitlSii@PROPOSED@esterrsd\endcsname{72}
\expandafter\def\csname v@sitlSii@PROPOSED@DW\endcsname{2.05}
\expandafter\def\csname v@sitlSii@PROPOSED@DWsd\endcsname{0.31}
\expandafter\def\csname v@sitlSii@PROPOSED@DWfive\endcsname{1.74}
\expandafter\def\csname v@sitlSii@PROPOSED@DWfivesd\endcsname{0.09}
\expandafter\def\csname v@sitlSii@PROPOSED@TV\endcsname{3088}
\expandafter\def\csname v@sitlSii@PROPOSED@TVsd\endcsname{170}
\expandafter\def\csname v@sitlSii@PROPOSED@cpu\endcsname{4.9}
\expandafter\def\csname v@sitlSii@PROPOSED@cpusd\endcsname{0.4}
\expandafter\def\csname v@sitlSii@PROPOSED@cpuP\endcsname{10.9}
\expandafter\def\csname v@sitlSii@PROPOSED@cpuPsd\endcsname{3.9}
\expandafter\def\csname v@sitlSii@PROPOSED@N\endcsname{5}
\expandafter\def\csname v@sitlWind@LQR@RMSE5\endcsname{729}
\expandafter\def\csname v@sitlWind@LQR@RMSE5sd\endcsname{85}
\expandafter\def\csname v@sitlWind@LQR@RMSEest\endcsname{514}
\expandafter\def\csname v@sitlWind@LQR@RMSEestsd\endcsname{18}
\expandafter\def\csname v@sitlWind@LQR@esterr\endcsname{381}
\expandafter\def\csname v@sitlWind@LQR@esterrsd\endcsname{54}
\expandafter\def\csname v@sitlWind@LQR@DW\endcsname{1.80}
\expandafter\def\csname v@sitlWind@LQR@DWsd\endcsname{0.06}
\expandafter\def\csname v@sitlWind@LQR@DWfive\endcsname{1.76}
\expandafter\def\csname v@sitlWind@LQR@DWfivesd\endcsname{0.04}
\expandafter\def\csname v@sitlWind@LQR@TV\endcsname{2584}
\expandafter\def\csname v@sitlWind@LQR@TVsd\endcsname{23}
\expandafter\def\csname v@sitlWind@LQR@cpu\endcsname{0.7}
\expandafter\def\csname v@sitlWind@LQR@cpusd\endcsname{0.1}
\expandafter\def\csname v@sitlWind@LQR@cpuP\endcsname{1.7}
\expandafter\def\csname v@sitlWind@LQR@cpuPsd\endcsname{0.6}
\expandafter\def\csname v@sitlWind@LQR@N\endcsname{5}
\expandafter\def\csname v@sitlWind@PROPOSED@RMSE5\endcsname{499}
\expandafter\def\csname v@sitlWind@PROPOSED@RMSE5sd\endcsname{63}
\expandafter\def\csname v@sitlWind@PROPOSED@RMSEest\endcsname{213}
\expandafter\def\csname v@sitlWind@PROPOSED@RMSEestsd\endcsname{25}
\expandafter\def\csname v@sitlWind@PROPOSED@esterr\endcsname{372}
\expandafter\def\csname v@sitlWind@PROPOSED@esterrsd\endcsname{66}
\expandafter\def\csname v@sitlWind@PROPOSED@DW\endcsname{2.77}
\expandafter\def\csname v@sitlWind@PROPOSED@DWsd\endcsname{0.61}
\expandafter\def\csname v@sitlWind@PROPOSED@DWfive\endcsname{2.30}
\expandafter\def\csname v@sitlWind@PROPOSED@DWfivesd\endcsname{0.19}
\expandafter\def\csname v@sitlWind@PROPOSED@TV\endcsname{3395}
\expandafter\def\csname v@sitlWind@PROPOSED@TVsd\endcsname{204}
\expandafter\def\csname v@sitlWind@PROPOSED@cpu\endcsname{4.7}
\expandafter\def\csname v@sitlWind@PROPOSED@cpusd\endcsname{0.1}
\expandafter\def\csname v@sitlWind@PROPOSED@cpuP\endcsname{9.6}
\expandafter\def\csname v@sitlWind@PROPOSED@cpuPsd\endcsname{2.3}
\expandafter\def\csname v@sitlWind@PROPOSED@N\endcsname{5}
\expandafter\def\csname v@sitlHover@LQR@RMSE5\endcsname{583}
\expandafter\def\csname v@sitlHover@LQR@RMSE5sd\endcsname{148}
\expandafter\def\csname v@sitlHover@LQR@RMSEest\endcsname{136}
\expandafter\def\csname v@sitlHover@LQR@RMSEestsd\endcsname{20}
\expandafter\def\csname v@sitlHover@LQR@esterr\endcsname{540}
\expandafter\def\csname v@sitlHover@LQR@esterrsd\endcsname{170}
\expandafter\def\csname v@sitlHover@LQR@DW\endcsname{1.49}
\expandafter\def\csname v@sitlHover@LQR@DWsd\endcsname{0.66}
\expandafter\def\csname v@sitlHover@LQR@DWfive\endcsname{0.70}
\expandafter\def\csname v@sitlHover@LQR@DWfivesd\endcsname{0.10}
\expandafter\def\csname v@sitlHover@LQR@TV\endcsname{1987}
\expandafter\def\csname v@sitlHover@LQR@TVsd\endcsname{54}
\expandafter\def\csname v@sitlHover@LQR@cpu\endcsname{0.7}
\expandafter\def\csname v@sitlHover@LQR@cpusd\endcsname{0.0}
\expandafter\def\csname v@sitlHover@LQR@cpuP\endcsname{1.7}
\expandafter\def\csname v@sitlHover@LQR@cpuPsd\endcsname{0.4}
\expandafter\def\csname v@sitlHover@LQR@N\endcsname{5}
\expandafter\def\csname v@sitlHover@PROPOSED@RMSE5\endcsname{501}
\expandafter\def\csname v@sitlHover@PROPOSED@RMSE5sd\endcsname{215}
\expandafter\def\csname v@sitlHover@PROPOSED@RMSEest\endcsname{125}
\expandafter\def\csname v@sitlHover@PROPOSED@RMSEestsd\endcsname{19}
\expandafter\def\csname v@sitlHover@PROPOSED@esterr\endcsname{439}
\expandafter\def\csname v@sitlHover@PROPOSED@esterrsd\endcsname{240}
\expandafter\def\csname v@sitlHover@PROPOSED@DW\endcsname{1.89}
\expandafter\def\csname v@sitlHover@PROPOSED@DWsd\endcsname{1.08}
\expandafter\def\csname v@sitlHover@PROPOSED@DWfive\endcsname{0.68}
\expandafter\def\csname v@sitlHover@PROPOSED@DWfivesd\endcsname{0.01}
\expandafter\def\csname v@sitlHover@PROPOSED@TV\endcsname{2324}
\expandafter\def\csname v@sitlHover@PROPOSED@TVsd\endcsname{103}
\expandafter\def\csname v@sitlHover@PROPOSED@cpu\endcsname{4.9}
\expandafter\def\csname v@sitlHover@PROPOSED@cpusd\endcsname{0.4}
\expandafter\def\csname v@sitlHover@PROPOSED@cpuP\endcsname{9.6}
\expandafter\def\csname v@sitlHover@PROPOSED@cpuPsd\endcsname{4.4}
\expandafter\def\csname v@sitlHover@PROPOSED@N\endcsname{5}
\expandafter\def\csname v@sitlGTSii@LQR@RMSE5\endcsname{231.3}
\expandafter\def\csname v@sitlGTSii@LQR@RMSE5sd\endcsname{0.0}
\expandafter\def\csname v@sitlGTSii@LQR@RMSEest\endcsname{231}
\expandafter\def\csname v@sitlGTSii@LQR@RMSEestsd\endcsname{0}
\expandafter\def\csname v@sitlGTSii@LQR@esterr\endcsname{0}
\expandafter\def\csname v@sitlGTSii@LQR@esterrsd\endcsname{0}
\expandafter\def\csname v@sitlGTSii@LQR@DW\endcsname{1.10}
\expandafter\def\csname v@sitlGTSii@LQR@DWsd\endcsname{0.00}
\expandafter\def\csname v@sitlGTSii@LQR@DWfive\endcsname{1.15}
\expandafter\def\csname v@sitlGTSii@LQR@DWfivesd\endcsname{0.00}
\expandafter\def\csname v@sitlGTSii@LQR@TV\endcsname{167}
\expandafter\def\csname v@sitlGTSii@LQR@TVsd\endcsname{0}
\expandafter\def\csname v@sitlGTSii@LQR@cpu\endcsname{0.7}
\expandafter\def\csname v@sitlGTSii@LQR@cpusd\endcsname{0.0}
\expandafter\def\csname v@sitlGTSii@LQR@cpuP\endcsname{1.3}
\expandafter\def\csname v@sitlGTSii@LQR@cpuPsd\endcsname{0.0}
\expandafter\def\csname v@sitlGTSii@LQR@N\endcsname{1}
\expandafter\def\csname v@sitlGTSii@PROPOSED@RMSE5\endcsname{29.7}
\expandafter\def\csname v@sitlGTSii@PROPOSED@RMSE5sd\endcsname{0.0}
\expandafter\def\csname v@sitlGTSii@PROPOSED@RMSEest\endcsname{30}
\expandafter\def\csname v@sitlGTSii@PROPOSED@RMSEestsd\endcsname{0}
\expandafter\def\csname v@sitlGTSii@PROPOSED@esterr\endcsname{0}
\expandafter\def\csname v@sitlGTSii@PROPOSED@esterrsd\endcsname{0}
\expandafter\def\csname v@sitlGTSii@PROPOSED@DW\endcsname{1.05}
\expandafter\def\csname v@sitlGTSii@PROPOSED@DWsd\endcsname{0.00}
\expandafter\def\csname v@sitlGTSii@PROPOSED@DWfive\endcsname{1.09}
\expandafter\def\csname v@sitlGTSii@PROPOSED@DWfivesd\endcsname{0.00}
\expandafter\def\csname v@sitlGTSii@PROPOSED@TV\endcsname{279}
\expandafter\def\csname v@sitlGTSii@PROPOSED@TVsd\endcsname{0}
\expandafter\def\csname v@sitlGTSii@PROPOSED@cpu\endcsname{4.6}
\expandafter\def\csname v@sitlGTSii@PROPOSED@cpusd\endcsname{0.0}
\expandafter\def\csname v@sitlGTSii@PROPOSED@cpuP\endcsname{8.5}
\expandafter\def\csname v@sitlGTSii@PROPOSED@cpuPsd\endcsname{0.0}
\expandafter\def\csname v@sitlGTSii@PROPOSED@N\endcsname{1}
\expandafter\def\csname v@sitlGTWind@LQR@RMSE5\endcsname{431.7}
\expandafter\def\csname v@sitlGTWind@LQR@RMSE5sd\endcsname{0.0}
\expandafter\def\csname v@sitlGTWind@LQR@RMSEest\endcsname{432}
\expandafter\def\csname v@sitlGTWind@LQR@RMSEestsd\endcsname{0}
\expandafter\def\csname v@sitlGTWind@LQR@esterr\endcsname{0}
\expandafter\def\csname v@sitlGTWind@LQR@esterrsd\endcsname{0}
\expandafter\def\csname v@sitlGTWind@LQR@DW\endcsname{1.41}
\expandafter\def\csname v@sitlGTWind@LQR@DWsd\endcsname{0.00}
\expandafter\def\csname v@sitlGTWind@LQR@DWfive\endcsname{1.47}
\expandafter\def\csname v@sitlGTWind@LQR@DWfivesd\endcsname{0.00}
\expandafter\def\csname v@sitlGTWind@LQR@TV\endcsname{215}
\expandafter\def\csname v@sitlGTWind@LQR@TVsd\endcsname{0}
\expandafter\def\csname v@sitlGTWind@LQR@cpu\endcsname{0.7}
\expandafter\def\csname v@sitlGTWind@LQR@cpusd\endcsname{0.0}
\expandafter\def\csname v@sitlGTWind@LQR@cpuP\endcsname{1.3}
\expandafter\def\csname v@sitlGTWind@LQR@cpuPsd\endcsname{0.0}
\expandafter\def\csname v@sitlGTWind@LQR@N\endcsname{1}
\expandafter\def\csname v@sitlGTWind@PROPOSED@RMSE5\endcsname{48.1}
\expandafter\def\csname v@sitlGTWind@PROPOSED@RMSE5sd\endcsname{0.0}
\expandafter\def\csname v@sitlGTWind@PROPOSED@RMSEest\endcsname{48}
\expandafter\def\csname v@sitlGTWind@PROPOSED@RMSEestsd\endcsname{0}
\expandafter\def\csname v@sitlGTWind@PROPOSED@esterr\endcsname{0}
\expandafter\def\csname v@sitlGTWind@PROPOSED@esterrsd\endcsname{0}
\expandafter\def\csname v@sitlGTWind@PROPOSED@DW\endcsname{1.44}
\expandafter\def\csname v@sitlGTWind@PROPOSED@DWsd\endcsname{0.00}
\expandafter\def\csname v@sitlGTWind@PROPOSED@DWfive\endcsname{1.50}
\expandafter\def\csname v@sitlGTWind@PROPOSED@DWfivesd\endcsname{0.00}
\expandafter\def\csname v@sitlGTWind@PROPOSED@TV\endcsname{400}
\expandafter\def\csname v@sitlGTWind@PROPOSED@TVsd\endcsname{0}
\expandafter\def\csname v@sitlGTWind@PROPOSED@cpu\endcsname{4.7}
\expandafter\def\csname v@sitlGTWind@PROPOSED@cpusd\endcsname{0.0}
\expandafter\def\csname v@sitlGTWind@PROPOSED@cpuP\endcsname{8.6}
\expandafter\def\csname v@sitlGTWind@PROPOSED@cpuPsd\endcsname{0.0}
\expandafter\def\csname v@sitlGTWind@PROPOSED@N\endcsname{1}
\expandafter\def\csname v@sitlSii@all@wins\endcsname{5}
\expandafter\def\csname v@sitlSii@all@redmin\endcsname{17}
\expandafter\def\csname v@sitlSii@all@redmax\endcsname{43}
\expandafter\def\csname v@sitlWind@all@wins\endcsname{5}
\expandafter\def\csname v@sitlWind@all@redmin\endcsname{17}
\expandafter\def\csname v@sitlWind@all@redmax\endcsname{40}
\expandafter\def\csname v@sitl@all@nto\endcsname{19}
\expandafter\def\csname v@sitl@all@nruns\endcsname{34}
\expandafter\def\csname v@sitlHover@all@ratio\endcsname{0.97}
\expandafter\def\csname v@sitlSii@all@ratio\endcsname{1.36}
\expandafter\def\csname v@det@LQR@design\endcsname{340.0}
\expandafter\def\csname v@det@LQR@eval6\endcsname{482.9}
\expandafter\def\csname v@det@LQR@held\endcsname{536.6}
\expandafter\def\csname v@det@LQR@S1\endcsname{161.2}
\expandafter\def\csname v@det@LQR@DWS1\endcsname{0.04}
\expandafter\def\csname v@det@LQR@TVS1\endcsname{20}
\expandafter\def\csname v@det@LQR@S2\endcsname{230.9}
\expandafter\def\csname v@det@LQR@DWS2\endcsname{1.10}
\expandafter\def\csname v@det@LQR@TVS2\endcsname{168}
\expandafter\def\csname v@det@LQR@S3\endcsname{450.2}
\expandafter\def\csname v@det@LQR@DWS3\endcsname{0.04}
\expandafter\def\csname v@det@LQR@TVS3\endcsname{37}
\expandafter\def\csname v@det@LQR@S4\endcsname{339.0}
\expandafter\def\csname v@det@LQR@DWS4\endcsname{1.40}
\expandafter\def\csname v@det@LQR@TVS4\endcsname{255}
\expandafter\def\csname v@det@LQR@S5\endcsname{1126.5}
\expandafter\def\csname v@det@LQR@DWS5\endcsname{11.51}
\expandafter\def\csname v@det@LQR@TVS5\endcsname{36294}
\expandafter\def\csname v@det@LQR@S6\endcsname{0.0}
\expandafter\def\csname v@det@LQR@DWS6\endcsname{0.11}
\expandafter\def\csname v@det@LQR@TVS6\endcsname{88}
\expandafter\def\csname v@det@LQR@S7\endcsname{1.2}
\expandafter\def\csname v@det@LQR@DWS7\endcsname{12.41}
\expandafter\def\csname v@det@LQR@TVS7\endcsname{39516}
\expandafter\def\csname v@det@LQR@S8\endcsname{465.8}
\expandafter\def\csname v@det@LQR@DWS8\endcsname{11.76}
\expandafter\def\csname v@det@LQR@TVS8\endcsname{37476}
\expandafter\def\csname v@det@LQR@S9\endcsname{552.7}
\expandafter\def\csname v@det@LQR@DWS9\endcsname{13.67}
\expandafter\def\csname v@det@LQR@TVS9\endcsname{42744}
\expandafter\def\csname v@det@LQR@S10\endcsname{591.1}
\expandafter\def\csname v@det@LQR@DWS10\endcsname{11.27}
\expandafter\def\csname v@det@LQR@TVS10\endcsname{35905}
\expandafter\def\csname v@det@MRAC@design\endcsname{86.5}
\expandafter\def\csname v@det@MRAC@eval6\endcsname{83.8}
\expandafter\def\csname v@det@MRAC@held\endcsname{109.2}
\expandafter\def\csname v@det@MRAC@S1\endcsname{31.3}
\expandafter\def\csname v@det@MRAC@DWS1\endcsname{0.04}
\expandafter\def\csname v@det@MRAC@TVS1\endcsname{34}
\expandafter\def\csname v@det@MRAC@S2\endcsname{76.6}
\expandafter\def\csname v@det@MRAC@DWS2\endcsname{2.97}
\expandafter\def\csname v@det@MRAC@TVS2\endcsname{800}
\expandafter\def\csname v@det@MRAC@S3\endcsname{88.8}
\expandafter\def\csname v@det@MRAC@DWS3\endcsname{0.15}
\expandafter\def\csname v@det@MRAC@TVS3\endcsname{255}
\expandafter\def\csname v@det@MRAC@S4\endcsname{93.9}
\expandafter\def\csname v@det@MRAC@DWS4\endcsname{4.08}
\expandafter\def\csname v@det@MRAC@TVS4\endcsname{1259}
\expandafter\def\csname v@det@MRAC@S5\endcsname{138.4}
\expandafter\def\csname v@det@MRAC@DWS5\endcsname{26.62}
\expandafter\def\csname v@det@MRAC@TVS5\endcsname{72263}
\expandafter\def\csname v@det@MRAC@S6\endcsname{5.5}
\expandafter\def\csname v@det@MRAC@DWS6\endcsname{0.12}
\expandafter\def\csname v@det@MRAC@TVS6\endcsname{159}
\expandafter\def\csname v@det@MRAC@S7\endcsname{3.6}
\expandafter\def\csname v@det@MRAC@DWS7\endcsname{12.68}
\expandafter\def\csname v@det@MRAC@TVS7\endcsname{40368}
\expandafter\def\csname v@det@MRAC@S8\endcsname{68.0}
\expandafter\def\csname v@det@MRAC@DWS8\endcsname{12.09}
\expandafter\def\csname v@det@MRAC@TVS8\endcsname{38517}
\expandafter\def\csname v@det@MRAC@S9\endcsname{147.6}
\expandafter\def\csname v@det@MRAC@DWS9\endcsname{38.36}
\expandafter\def\csname v@det@MRAC@TVS9\endcsname{100375}
\expandafter\def\csname v@det@MRAC@S10\endcsname{112.2}
\expandafter\def\csname v@det@MRAC@DWS10\endcsname{16.38}
\expandafter\def\csname v@det@MRAC@TVS10\endcsname{51260}
\expandafter\def\csname v@det@B1@S1\endcsname{36.2}
\expandafter\def\csname v@det@B1@DWS1\endcsname{0.28}
\expandafter\def\csname v@det@B1@TVS1\endcsname{151}
\expandafter\def\csname v@det@B1@S2\endcsname{85.6}
\expandafter\def\csname v@det@B1@DWS2\endcsname{2.31}
\expandafter\def\csname v@det@B1@TVS2\endcsname{1195}
\expandafter\def\csname v@det@B1@S3\endcsname{36818.0}
\expandafter\def\csname v@det@B1@DWS3\endcsname{6.38}
\expandafter\def\csname v@det@B1@TVS3\endcsname{4475}
\expandafter\def\csname v@det@B1@S4\endcsname{136.4}
\expandafter\def\csname v@det@B1@DWS4\endcsname{4.16}
\expandafter\def\csname v@det@B1@TVS4\endcsname{1591}
\expandafter\def\csname v@det@B1@S5\endcsname{31541.3}
\expandafter\def\csname v@det@B1@DWS5\endcsname{23.21}
\expandafter\def\csname v@det@B1@TVS5\endcsname{22884}
\expandafter\def\csname v@det@B1@S6\endcsname{15.2}
\expandafter\def\csname v@det@B1@DWS6\endcsname{0.66}
\expandafter\def\csname v@det@B1@TVS6\endcsname{555}
\expandafter\def\csname v@det@B1@S7\endcsname{8.7}
\expandafter\def\csname v@det@B1@DWS7\endcsname{10.76}
\expandafter\def\csname v@det@B1@TVS7\endcsname{32797}
\expandafter\def\csname v@det@B1@S8\endcsname{23549.2}
\expandafter\def\csname v@det@B1@DWS8\endcsname{16.32}
\expandafter\def\csname v@det@B1@TVS8\endcsname{22148}
\expandafter\def\csname v@det@B1@S9\endcsname{23526.0}
\expandafter\def\csname v@det@B1@DWS9\endcsname{31.31}
\expandafter\def\csname v@det@B1@TVS9\endcsname{27150}
\expandafter\def\csname v@det@B1@S10\endcsname{34132.4}
\expandafter\def\csname v@det@B1@DWS10\endcsname{15.24}
\expandafter\def\csname v@det@B1@TVS10\endcsname{18419}
\expandafter\def\csname v@det@NNMRAC@design\endcsname{82.6}
\expandafter\def\csname v@det@NNMRAC@eval6\endcsname{84.5}
\expandafter\def\csname v@det@NNMRAC@held\endcsname{104.9}
\expandafter\def\csname v@det@NNMRAC@S1\endcsname{37.0}
\expandafter\def\csname v@det@NNMRAC@DWS1\endcsname{0.04}
\expandafter\def\csname v@det@NNMRAC@TVS1\endcsname{26}
\expandafter\def\csname v@det@NNMRAC@S2\endcsname{55.5}
\expandafter\def\csname v@det@NNMRAC@DWS2\endcsname{1.45}
\expandafter\def\csname v@det@NNMRAC@TVS2\endcsname{290}
\expandafter\def\csname v@det@NNMRAC@S3\endcsname{113.6}
\expandafter\def\csname v@det@NNMRAC@DWS3\endcsname{0.09}
\expandafter\def\csname v@det@NNMRAC@TVS3\endcsname{129}
\expandafter\def\csname v@det@NNMRAC@S4\endcsname{78.6}
\expandafter\def\csname v@det@NNMRAC@DWS4\endcsname{2.21}
\expandafter\def\csname v@det@NNMRAC@TVS4\endcsname{436}
\expandafter\def\csname v@det@NNMRAC@S5\endcsname{153.8}
\expandafter\def\csname v@det@NNMRAC@DWS5\endcsname{15.41}
\expandafter\def\csname v@det@NNMRAC@TVS5\endcsname{45459}
\expandafter\def\csname v@det@NNMRAC@S6\endcsname{1.7}
\expandafter\def\csname v@det@NNMRAC@DWS6\endcsname{0.12}
\expandafter\def\csname v@det@NNMRAC@TVS6\endcsname{124}
\expandafter\def\csname v@det@NNMRAC@S7\endcsname{1.6}
\expandafter\def\csname v@det@NNMRAC@DWS7\endcsname{12.51}
\expandafter\def\csname v@det@NNMRAC@TVS7\endcsname{39839}
\expandafter\def\csname v@det@NNMRAC@S8\endcsname{92.6}
\expandafter\def\csname v@det@NNMRAC@DWS8\endcsname{12.10}
\expandafter\def\csname v@det@NNMRAC@TVS8\endcsname{38535}
\expandafter\def\csname v@det@NNMRAC@S9\endcsname{125.9}
\expandafter\def\csname v@det@NNMRAC@DWS9\endcsname{18.80}
\expandafter\def\csname v@det@NNMRAC@TVS9\endcsname{54798}
\expandafter\def\csname v@det@NNMRAC@S10\endcsname{96.3}
\expandafter\def\csname v@det@NNMRAC@DWS10\endcsname{11.99}
\expandafter\def\csname v@det@NNMRAC@TVS10\endcsname{38123}
\expandafter\def\csname v@det@CLucmd@design\endcsname{77.8}
\expandafter\def\csname v@det@CLucmd@eval6\endcsname{82.1}
\expandafter\def\csname v@det@CLucmd@held\endcsname{104.3}
\expandafter\def\csname v@det@CLucmd@S1\endcsname{21.8}
\expandafter\def\csname v@det@CLucmd@DWS1\endcsname{0.04}
\expandafter\def\csname v@det@CLucmd@TVS1\endcsname{27}
\expandafter\def\csname v@det@CLucmd@S2\endcsname{74.0}
\expandafter\def\csname v@det@CLucmd@DWS2\endcsname{1.66}
\expandafter\def\csname v@det@CLucmd@TVS2\endcsname{296}
\expandafter\def\csname v@det@CLucmd@S3\endcsname{63.3}
\expandafter\def\csname v@det@CLucmd@DWS3\endcsname{0.07}
\expandafter\def\csname v@det@CLucmd@TVS3\endcsname{78}
\expandafter\def\csname v@det@CLucmd@S4\endcsname{96.1}
\expandafter\def\csname v@det@CLucmd@DWS4\endcsname{2.51}
\expandafter\def\csname v@det@CLucmd@TVS4\endcsname{461}
\expandafter\def\csname v@det@CLucmd@S5\endcsname{132.7}
\expandafter\def\csname v@det@CLucmd@DWS5\endcsname{22.15}
\expandafter\def\csname v@det@CLucmd@TVS5\endcsname{65080}
\expandafter\def\csname v@det@CLucmd@S6\endcsname{25.5}
\expandafter\def\csname v@det@CLucmd@DWS6\endcsname{0.11}
\expandafter\def\csname v@det@CLucmd@TVS6\endcsname{134}
\expandafter\def\csname v@det@CLucmd@S7\endcsname{15.0}
\expandafter\def\csname v@det@CLucmd@DWS7\endcsname{12.70}
\expandafter\def\csname v@det@CLucmd@TVS7\endcsname{40440}
\expandafter\def\csname v@det@CLucmd@S8\endcsname{97.7}
\expandafter\def\csname v@det@CLucmd@DWS8\endcsname{17.43}
\expandafter\def\csname v@det@CLucmd@TVS8\endcsname{53934}
\expandafter\def\csname v@det@CLucmd@S9\endcsname{137.8}
\expandafter\def\csname v@det@CLucmd@DWS9\endcsname{23.76}
\expandafter\def\csname v@det@CLucmd@TVS9\endcsname{71023}
\expandafter\def\csname v@det@CLucmd@S10\endcsname{77.3}
\expandafter\def\csname v@det@CLucmd@DWS10\endcsname{14.47}
\expandafter\def\csname v@det@CLucmd@TVS10\endcsname{45806}
\expandafter\def\csname v@det@CLatt@design\endcsname{46.2}
\expandafter\def\csname v@det@CLatt@eval6\endcsname{57.0}
\expandafter\def\csname v@det@CLatt@held\endcsname{57.9}
\expandafter\def\csname v@det@CLatt@S1\endcsname{25.4}
\expandafter\def\csname v@det@CLatt@DWS1\endcsname{0.06}
\expandafter\def\csname v@det@CLatt@TVS1\endcsname{31}
\expandafter\def\csname v@det@CLatt@S2\endcsname{41.5}
\expandafter\def\csname v@det@CLatt@DWS2\endcsname{1.13}
\expandafter\def\csname v@det@CLatt@TVS2\endcsname{201}
\expandafter\def\csname v@det@CLatt@S3\endcsname{46.1}
\expandafter\def\csname v@det@CLatt@DWS3\endcsname{0.11}
\expandafter\def\csname v@det@CLatt@TVS3\endcsname{75}
\expandafter\def\csname v@det@CLatt@S4\endcsname{50.9}
\expandafter\def\csname v@det@CLatt@DWS4\endcsname{2.53}
\expandafter\def\csname v@det@CLatt@TVS4\endcsname{451}
\expandafter\def\csname v@det@CLatt@S5\endcsname{142.2}
\expandafter\def\csname v@det@CLatt@DWS5\endcsname{20.47}
\expandafter\def\csname v@det@CLatt@TVS5\endcsname{62118}
\expandafter\def\csname v@det@CLatt@S6\endcsname{0.3}
\expandafter\def\csname v@det@CLatt@DWS6\endcsname{0.16}
\expandafter\def\csname v@det@CLatt@TVS6\endcsname{141}
\expandafter\def\csname v@det@CLatt@S7\endcsname{1.2}
\expandafter\def\csname v@det@CLatt@DWS7\endcsname{12.93}
\expandafter\def\csname v@det@CLatt@TVS7\endcsname{41160}
\expandafter\def\csname v@det@CLatt@S8\endcsname{69.5}
\expandafter\def\csname v@det@CLatt@DWS8\endcsname{19.02}
\expandafter\def\csname v@det@CLatt@TVS8\endcsname{58711}
\expandafter\def\csname v@det@CLatt@S9\endcsname{67.7}
\expandafter\def\csname v@det@CLatt@DWS9\endcsname{24.21}
\expandafter\def\csname v@det@CLatt@TVS9\endcsname{73213}
\expandafter\def\csname v@det@CLatt@S10\endcsname{36.7}
\expandafter\def\csname v@det@CLatt@DWS10\endcsname{17.19}
\expandafter\def\csname v@det@CLatt@TVS10\endcsname{54114}
\expandafter\def\csname v@det@PREDouter@design\endcsname{46.2}
\expandafter\def\csname v@det@PREDouter@eval6\endcsname{57.1}
\expandafter\def\csname v@det@PREDouter@held\endcsname{58.2}
\expandafter\def\csname v@det@PREDouter@S1\endcsname{25.4}
\expandafter\def\csname v@det@PREDouter@DWS1\endcsname{0.05}
\expandafter\def\csname v@det@PREDouter@TVS1\endcsname{30}
\expandafter\def\csname v@det@PREDouter@S2\endcsname{41.5}
\expandafter\def\csname v@det@PREDouter@DWS2\endcsname{1.14}
\expandafter\def\csname v@det@PREDouter@TVS2\endcsname{201}
\expandafter\def\csname v@det@PREDouter@S3\endcsname{46.1}
\expandafter\def\csname v@det@PREDouter@DWS3\endcsname{0.11}
\expandafter\def\csname v@det@PREDouter@TVS3\endcsname{74}
\expandafter\def\csname v@det@PREDouter@S4\endcsname{51.0}
\expandafter\def\csname v@det@PREDouter@DWS4\endcsname{2.55}
\expandafter\def\csname v@det@PREDouter@TVS4\endcsname{454}
\expandafter\def\csname v@det@PREDouter@S5\endcsname{142.3}
\expandafter\def\csname v@det@PREDouter@DWS5\endcsname{20.48}
\expandafter\def\csname v@det@PREDouter@TVS5\endcsname{62106}
\expandafter\def\csname v@det@PREDouter@S6\endcsname{0.4}
\expandafter\def\csname v@det@PREDouter@DWS6\endcsname{0.16}
\expandafter\def\csname v@det@PREDouter@TVS6\endcsname{142}
\expandafter\def\csname v@det@PREDouter@S7\endcsname{1.4}
\expandafter\def\csname v@det@PREDouter@DWS7\endcsname{12.89}
\expandafter\def\csname v@det@PREDouter@TVS7\endcsname{41042}
\expandafter\def\csname v@det@PREDouter@S8\endcsname{69.6}
\expandafter\def\csname v@det@PREDouter@DWS8\endcsname{19.01}
\expandafter\def\csname v@det@PREDouter@TVS8\endcsname{58697}
\expandafter\def\csname v@det@PREDouter@S9\endcsname{68.0}
\expandafter\def\csname v@det@PREDouter@DWS9\endcsname{24.25}
\expandafter\def\csname v@det@PREDouter@TVS9\endcsname{73319}
\expandafter\def\csname v@det@PREDouter@S10\endcsname{36.9}
\expandafter\def\csname v@det@PREDouter@DWS10\endcsname{17.17}
\expandafter\def\csname v@det@PREDouter@TVS10\endcsname{54031}
\expandafter\def\csname v@det@PREDinner@design\endcsname{37.3}
\expandafter\def\csname v@det@PREDinner@eval6\endcsname{46.1}
\expandafter\def\csname v@det@PREDinner@held\endcsname{47.2}
\expandafter\def\csname v@det@PREDinner@S1\endcsname{22.1}
\expandafter\def\csname v@det@PREDinner@DWS1\endcsname{0.11}
\expandafter\def\csname v@det@PREDinner@TVS1\endcsname{60}
\expandafter\def\csname v@det@PREDinner@S2\endcsname{29.4}
\expandafter\def\csname v@det@PREDinner@DWS2\endcsname{1.02}
\expandafter\def\csname v@det@PREDinner@TVS2\endcsname{283}
\expandafter\def\csname v@det@PREDinner@S3\endcsname{37.3}
\expandafter\def\csname v@det@PREDinner@DWS3\endcsname{0.24}
\expandafter\def\csname v@det@PREDinner@TVS3\endcsname{166}
\expandafter\def\csname v@det@PREDinner@S4\endcsname{45.2}
\expandafter\def\csname v@det@PREDinner@DWS4\endcsname{3.27}
\expandafter\def\csname v@det@PREDinner@TVS4\endcsname{738}
\expandafter\def\csname v@det@PREDinner@S5\endcsname{112.6}
\expandafter\def\csname v@det@PREDinner@DWS5\endcsname{23.08}
\expandafter\def\csname v@det@PREDinner@TVS5\endcsname{69566}
\expandafter\def\csname v@det@PREDinner@S6\endcsname{0.3}
\expandafter\def\csname v@det@PREDinner@DWS6\endcsname{0.33}
\expandafter\def\csname v@det@PREDinner@TVS6\endcsname{291}
\expandafter\def\csname v@det@PREDinner@S7\endcsname{1.1}
\expandafter\def\csname v@det@PREDinner@DWS7\endcsname{13.01}
\expandafter\def\csname v@det@PREDinner@TVS7\endcsname{41394}
\expandafter\def\csname v@det@PREDinner@S8\endcsname{53.5}
\expandafter\def\csname v@det@PREDinner@DWS8\endcsname{21.18}
\expandafter\def\csname v@det@PREDinner@TVS8\endcsname{64683}
\expandafter\def\csname v@det@PREDinner@S9\endcsname{60.1}
\expandafter\def\csname v@det@PREDinner@DWS9\endcsname{26.02}
\expandafter\def\csname v@det@PREDinner@TVS9\endcsname{78067}
\expandafter\def\csname v@det@PREDinner@S10\endcsname{28.1}
\expandafter\def\csname v@det@PREDinner@DWS10\endcsname{23.06}
\expandafter\def\csname v@det@PREDinner@TVS10\endcsname{72245}
\expandafter\def\csname v@det@PROPOSED@design\endcsname{35.8}
\expandafter\def\csname v@det@PROPOSED@eval6\endcsname{45.1}
\expandafter\def\csname v@det@PROPOSED@held\endcsname{45.1}
\expandafter\def\csname v@det@PROPOSED@S1\endcsname{21.4}
\expandafter\def\csname v@det@PROPOSED@DWS1\endcsname{0.16}
\expandafter\def\csname v@det@PROPOSED@TVS1\endcsname{85}
\expandafter\def\csname v@det@PROPOSED@S2\endcsname{27.5}
\expandafter\def\csname v@det@PROPOSED@DWS2\endcsname{1.01}
\expandafter\def\csname v@det@PROPOSED@TVS2\endcsname{350}
\expandafter\def\csname v@det@PROPOSED@S3\endcsname{35.8}
\expandafter\def\csname v@det@PROPOSED@DWS3\endcsname{0.38}
\expandafter\def\csname v@det@PROPOSED@TVS3\endcsname{246}
\expandafter\def\csname v@det@PROPOSED@S4\endcsname{44.0}
\expandafter\def\csname v@det@PROPOSED@DWS4\endcsname{3.40}
\expandafter\def\csname v@det@PROPOSED@TVS4\endcsname{838}
\expandafter\def\csname v@det@PROPOSED@S5\endcsname{113.6}
\expandafter\def\csname v@det@PROPOSED@DWS5\endcsname{22.92}
\expandafter\def\csname v@det@PROPOSED@TVS5\endcsname{68993}
\expandafter\def\csname v@det@PROPOSED@S6\endcsname{0.4}
\expandafter\def\csname v@det@PROPOSED@DWS6\endcsname{0.58}
\expandafter\def\csname v@det@PROPOSED@TVS6\endcsname{447}
\expandafter\def\csname v@det@PROPOSED@S7\endcsname{1.3}
\expandafter\def\csname v@det@PROPOSED@DWS7\endcsname{12.98}
\expandafter\def\csname v@det@PROPOSED@TVS7\endcsname{41253}
\expandafter\def\csname v@det@PROPOSED@S8\endcsname{51.2}
\expandafter\def\csname v@det@PROPOSED@DWS8\endcsname{21.87}
\expandafter\def\csname v@det@PROPOSED@TVS8\endcsname{66759}
\expandafter\def\csname v@det@PROPOSED@S9\endcsname{57.0}
\expandafter\def\csname v@det@PROPOSED@DWS9\endcsname{27.66}
\expandafter\def\csname v@det@PROPOSED@TVS9\endcsname{82824}
\expandafter\def\csname v@det@PROPOSED@S10\endcsname{27.3}
\expandafter\def\csname v@det@PROPOSED@DWS10\endcsname{23.33}
\expandafter\def\csname v@det@PROPOSED@TVS10\endcsname{72849}
\expandafter\def\csname v@det@GUARDnone@design\endcsname{49.6}
\expandafter\def\csname v@det@GUARDnone@eval6\endcsname{60.5}
\expandafter\def\csname v@det@GUARDnone@held\endcsname{61.8}
\expandafter\def\csname v@det@GUARDnone@S1\endcsname{25.5}
\expandafter\def\csname v@det@GUARDnone@DWS1\endcsname{0.05}
\expandafter\def\csname v@det@GUARDnone@S2\endcsname{44.4}
\expandafter\def\csname v@det@GUARDnone@DWS2\endcsname{1.16}
\expandafter\def\csname v@det@GUARDnone@S3\endcsname{49.2}
\expandafter\def\csname v@det@GUARDnone@DWS3\endcsname{0.09}
\expandafter\def\csname v@det@GUARDnone@S4\endcsname{55.0}
\expandafter\def\csname v@det@GUARDnone@DWS4\endcsname{2.15}
\expandafter\def\csname v@det@GUARDnone@S5\endcsname{151.4}
\expandafter\def\csname v@det@GUARDnone@DWS5\endcsname{20.05}
\expandafter\def\csname v@det@GUARDnone@S6\endcsname{0.4}
\expandafter\def\csname v@det@GUARDnone@DWS6\endcsname{0.13}
\expandafter\def\csname v@det@GUARDnone@S7\endcsname{1.2}
\expandafter\def\csname v@det@GUARDnone@DWS7\endcsname{12.57}
\expandafter\def\csname v@det@GUARDnone@S8\endcsname{74.0}
\expandafter\def\csname v@det@GUARDnone@DWS8\endcsname{18.26}
\expandafter\def\csname v@det@GUARDnone@S9\endcsname{69.4}
\expandafter\def\csname v@det@GUARDnone@DWS9\endcsname{22.59}
\expandafter\def\csname v@det@GUARDnone@S10\endcsname{42.1}
\expandafter\def\csname v@det@GUARDnone@DWS10\endcsname{15.75}
\expandafter\def\csname v@det@GUARDouter@design\endcsname{49.6}
\expandafter\def\csname v@det@GUARDouter@eval6\endcsname{60.5}
\expandafter\def\csname v@det@GUARDouter@held\endcsname{62.0}
\expandafter\def\csname v@det@GUARDouter@S1\endcsname{25.5}
\expandafter\def\csname v@det@GUARDouter@DWS1\endcsname{0.05}
\expandafter\def\csname v@det@GUARDouter@S2\endcsname{44.5}
\expandafter\def\csname v@det@GUARDouter@DWS2\endcsname{1.16}
\expandafter\def\csname v@det@GUARDouter@S3\endcsname{49.3}
\expandafter\def\csname v@det@GUARDouter@DWS3\endcsname{0.09}
\expandafter\def\csname v@det@GUARDouter@S4\endcsname{55.1}
\expandafter\def\csname v@det@GUARDouter@DWS4\endcsname{2.17}
\expandafter\def\csname v@det@GUARDouter@S5\endcsname{151.3}
\expandafter\def\csname v@det@GUARDouter@DWS5\endcsname{20.05}
\expandafter\def\csname v@det@GUARDouter@S6\endcsname{0.4}
\expandafter\def\csname v@det@GUARDouter@DWS6\endcsname{0.13}
\expandafter\def\csname v@det@GUARDouter@S7\endcsname{1.4}
\expandafter\def\csname v@det@GUARDouter@DWS7\endcsname{12.54}
\expandafter\def\csname v@det@GUARDouter@S8\endcsname{74.2}
\expandafter\def\csname v@det@GUARDouter@DWS8\endcsname{18.26}
\expandafter\def\csname v@det@GUARDouter@S9\endcsname{69.6}
\expandafter\def\csname v@det@GUARDouter@DWS9\endcsname{22.63}
\expandafter\def\csname v@det@GUARDouter@S10\endcsname{42.3}
\expandafter\def\csname v@det@GUARDouter@DWS10\endcsname{15.74}
\expandafter\def\csname v@det@GUARDinner@design\endcsname{42.0}
\expandafter\def\csname v@det@GUARDinner@eval6\endcsname{51.9}
\expandafter\def\csname v@det@GUARDinner@held\endcsname{54.1}
\expandafter\def\csname v@det@GUARDinner@S1\endcsname{24.9}
\expandafter\def\csname v@det@GUARDinner@DWS1\endcsname{0.06}
\expandafter\def\csname v@det@GUARDinner@S2\endcsname{36.1}
\expandafter\def\csname v@det@GUARDinner@DWS2\endcsname{1.06}
\expandafter\def\csname v@det@GUARDinner@S3\endcsname{43.1}
\expandafter\def\csname v@det@GUARDinner@DWS3\endcsname{0.15}
\expandafter\def\csname v@det@GUARDinner@S4\endcsname{46.8}
\expandafter\def\csname v@det@GUARDinner@DWS4\endcsname{2.65}
\expandafter\def\csname v@det@GUARDinner@S5\endcsname{123.8}
\expandafter\def\csname v@det@GUARDinner@DWS5\endcsname{22.16}
\expandafter\def\csname v@det@GUARDinner@S6\endcsname{0.3}
\expandafter\def\csname v@det@GUARDinner@DWS6\endcsname{0.19}
\expandafter\def\csname v@det@GUARDinner@S7\endcsname{1.1}
\expandafter\def\csname v@det@GUARDinner@DWS7\endcsname{12.74}
\expandafter\def\csname v@det@GUARDinner@S8\endcsname{62.8}
\expandafter\def\csname v@det@GUARDinner@DWS8\endcsname{19.17}
\expandafter\def\csname v@det@GUARDinner@S9\endcsname{67.3}
\expandafter\def\csname v@det@GUARDinner@DWS9\endcsname{24.61}
\expandafter\def\csname v@det@GUARDinner@S10\endcsname{32.2}
\expandafter\def\csname v@det@GUARDinner@DWS10\endcsname{19.11}
\expandafter\def\csname v@det@GUARDboth@design\endcsname{37.3}
\expandafter\def\csname v@det@GUARDboth@eval6\endcsname{46.4}
\expandafter\def\csname v@det@GUARDboth@held\endcsname{47.1}
\expandafter\def\csname v@det@GUARDboth@S1\endcsname{22.1}
\expandafter\def\csname v@det@GUARDboth@DWS1\endcsname{0.11}
\expandafter\def\csname v@det@GUARDboth@S2\endcsname{29.4}
\expandafter\def\csname v@det@GUARDboth@DWS2\endcsname{1.03}
\expandafter\def\csname v@det@GUARDboth@S3\endcsname{37.2}
\expandafter\def\csname v@det@GUARDboth@DWS3\endcsname{0.25}
\expandafter\def\csname v@det@GUARDboth@S4\endcsname{45.2}
\expandafter\def\csname v@det@GUARDboth@DWS4\endcsname{3.28}
\expandafter\def\csname v@det@GUARDboth@S5\endcsname{114.7}
\expandafter\def\csname v@det@GUARDboth@DWS5\endcsname{22.83}
\expandafter\def\csname v@det@GUARDboth@S6\endcsname{0.4}
\expandafter\def\csname v@det@GUARDboth@DWS6\endcsname{0.32}
\expandafter\def\csname v@det@GUARDboth@S7\endcsname{1.3}
\expandafter\def\csname v@det@GUARDboth@DWS7\endcsname{12.76}
\expandafter\def\csname v@det@GUARDboth@S8\endcsname{53.6}
\expandafter\def\csname v@det@GUARDboth@DWS8\endcsname{21.15}
\expandafter\def\csname v@det@GUARDboth@S9\endcsname{59.7}
\expandafter\def\csname v@det@GUARDboth@DWS9\endcsname{26.22}
\expandafter\def\csname v@det@GUARDboth@S10\endcsname{28.2}
\expandafter\def\csname v@det@GUARDboth@DWS10\endcsname{22.75}
\expandafter\def\csname v@det@GEODOB@design\endcsname{57.0}
\expandafter\def\csname v@det@GEODOB@eval6\endcsname{154.3}
\expandafter\def\csname v@det@GEODOB@held\endcsname{217.6}
\expandafter\def\csname v@det@GEODOB@S1\endcsname{16.9}
\expandafter\def\csname v@det@GEODOB@DWS1\endcsname{0.02}
\expandafter\def\csname v@det@GEODOB@TVS1\endcsname{16}
\expandafter\def\csname v@det@GEODOB@S2\endcsname{38.6}
\expandafter\def\csname v@det@GEODOB@DWS2\endcsname{1.32}
\expandafter\def\csname v@det@GEODOB@TVS2\endcsname{239}
\expandafter\def\csname v@det@GEODOB@S3\endcsname{69.7}
\expandafter\def\csname v@det@GEODOB@DWS3\endcsname{0.10}
\expandafter\def\csname v@det@GEODOB@TVS3\endcsname{217}
\expandafter\def\csname v@det@GEODOB@S4\endcsname{62.7}
\expandafter\def\csname v@det@GEODOB@DWS4\endcsname{1.90}
\expandafter\def\csname v@det@GEODOB@TVS4\endcsname{359}
\expandafter\def\csname v@det@GEODOB@S5\endcsname{255.6}
\expandafter\def\csname v@det@GEODOB@DWS5\endcsname{15.06}
\expandafter\def\csname v@det@GEODOB@TVS5\endcsname{45583}
\expandafter\def\csname v@det@GEODOB@S6\endcsname{0.9}
\expandafter\def\csname v@det@GEODOB@DWS6\endcsname{0.07}
\expandafter\def\csname v@det@GEODOB@TVS6\endcsname{77}
\expandafter\def\csname v@det@GEODOB@S7\endcsname{1.5}
\expandafter\def\csname v@det@GEODOB@DWS7\endcsname{13.01}
\expandafter\def\csname v@det@GEODOB@TVS7\endcsname{41411}
\expandafter\def\csname v@det@GEODOB@S8\endcsname{80.7}
\expandafter\def\csname v@det@GEODOB@DWS8\endcsname{12.31}
\expandafter\def\csname v@det@GEODOB@TVS8\endcsname{38881}
\expandafter\def\csname v@det@GEODOB@S9\endcsname{111.2}
\expandafter\def\csname v@det@GEODOB@DWS9\endcsname{19.25}
\expandafter\def\csname v@det@GEODOB@TVS9\endcsname{57069}
\expandafter\def\csname v@det@GEODOB@S10\endcsname{460.8}
\expandafter\def\csname v@det@GEODOB@DWS10\endcsname{13.08}
\expandafter\def\csname v@det@GEODOB@TVS10\endcsname{40672}
\expandafter\def\csname v@det@INDI@design\endcsname{101.6}
\expandafter\def\csname v@det@INDI@eval6\endcsname{235.2}
\expandafter\def\csname v@det@INDI@held\endcsname{366.7}
\expandafter\def\csname v@det@INDI@S1\endcsname{34.4}
\expandafter\def\csname v@det@INDI@DWS1\endcsname{0.06}
\expandafter\def\csname v@det@INDI@TVS1\endcsname{42}
\expandafter\def\csname v@det@INDI@S2\endcsname{75.1}
\expandafter\def\csname v@det@INDI@DWS2\endcsname{0.57}
\expandafter\def\csname v@det@INDI@TVS2\endcsname{132}
\expandafter\def\csname v@det@INDI@S3\endcsname{122.1}
\expandafter\def\csname v@det@INDI@DWS3\endcsname{0.18}
\expandafter\def\csname v@det@INDI@TVS3\endcsname{433}
\expandafter\def\csname v@det@INDI@S4\endcsname{107.5}
\expandafter\def\csname v@det@INDI@DWS4\endcsname{0.75}
\expandafter\def\csname v@det@INDI@TVS4\endcsname{215}
\expandafter\def\csname v@det@INDI@S5\endcsname{276.6}
\expandafter\def\csname v@det@INDI@DWS5\endcsname{11.36}
\expandafter\def\csname v@det@INDI@TVS5\endcsname{35863}
\expandafter\def\csname v@det@INDI@S6\endcsname{0.3}
\expandafter\def\csname v@det@INDI@DWS6\endcsname{0.15}
\expandafter\def\csname v@det@INDI@TVS6\endcsname{208}
\expandafter\def\csname v@det@INDI@S7\endcsname{1.5}
\expandafter\def\csname v@det@INDI@DWS7\endcsname{11.79}
\expandafter\def\csname v@det@INDI@TVS7\endcsname{37447}
\expandafter\def\csname v@det@INDI@S8\endcsname{81.1}
\expandafter\def\csname v@det@INDI@DWS8\endcsname{11.12}
\expandafter\def\csname v@det@INDI@TVS8\endcsname{35364}
\expandafter\def\csname v@det@INDI@S9\endcsname{173.7}
\expandafter\def\csname v@det@INDI@DWS9\endcsname{13.77}
\expandafter\def\csname v@det@INDI@TVS9\endcsname{42737}
\expandafter\def\csname v@det@INDI@S10\endcsname{845.2}
\expandafter\def\csname v@det@INDI@DWS10\endcsname{10.33}
\expandafter\def\csname v@det@INDI@TVS10\endcsname{32469}
\expandafter\def\csname v@det@L1@design\endcsname{100.8}
\expandafter\def\csname v@det@L1@eval6\endcsname{111.3}
\expandafter\def\csname v@det@L1@held\endcsname{94.7}
\expandafter\def\csname v@det@L1@S1\endcsname{53.8}
\expandafter\def\csname v@det@L1@DWS1\endcsname{0.04}
\expandafter\def\csname v@det@L1@TVS1\endcsname{21}
\expandafter\def\csname v@det@L1@S2\endcsname{80.2}
\expandafter\def\csname v@det@L1@DWS2\endcsname{1.11}
\expandafter\def\csname v@det@L1@TVS2\endcsname{168}
\expandafter\def\csname v@det@L1@S3\endcsname{130.0}
\expandafter\def\csname v@det@L1@DWS3\endcsname{0.06}
\expandafter\def\csname v@det@L1@TVS3\endcsname{57}
\expandafter\def\csname v@det@L1@S4\endcsname{92.1}
\expandafter\def\csname v@det@L1@DWS4\endcsname{1.46}
\expandafter\def\csname v@det@L1@TVS4\endcsname{266}
\expandafter\def\csname v@det@L1@S5\endcsname{329.4}
\expandafter\def\csname v@det@L1@DWS5\endcsname{12.40}
\expandafter\def\csname v@det@L1@TVS5\endcsname{38873}
\expandafter\def\csname v@det@L1@S6\endcsname{0.6}
\expandafter\def\csname v@det@L1@DWS6\endcsname{0.11}
\expandafter\def\csname v@det@L1@TVS6\endcsname{90}
\expandafter\def\csname v@det@L1@S7\endcsname{1.5}
\expandafter\def\csname v@det@L1@DWS7\endcsname{12.99}
\expandafter\def\csname v@det@L1@TVS7\endcsname{41310}
\expandafter\def\csname v@det@L1@S8\endcsname{96.3}
\expandafter\def\csname v@det@L1@DWS8\endcsname{12.31}
\expandafter\def\csname v@det@L1@TVS8\endcsname{39186}
\expandafter\def\csname v@det@L1@S9\endcsname{119.9}
\expandafter\def\csname v@det@L1@DWS9\endcsname{14.86}
\expandafter\def\csname v@det@L1@TVS9\endcsname{46314}
\expandafter\def\csname v@det@L1@S10\endcsname{67.9}
\expandafter\def\csname v@det@L1@DWS10\endcsname{11.75}
\expandafter\def\csname v@det@L1@TVS10\endcsname{37378}
\expandafter\def\csname v@mcG1@LQR@mean\endcsname{343.1}
\expandafter\def\csname v@mcG1@LQR@med\endcsname{330.2}
\expandafter\def\csname v@mcG1@LQR@p95\endcsname{522.5}
\expandafter\def\csname v@mcG1@LQR@dw\endcsname{12.2}
\expandafter\def\csname v@mcG1@LQR@inc\endcsname{0}
\expandafter\def\csname v@mcG1@LQR@acc\endcsname{0}
\expandafter\def\csname v@mcG2@LQR@mean\endcsname{396.3}
\expandafter\def\csname v@mcG2@LQR@med\endcsname{404.1}
\expandafter\def\csname v@mcG2@LQR@p95\endcsname{559.9}
\expandafter\def\csname v@mcG2@LQR@dw\endcsname{12.3}
\expandafter\def\csname v@mcG2@LQR@inc\endcsname{0}
\expandafter\def\csname v@mcG2@LQR@acc\endcsname{0}
\expandafter\def\csname v@mcG1@MRAC@mean\endcsname{93.0}
\expandafter\def\csname v@mcG1@MRAC@med\endcsname{91.8}
\expandafter\def\csname v@mcG1@MRAC@p95\endcsname{124.1}
\expandafter\def\csname v@mcG1@MRAC@dw\endcsname{21.6}
\expandafter\def\csname v@mcG1@MRAC@inc\endcsname{0}
\expandafter\def\csname v@mcG1@MRAC@acc\endcsname{0}
\expandafter\def\csname v@mcG2@MRAC@mean\endcsname{116.6}
\expandafter\def\csname v@mcG2@MRAC@med\endcsname{111.9}
\expandafter\def\csname v@mcG2@MRAC@p95\endcsname{157.2}
\expandafter\def\csname v@mcG2@MRAC@dw\endcsname{25.1}
\expandafter\def\csname v@mcG2@MRAC@inc\endcsname{2}
\expandafter\def\csname v@mcG2@MRAC@acc\endcsname{0}
\expandafter\def\csname v@mcG1@B1@mean\endcsname{345.2}
\expandafter\def\csname v@mcG1@B1@med\endcsname{400.5}
\expandafter\def\csname v@mcG1@B1@p95\endcsname{838.4}
\expandafter\def\csname v@mcG1@B1@dw\endcsname{28.0}
\expandafter\def\csname v@mcG1@B1@inc\endcsname{43}
\expandafter\def\csname v@mcG1@B1@acc\endcsname{0}
\expandafter\def\csname v@mcG2@B1@mean\endcsname{214.3}
\expandafter\def\csname v@mcG2@B1@med\endcsname{162.4}
\expandafter\def\csname v@mcG2@B1@p95\endcsname{406.3}
\expandafter\def\csname v@mcG2@B1@dw\endcsname{18.3}
\expandafter\def\csname v@mcG2@B1@inc\endcsname{40}
\expandafter\def\csname v@mcG2@B1@acc\endcsname{0}
\expandafter\def\csname v@mcG1@NNMRAC@mean\endcsname{68.6}
\expandafter\def\csname v@mcG1@NNMRAC@med\endcsname{67.4}
\expandafter\def\csname v@mcG1@NNMRAC@p95\endcsname{84.1}
\expandafter\def\csname v@mcG1@NNMRAC@dw\endcsname{13.7}
\expandafter\def\csname v@mcG1@NNMRAC@inc\endcsname{0}
\expandafter\def\csname v@mcG1@NNMRAC@acc\endcsname{0}
\expandafter\def\csname v@mcG2@NNMRAC@mean\endcsname{86.3}
\expandafter\def\csname v@mcG2@NNMRAC@med\endcsname{84.4}
\expandafter\def\csname v@mcG2@NNMRAC@p95\endcsname{100.5}
\expandafter\def\csname v@mcG2@NNMRAC@dw\endcsname{15.0}
\expandafter\def\csname v@mcG2@NNMRAC@inc\endcsname{0}
\expandafter\def\csname v@mcG2@NNMRAC@acc\endcsname{0}
\expandafter\def\csname v@mcG1@CLucmd@mean\endcsname{75.6}
\expandafter\def\csname v@mcG1@CLucmd@med\endcsname{76.0}
\expandafter\def\csname v@mcG1@CLucmd@p95\endcsname{79.3}
\expandafter\def\csname v@mcG1@CLucmd@dw\endcsname{16.8}
\expandafter\def\csname v@mcG1@CLucmd@inc\endcsname{0}
\expandafter\def\csname v@mcG1@CLucmd@acc\endcsname{0}
\expandafter\def\csname v@mcG2@CLucmd@mean\endcsname{100.3}
\expandafter\def\csname v@mcG2@CLucmd@med\endcsname{98.1}
\expandafter\def\csname v@mcG2@CLucmd@p95\endcsname{123.5}
\expandafter\def\csname v@mcG2@CLucmd@dw\endcsname{19.6}
\expandafter\def\csname v@mcG2@CLucmd@inc\endcsname{0}
\expandafter\def\csname v@mcG2@CLucmd@acc\endcsname{0}
\expandafter\def\csname v@mcG1@CLatt@mean\endcsname{47.1}
\expandafter\def\csname v@mcG1@CLatt@med\endcsname{45.7}
\expandafter\def\csname v@mcG1@CLatt@p95\endcsname{56.9}
\expandafter\def\csname v@mcG1@CLatt@dw\endcsname{16.7}
\expandafter\def\csname v@mcG1@CLatt@inc\endcsname{0}
\expandafter\def\csname v@mcG1@CLatt@acc\endcsname{0}
\expandafter\def\csname v@mcG2@CLatt@mean\endcsname{54.8}
\expandafter\def\csname v@mcG2@CLatt@med\endcsname{53.7}
\expandafter\def\csname v@mcG2@CLatt@p95\endcsname{69.1}
\expandafter\def\csname v@mcG2@CLatt@dw\endcsname{20.0}
\expandafter\def\csname v@mcG2@CLatt@inc\endcsname{0}
\expandafter\def\csname v@mcG2@CLatt@acc\endcsname{0}
\expandafter\def\csname v@mcG1@PREDouter@mean\endcsname{47.1}
\expandafter\def\csname v@mcG1@PREDouter@med\endcsname{45.7}
\expandafter\def\csname v@mcG1@PREDouter@p95\endcsname{56.9}
\expandafter\def\csname v@mcG1@PREDouter@dw\endcsname{16.7}
\expandafter\def\csname v@mcG1@PREDouter@inc\endcsname{0}
\expandafter\def\csname v@mcG1@PREDouter@acc\endcsname{0}
\expandafter\def\csname v@mcG2@PREDouter@mean\endcsname{55.0}
\expandafter\def\csname v@mcG2@PREDouter@med\endcsname{53.9}
\expandafter\def\csname v@mcG2@PREDouter@p95\endcsname{68.8}
\expandafter\def\csname v@mcG2@PREDouter@dw\endcsname{20.0}
\expandafter\def\csname v@mcG2@PREDouter@inc\endcsname{0}
\expandafter\def\csname v@mcG2@PREDouter@acc\endcsname{0}
\expandafter\def\csname v@mcG1@PREDinner@mean\endcsname{31.2}
\expandafter\def\csname v@mcG1@PREDinner@med\endcsname{30.6}
\expandafter\def\csname v@mcG1@PREDinner@p95\endcsname{35.2}
\expandafter\def\csname v@mcG1@PREDinner@dw\endcsname{19.3}
\expandafter\def\csname v@mcG1@PREDinner@inc\endcsname{0}
\expandafter\def\csname v@mcG1@PREDinner@acc\endcsname{0}
\expandafter\def\csname v@mcG2@PREDinner@mean\endcsname{53.5}
\expandafter\def\csname v@mcG2@PREDinner@med\endcsname{48.3}
\expandafter\def\csname v@mcG2@PREDinner@p95\endcsname{121.3}
\expandafter\def\csname v@mcG2@PREDinner@dw\endcsname{24.1}
\expandafter\def\csname v@mcG2@PREDinner@inc\endcsname{0}
\expandafter\def\csname v@mcG2@PREDinner@acc\endcsname{0}
\expandafter\def\csname v@mcG1@PROPOSED@mean\endcsname{29.8}
\expandafter\def\csname v@mcG1@PROPOSED@med\endcsname{29.4}
\expandafter\def\csname v@mcG1@PROPOSED@p95\endcsname{34.0}
\expandafter\def\csname v@mcG1@PROPOSED@dw\endcsname{19.5}
\expandafter\def\csname v@mcG1@PROPOSED@inc\endcsname{0}
\expandafter\def\csname v@mcG1@PROPOSED@acc\endcsname{0}
\expandafter\def\csname v@mcG2@PROPOSED@mean\endcsname{62.4}
\expandafter\def\csname v@mcG2@PROPOSED@med\endcsname{49.0}
\expandafter\def\csname v@mcG2@PROPOSED@p95\endcsname{161.2}
\expandafter\def\csname v@mcG2@PROPOSED@dw\endcsname{24.2}
\expandafter\def\csname v@mcG2@PROPOSED@inc\endcsname{0}
\expandafter\def\csname v@mcG2@PROPOSED@acc\endcsname{0}
\expandafter\def\csname v@mcG1@GUARDnone@mean\endcsname{50.7}
\expandafter\def\csname v@mcG1@GUARDnone@med\endcsname{49.5}
\expandafter\def\csname v@mcG1@GUARDnone@p95\endcsname{61.6}
\expandafter\def\csname v@mcG1@GUARDnone@dw\endcsname{16.3}
\expandafter\def\csname v@mcG1@GUARDnone@inc\endcsname{0}
\expandafter\def\csname v@mcG1@GUARDnone@acc\endcsname{0}
\expandafter\def\csname v@mcG2@GUARDnone@mean\endcsname{57.5}
\expandafter\def\csname v@mcG2@GUARDnone@med\endcsname{55.7}
\expandafter\def\csname v@mcG2@GUARDnone@p95\endcsname{71.6}
\expandafter\def\csname v@mcG2@GUARDnone@dw\endcsname{19.2}
\expandafter\def\csname v@mcG2@GUARDnone@inc\endcsname{0}
\expandafter\def\csname v@mcG2@GUARDnone@acc\endcsname{0}
\expandafter\def\csname v@mcG1@GUARDouter@mean\endcsname{50.8}
\expandafter\def\csname v@mcG1@GUARDouter@med\endcsname{49.6}
\expandafter\def\csname v@mcG1@GUARDouter@p95\endcsname{61.5}
\expandafter\def\csname v@mcG1@GUARDouter@dw\endcsname{16.2}
\expandafter\def\csname v@mcG1@GUARDouter@inc\endcsname{0}
\expandafter\def\csname v@mcG1@GUARDouter@acc\endcsname{0}
\expandafter\def\csname v@mcG2@GUARDouter@mean\endcsname{57.7}
\expandafter\def\csname v@mcG2@GUARDouter@med\endcsname{55.9}
\expandafter\def\csname v@mcG2@GUARDouter@p95\endcsname{72.0}
\expandafter\def\csname v@mcG2@GUARDouter@dw\endcsname{19.2}
\expandafter\def\csname v@mcG2@GUARDouter@inc\endcsname{0}
\expandafter\def\csname v@mcG2@GUARDouter@acc\endcsname{0}
\expandafter\def\csname v@mcG1@GUARDinner@mean\endcsname{38.0}
\expandafter\def\csname v@mcG1@GUARDinner@med\endcsname{37.0}
\expandafter\def\csname v@mcG1@GUARDinner@p95\endcsname{44.8}
\expandafter\def\csname v@mcG1@GUARDinner@dw\endcsname{18.1}
\expandafter\def\csname v@mcG1@GUARDinner@inc\endcsname{0}
\expandafter\def\csname v@mcG1@GUARDinner@acc\endcsname{0}
\expandafter\def\csname v@mcG2@GUARDinner@mean\endcsname{49.3}
\expandafter\def\csname v@mcG2@GUARDinner@med\endcsname{48.7}
\expandafter\def\csname v@mcG2@GUARDinner@p95\endcsname{67.9}
\expandafter\def\csname v@mcG2@GUARDinner@dw\endcsname{22.4}
\expandafter\def\csname v@mcG2@GUARDinner@inc\endcsname{0}
\expandafter\def\csname v@mcG2@GUARDinner@acc\endcsname{0}
\expandafter\def\csname v@mcG1@GUARDboth@mean\endcsname{31.5}
\expandafter\def\csname v@mcG1@GUARDboth@med\endcsname{30.9}
\expandafter\def\csname v@mcG1@GUARDboth@p95\endcsname{35.4}
\expandafter\def\csname v@mcG1@GUARDboth@dw\endcsname{19.2}
\expandafter\def\csname v@mcG1@GUARDboth@inc\endcsname{0}
\expandafter\def\csname v@mcG1@GUARDboth@acc\endcsname{0}
\expandafter\def\csname v@mcG2@GUARDboth@mean\endcsname{49.8}
\expandafter\def\csname v@mcG2@GUARDboth@med\endcsname{47.6}
\expandafter\def\csname v@mcG2@GUARDboth@p95\endcsname{80.8}
\expandafter\def\csname v@mcG2@GUARDboth@dw\endcsname{23.6}
\expandafter\def\csname v@mcG2@GUARDboth@inc\endcsname{0}
\expandafter\def\csname v@mcG2@GUARDboth@acc\endcsname{0}
\expandafter\def\csname v@mcG1@GEODOB@mean\endcsname{226.9}
\expandafter\def\csname v@mcG1@GEODOB@med\endcsname{67.5}
\expandafter\def\csname v@mcG1@GEODOB@p95\endcsname{1153.6}
\expandafter\def\csname v@mcG1@GEODOB@dw\endcsname{14.5}
\expandafter\def\csname v@mcG1@GEODOB@inc\endcsname{3}
\expandafter\def\csname v@mcG1@GEODOB@acc\endcsname{0}
\expandafter\def\csname v@mcG2@GEODOB@mean\endcsname{692.2}
\expandafter\def\csname v@mcG2@GEODOB@med\endcsname{96.5}
\expandafter\def\csname v@mcG2@GEODOB@p95\endcsname{3251.0}
\expandafter\def\csname v@mcG2@GEODOB@dw\endcsname{15.1}
\expandafter\def\csname v@mcG2@GEODOB@inc\endcsname{3}
\expandafter\def\csname v@mcG2@GEODOB@acc\endcsname{0}
\expandafter\def\csname v@mcG1@INDI@mean\endcsname{134.8}
\expandafter\def\csname v@mcG1@INDI@med\endcsname{90.6}
\expandafter\def\csname v@mcG1@INDI@p95\endcsname{257.9}
\expandafter\def\csname v@mcG1@INDI@dw\endcsname{11.7}
\expandafter\def\csname v@mcG1@INDI@inc\endcsname{3}
\expandafter\def\csname v@mcG1@INDI@acc\endcsname{0}
\expandafter\def\csname v@mcG2@INDI@mean\endcsname{342.0}
\expandafter\def\csname v@mcG2@INDI@med\endcsname{146.9}
\expandafter\def\csname v@mcG2@INDI@p95\endcsname{1485.3}
\expandafter\def\csname v@mcG2@INDI@dw\endcsname{11.8}
\expandafter\def\csname v@mcG2@INDI@inc\endcsname{2}
\expandafter\def\csname v@mcG2@INDI@acc\endcsname{0}
\expandafter\def\csname v@mcG1@L1@mean\endcsname{103.7}
\expandafter\def\csname v@mcG1@L1@med\endcsname{89.7}
\expandafter\def\csname v@mcG1@L1@p95\endcsname{117.6}
\expandafter\def\csname v@mcG1@L1@dw\endcsname{13.0}
\expandafter\def\csname v@mcG1@L1@inc\endcsname{5}
\expandafter\def\csname v@mcG1@L1@acc\endcsname{0}
\expandafter\def\csname v@mcG2@L1@mean\endcsname{100.4}
\expandafter\def\csname v@mcG2@L1@med\endcsname{100.7}
\expandafter\def\csname v@mcG2@L1@p95\endcsname{127.1}
\expandafter\def\csname v@mcG2@L1@dw\endcsname{13.0}
\expandafter\def\csname v@mcG2@L1@inc\endcsname{11}
\expandafter\def\csname v@mcG2@L1@acc\endcsname{0}
\expandafter\def\csname v@pairG1@INDI@wins\endcsname{47}
\expandafter\def\csname v@pairG1@INDI@n\endcsname{47}
\expandafter\def\csname v@pairG1@INDI@diff\endcsname{-103.5}
\expandafter\def\csname v@pairG1@INDI@lo\endcsname{-171.0}
\expandafter\def\csname v@pairG1@INDI@hi\endcsname{-60.7}
\expandafter\def\csname v@pairG1@INDI@p\endcsname{1.4e-14}
\expandafter\def\csname v@pairG2@INDI@wins\endcsname{48}
\expandafter\def\csname v@pairG2@INDI@n\endcsname{48}
\expandafter\def\csname v@pairG2@INDI@diff\endcsname{-291.9}
\expandafter\def\csname v@pairG2@INDI@lo\endcsname{-427.2}
\expandafter\def\csname v@pairG2@INDI@hi\endcsname{-177.2}
\expandafter\def\csname v@pairG2@INDI@p\endcsname{7.1e-15}
\expandafter\def\csname v@pairG1@L1@wins\endcsname{45}
\expandafter\def\csname v@pairG1@L1@n\endcsname{45}
\expandafter\def\csname v@pairG1@L1@diff\endcsname{-72.5}
\expandafter\def\csname v@pairG1@L1@lo\endcsname{-98.5}
\expandafter\def\csname v@pairG1@L1@hi\endcsname{-58.0}
\expandafter\def\csname v@pairG1@L1@p\endcsname{5.7e-14}
\expandafter\def\csname v@pairG2@L1@wins\endcsname{39}
\expandafter\def\csname v@pairG2@L1@n\endcsname{39}
\expandafter\def\csname v@pairG2@L1@diff\endcsname{-54.2}
\expandafter\def\csname v@pairG2@L1@lo\endcsname{-60.5}
\expandafter\def\csname v@pairG2@L1@hi\endcsname{-49.0}
\expandafter\def\csname v@pairG2@L1@p\endcsname{3.6e-12}
\expandafter\def\csname v@pairG1@GEODOB@wins\endcsname{47}
\expandafter\def\csname v@pairG1@GEODOB@n\endcsname{47}
\expandafter\def\csname v@pairG1@GEODOB@diff\endcsname{-195.6}
\expandafter\def\csname v@pairG1@GEODOB@lo\endcsname{-343.0}
\expandafter\def\csname v@pairG1@GEODOB@hi\endcsname{-84.6}
\expandafter\def\csname v@pairG1@GEODOB@p\endcsname{1.4e-14}
\expandafter\def\csname v@pairG2@GEODOB@wins\endcsname{47}
\expandafter\def\csname v@pairG2@GEODOB@n\endcsname{47}
\expandafter\def\csname v@pairG2@GEODOB@diff\endcsname{-642.5}
\expandafter\def\csname v@pairG2@GEODOB@lo\endcsname{-985.4}
\expandafter\def\csname v@pairG2@GEODOB@hi\endcsname{-340.6}
\expandafter\def\csname v@pairG2@GEODOB@p\endcsname{1.4e-14}
\expandafter\def\csname v@pairG1@GUARDinner@wins\endcsname{50}
\expandafter\def\csname v@pairG1@GUARDinner@n\endcsname{50}
\expandafter\def\csname v@pairG1@GUARDinner@diff\endcsname{-6.6}
\expandafter\def\csname v@pairG1@GUARDinner@lo\endcsname{-7.0}
\expandafter\def\csname v@pairG1@GUARDinner@hi\endcsname{-6.1}
\expandafter\def\csname v@pairG1@GUARDinner@p\endcsname{1.8e-15}
\expandafter\def\csname v@pairG2@GUARDinner@wins\endcsname{35}
\expandafter\def\csname v@pairG2@GUARDinner@n\endcsname{50}
\expandafter\def\csname v@pairG2@GUARDinner@diff\endcsname{0.5}
\expandafter\def\csname v@pairG2@GUARDinner@lo\endcsname{-1.1}
\expandafter\def\csname v@pairG2@GUARDinner@hi\endcsname{2.6}
\expandafter\def\csname v@pairG2@GUARDinner@p\endcsname{0.051}
\expandafter\def\csname v@tune@INDI@pass\endcsname{100}
\expandafter\def\csname v@tune@INDI@J\endcsname{101.583}
\expandafter\def\csname v@tune@INDI@DWseven\endcsname{11.785}
\expandafter\def\csname v@tune@INDI@adm\endcsname{26}
\expandafter\def\csname v@tune@INDI@grid\endcsname{107}
\expandafter\def\csname v@tune@INDI@cfg\endcsname{[2 0.5 0.2]}
\expandafter\def\csname v@tune@INDI@medratio\endcsname{0.955}
\expandafter\def\csname v@tune@INDI@pairpass\endcsname{100}
\expandafter\def\csname v@tune@L1@pass\endcsname{92}
\expandafter\def\csname v@tune@L1@J\endcsname{100.765}
\expandafter\def\csname v@tune@L1@DWseven\endcsname{12.989}
\expandafter\def\csname v@tune@L1@adm\endcsname{62}
\expandafter\def\csname v@tune@L1@grid\endcsname{168}
\expandafter\def\csname v@tune@L1@cfg\endcsname{[10 5 10 1]}
\expandafter\def\csname v@tune@L1@medratio\endcsname{1.046}
\expandafter\def\csname v@tune@L1@pairpass\endcsname{100}
\expandafter\def\csname v@par@all@bothlo\endcsname{1.00}
\expandafter\def\csname v@par@all@bothhi\endcsname{1.35}
\expandafter\def\csname v@par@1p05@best\endcsname{CL-Both}
\expandafter\def\csname v@par@1p05@Jboth\endcsname{35.8}
\expandafter\def\csname v@par@1p05@Jatt\endcsname{46.2}
\expandafter\def\csname v@par@1p05@Jindi\endcsname{101.6}
\expandafter\def\csname v@par@1p05@Jinner\endcsname{37.3}
\expandafter\def\csname v@par@1p05@Jbest\endcsname{35.8}
\expandafter\def\csname v@par@1p40@best\endcsname{CL-att}
\expandafter\def\csname v@par@1p40@Jboth\endcsname{35.8}
\expandafter\def\csname v@par@1p40@Jatt\endcsname{35.5}
\expandafter\def\csname v@par@1p40@Jindi\endcsname{59.1}
\expandafter\def\csname v@par@1p40@Jinner\endcsname{35.9}
\expandafter\def\csname v@par@1p40@Jbest\endcsname{35.5}
\expandafter\def\csname v@par@1p50@best\endcsname{CL-att}
\expandafter\def\csname v@par@1p50@Jboth\endcsname{35.8}
\expandafter\def\csname v@par@1p50@Jatt\endcsname{34.2}
\expandafter\def\csname v@par@1p50@Jindi\endcsname{59.1}
\expandafter\def\csname v@par@1p50@Jinner\endcsname{35.9}
\expandafter\def\csname v@par@1p50@Jbest\endcsname{34.2}
\expandafter\def\csname v@par@2p00@best\endcsname{GEO-DOB}
\expandafter\def\csname v@par@2p00@Jboth\endcsname{35.8}
\expandafter\def\csname v@par@2p00@Jatt\endcsname{34.2}
\expandafter\def\csname v@par@2p00@Jindi\endcsname{51.4}
\expandafter\def\csname v@par@2p00@Jinner\endcsname{35.9}
\expandafter\def\csname v@par@2p00@Jbest\endcsname{31.3}
\expandafter\def\csname v@par@all@lqrflight\endcsname{0.85}
\expandafter\def\csname v@flt@1p2@MRAC\endcsname{150.3}
\expandafter\def\csname v@flt@1p2@MRACS7\endcsname{1.00}
\expandafter\def\csname v@flt@1p2@NNMRAC\endcsname{134.9}
\expandafter\def\csname v@flt@1p2@NNMRACS7\endcsname{1.00}
\expandafter\def\csname v@flt@1p2@CLatt\endcsname{65.0}
\expandafter\def\csname v@flt@1p2@CLattS7\endcsname{1.00}
\expandafter\def\csname v@flt@1p2@CLOuter\endcsname{71.2}
\expandafter\def\csname v@flt@1p2@CLOuterS7\endcsname{1.00}
\expandafter\def\csname v@flt@1p2@CLInner\endcsname{60.0}
\expandafter\def\csname v@flt@1p2@CLInnerS7\endcsname{1.00}
\expandafter\def\csname v@flt@1p2@CLBoth\endcsname{60.0}
\expandafter\def\csname v@flt@1p2@CLBothS7\endcsname{1.00}
\expandafter\def\csname v@flt@1p2@GEODOB\endcsname{39.9}
\expandafter\def\csname v@flt@1p2@GEODOBS7\endcsname{1.86}
\expandafter\def\csname v@flt@1p2@INDI\endcsname{26.6}
\expandafter\def\csname v@flt@1p2@INDIS7\endcsname{13.30}
\expandafter\def\csname v@flt@1p2@L1\endcsname{78.7}
\expandafter\def\csname v@flt@1p2@L1S7\endcsname{2.63}
\expandafter\def\csname v@flt@1p2@best\endcsname{INDI}
\expandafter\def\csname v@flt@1p5@MRAC\endcsname{118.5}
\expandafter\def\csname v@flt@1p5@MRACS7\endcsname{1.00}
\expandafter\def\csname v@flt@1p5@NNMRAC\endcsname{82.6}
\expandafter\def\csname v@flt@1p5@NNMRACS7\endcsname{1.01}
\expandafter\def\csname v@flt@1p5@CLucmd\endcsname{84.8}
\expandafter\def\csname v@flt@1p5@CLucmdS7\endcsname{1.01}
\expandafter\def\csname v@flt@1p5@CLatt\endcsname{44.4}
\expandafter\def\csname v@flt@1p5@CLattS7\endcsname{1.09}
\expandafter\def\csname v@flt@1p5@CLOuter\endcsname{44.3}
\expandafter\def\csname v@flt@1p5@CLOuterS7\endcsname{1.08}
\expandafter\def\csname v@flt@1p5@CLInner\endcsname{43.6}
\expandafter\def\csname v@flt@1p5@CLInnerS7\endcsname{1.02}
\expandafter\def\csname v@flt@1p5@CLBoth\endcsname{43.5}
\expandafter\def\csname v@flt@1p5@CLBothS7\endcsname{1.02}
\expandafter\def\csname v@flt@1p5@GEODOB\endcsname{31.3}
\expandafter\def\csname v@flt@1p5@GEODOBS7\endcsname{1.96}
\expandafter\def\csname v@flt@1p5@INDI\endcsname{26.6}
\expandafter\def\csname v@flt@1p5@INDIS7\endcsname{13.30}
\expandafter\def\csname v@flt@1p5@L1\endcsname{78.7}
\expandafter\def\csname v@flt@1p5@L1S7\endcsname{2.63}
\expandafter\def\csname v@flt@1p5@best\endcsname{INDI}
\expandafter\def\csname v@flt@2p0@MRAC\endcsname{91.5}
\expandafter\def\csname v@flt@2p0@MRACS7\endcsname{1.01}
\expandafter\def\csname v@flt@2p0@NNMRAC\endcsname{82.6}
\expandafter\def\csname v@flt@2p0@NNMRACS7\endcsname{1.01}
\expandafter\def\csname v@flt@2p0@CLucmd\endcsname{77.8}
\expandafter\def\csname v@flt@2p0@CLucmdS7\endcsname{1.02}
\expandafter\def\csname v@flt@2p0@CLatt\endcsname{37.3}
\expandafter\def\csname v@flt@2p0@CLattS7\endcsname{1.29}
\expandafter\def\csname v@flt@2p0@CLOuter\endcsname{37.4}
\expandafter\def\csname v@flt@2p0@CLOuterS7\endcsname{1.28}
\expandafter\def\csname v@flt@2p0@CLInner\endcsname{35.9}
\expandafter\def\csname v@flt@2p0@CLInnerS7\endcsname{1.06}
\expandafter\def\csname v@flt@2p0@CLBoth\endcsname{35.8}
\expandafter\def\csname v@flt@2p0@CLBothS7\endcsname{1.05}
\expandafter\def\csname v@flt@2p0@GEODOB\endcsname{27.8}
\expandafter\def\csname v@flt@2p0@GEODOBS7\endcsname{2.07}
\expandafter\def\csname v@flt@2p0@INDI\endcsname{26.6}
\expandafter\def\csname v@flt@2p0@INDIS7\endcsname{13.30}
\expandafter\def\csname v@flt@2p0@L1\endcsname{78.7}
\expandafter\def\csname v@flt@2p0@L1S7\endcsname{2.63}
\expandafter\def\csname v@flt@2p0@best\endcsname{INDI}
\expandafter\def\csname v@dual@all@nnflight\endcsname{1.25}
\expandafter\def\csname v@dual@all@lqrflight12\endcsname{1.02}
\expandafter\def\csname v@dual@MRAC@singleJ\endcsname{86.5}
\expandafter\def\csname v@dual@MRAC@singleF\endcsname{2.40}
\expandafter\def\csname v@dual@MRAC@nnJ\endcsname{118.5}
\expandafter\def\csname v@dual@MRAC@nnF\endcsname{1.06}
\expandafter\def\csname v@dual@MRAC@lqr12J\endcsname{150.3}
\expandafter\def\csname v@dual@MRAC@lqr12F\endcsname{0.96}
\expandafter\def\csname v@dual@NNMRAC@singleJ\endcsname{82.6}
\expandafter\def\csname v@dual@NNMRAC@singleF\endcsname{1.25}
\expandafter\def\csname v@dual@NNMRAC@nnJ\endcsname{82.6}
\expandafter\def\csname v@dual@NNMRAC@nnF\endcsname{1.25}
\expandafter\def\csname v@dual@NNMRAC@lqr12J\endcsname{134.9}
\expandafter\def\csname v@dual@NNMRAC@lqr12F\endcsname{0.94}
\expandafter\def\csname v@dual@CLucmd@singleJ\endcsname{77.8}
\expandafter\def\csname v@dual@CLucmd@singleF\endcsname{1.42}
\expandafter\def\csname v@dual@CLucmd@nnJ\endcsname{84.8}
\expandafter\def\csname v@dual@CLucmd@nnF\endcsname{1.24}
\expandafter\def\csname v@dual@CLatt@singleJ\endcsname{46.2}
\expandafter\def\csname v@dual@CLatt@singleF\endcsname{1.26}
\expandafter\def\csname v@dual@CLatt@nnJ\endcsname{49.6}
\expandafter\def\csname v@dual@CLatt@nnF\endcsname{1.13}
\expandafter\def\csname v@dual@CLatt@lqr12J\endcsname{65.0}
\expandafter\def\csname v@dual@CLatt@lqr12F\endcsname{1.02}
\expandafter\def\csname v@dual@CLOuter@singleJ\endcsname{46.2}
\expandafter\def\csname v@dual@CLOuter@singleF\endcsname{1.27}
\expandafter\def\csname v@dual@CLOuter@nnJ\endcsname{49.6}
\expandafter\def\csname v@dual@CLOuter@nnF\endcsname{1.14}
\expandafter\def\csname v@dual@CLOuter@lqr12J\endcsname{71.2}
\expandafter\def\csname v@dual@CLOuter@lqr12F\endcsname{0.99}
\expandafter\def\csname v@dual@CLInner@singleJ\endcsname{37.3}
\expandafter\def\csname v@dual@CLInner@singleF\endcsname{1.51}
\expandafter\def\csname v@dual@CLInner@nnJ\endcsname{43.6}
\expandafter\def\csname v@dual@CLInner@nnF\endcsname{1.18}
\expandafter\def\csname v@dual@CLInner@lqr12J\endcsname{60.0}
\expandafter\def\csname v@dual@CLInner@lqr12F\endcsname{0.98}
\expandafter\def\csname v@dual@CLBoth@singleJ\endcsname{35.8}
\expandafter\def\csname v@dual@CLBoth@singleF\endcsname{1.60}
\expandafter\def\csname v@dual@CLBoth@nnJ\endcsname{43.5}
\expandafter\def\csname v@dual@CLBoth@nnF\endcsname{1.19}
\expandafter\def\csname v@dual@CLBoth@lqr12J\endcsname{60.0}
\expandafter\def\csname v@dual@CLBoth@lqr12F\endcsname{0.98}
\expandafter\def\csname v@dual@GEODOB@singleJ\endcsname{57.0}
\expandafter\def\csname v@dual@GEODOB@singleF\endcsname{1.11}
\expandafter\def\csname v@dual@GEODOB@nnJ\endcsname{57.0}
\expandafter\def\csname v@dual@GEODOB@nnF\endcsname{1.11}
\expandafter\def\csname v@dual@GEODOB@lqr12J\endcsname{69.6}
\expandafter\def\csname v@dual@GEODOB@lqr12F\endcsname{0.70}
\expandafter\def\csname v@dual@INDI@singleJ\endcsname{101.6}
\expandafter\def\csname v@dual@INDI@singleF\endcsname{0.50}
\expandafter\def\csname v@dual@INDI@nnJ\endcsname{101.6}
\expandafter\def\csname v@dual@INDI@nnF\endcsname{0.50}
\expandafter\def\csname v@dual@INDI@lqr12J\endcsname{101.6}
\expandafter\def\csname v@dual@INDI@lqr12F\endcsname{0.50}
\expandafter\def\csname v@dual@L1@singleJ\endcsname{100.8}
\expandafter\def\csname v@dual@L1@singleF\endcsname{0.88}
\expandafter\def\csname v@dual@L1@nnJ\endcsname{100.8}
\expandafter\def\csname v@dual@L1@nnF\endcsname{0.88}
\expandafter\def\csname v@dual@L1@lqr12J\endcsname{100.8}
\expandafter\def\csname v@dual@L1@lqr12F\endcsname{0.88}
\expandafter\def\csname v@exc@GUARDnoneS2@MedRankQo\endcsname{3}
\expandafter\def\csname v@exc@GUARDnoneS2@MaxRankQo\endcsname{4}
\expandafter\def\csname v@exc@GUARDnoneS2@MedRankQi\endcsname{3}
\expandafter\def\csname v@exc@GUARDnoneS2@MaxRankQi\endcsname{4}
\expandafter\def\csname v@exc@GUARDnoneS2@MedLamQo\endcsname{1.2e-13}
\expandafter\def\csname v@exc@GUARDnoneS2@MedLamQi\endcsname{3.7e-15}
\expandafter\def\csname v@exc@GUARDnoneS2@MaxLamQo\endcsname{1.8e-11}
\expandafter\def\csname v@exc@GUARDnoneS2@MaxLamQi\endcsname{3.2e-13}
\expandafter\def\csname v@exc@GUARDnoneS2@MedDWo\endcsname{0.33}
\expandafter\def\csname v@exc@GUARDnoneS2@MedDWi\endcsname{0.79}
\expandafter\def\csname v@exc@GUARDnoneS2@MaxDWo\endcsname{0.8}
\expandafter\def\csname v@exc@GUARDnoneS2@MaxDWi\endcsname{6.6}
\expandafter\def\csname v@exc@GUARDnoneS4@MedRankQo\endcsname{3}
\expandafter\def\csname v@exc@GUARDnoneS4@MaxRankQo\endcsname{4}
\expandafter\def\csname v@exc@GUARDnoneS4@MedRankQi\endcsname{3}
\expandafter\def\csname v@exc@GUARDnoneS4@MaxRankQi\endcsname{6}
\expandafter\def\csname v@exc@GUARDnoneS4@MedLamQo\endcsname{2.5e-12}
\expandafter\def\csname v@exc@GUARDnoneS4@MedLamQi\endcsname{1.1e-13}
\expandafter\def\csname v@exc@GUARDnoneS4@MaxLamQo\endcsname{5.2e-11}
\expandafter\def\csname v@exc@GUARDnoneS4@MaxLamQi\endcsname{3.5e-12}
\expandafter\def\csname v@exc@GUARDnoneS4@MedDWo\endcsname{0.57}
\expandafter\def\csname v@exc@GUARDnoneS4@MedDWi\endcsname{4.07}
\expandafter\def\csname v@exc@GUARDnoneS4@MaxDWo\endcsname{1.9}
\expandafter\def\csname v@exc@GUARDnoneS4@MaxDWi\endcsname{42.6}
\expandafter\def\csname v@exc@GUARDinnerS2@MedRankQo\endcsname{3}
\expandafter\def\csname v@exc@GUARDinnerS2@MaxRankQo\endcsname{4}
\expandafter\def\csname v@exc@GUARDinnerS2@MedRankQi\endcsname{3}
\expandafter\def\csname v@exc@GUARDinnerS2@MaxRankQi\endcsname{5}
\expandafter\def\csname v@exc@GUARDinnerS2@MedLamQo\endcsname{8.7e-14}
\expandafter\def\csname v@exc@GUARDinnerS2@MedLamQi\endcsname{2.1e-14}
\expandafter\def\csname v@exc@GUARDinnerS2@MaxLamQo\endcsname{1.9e-11}
\expandafter\def\csname v@exc@GUARDinnerS2@MaxLamQi\endcsname{8.4e-13}
\expandafter\def\csname v@exc@GUARDinnerS2@MedDWo\endcsname{0.51}
\expandafter\def\csname v@exc@GUARDinnerS2@MedDWi\endcsname{0.44}
\expandafter\def\csname v@exc@GUARDinnerS2@MaxDWo\endcsname{1.8}
\expandafter\def\csname v@exc@GUARDinnerS2@MaxDWi\endcsname{2.0}
\expandafter\def\csname v@exc@GUARDinnerS4@MedRankQo\endcsname{3}
\expandafter\def\csname v@exc@GUARDinnerS4@MaxRankQo\endcsname{5}
\expandafter\def\csname v@exc@GUARDinnerS4@MedRankQi\endcsname{4}
\expandafter\def\csname v@exc@GUARDinnerS4@MaxRankQi\endcsname{7}
\expandafter\def\csname v@exc@GUARDinnerS4@MedLamQo\endcsname{2.1e-12}
\expandafter\def\csname v@exc@GUARDinnerS4@MedLamQi\endcsname{6.9e-13}
\expandafter\def\csname v@exc@GUARDinnerS4@MaxLamQo\endcsname{1.2e-10}
\expandafter\def\csname v@exc@GUARDinnerS4@MaxLamQi\endcsname{2.4e-10}
\expandafter\def\csname v@exc@GUARDinnerS4@MedDWo\endcsname{1.09}
\expandafter\def\csname v@exc@GUARDinnerS4@MedDWi\endcsname{8.14}
\expandafter\def\csname v@exc@GUARDinnerS4@MaxDWo\endcsname{4.3}
\expandafter\def\csname v@exc@GUARDinnerS4@MaxDWi\endcsname{46.0}
\expandafter\def\csname v@exc@GUARDbothS2@MedRankQo\endcsname{3}
\expandafter\def\csname v@exc@GUARDbothS2@MaxRankQo\endcsname{4}
\expandafter\def\csname v@exc@GUARDbothS2@MedRankQi\endcsname{3}
\expandafter\def\csname v@exc@GUARDbothS2@MaxRankQi\endcsname{5}
\expandafter\def\csname v@exc@GUARDbothS2@MedLamQo\endcsname{8.7e-14}
\expandafter\def\csname v@exc@GUARDbothS2@MedLamQi\endcsname{1.0e-13}
\expandafter\def\csname v@exc@GUARDbothS2@MaxLamQo\endcsname{2.1e-11}
\expandafter\def\csname v@exc@GUARDbothS2@MaxLamQi\endcsname{3.6e-12}
\expandafter\def\csname v@exc@GUARDbothS2@MedDWo\endcsname{0.64}
\expandafter\def\csname v@exc@GUARDbothS2@MedDWi\endcsname{0.91}
\expandafter\def\csname v@exc@GUARDbothS2@MaxDWo\endcsname{3.8}
\expandafter\def\csname v@exc@GUARDbothS2@MaxDWi\endcsname{4.6}
\expandafter\def\csname v@exc@GUARDbothS4@MedRankQo\endcsname{3}
\expandafter\def\csname v@exc@GUARDbothS4@MaxRankQo\endcsname{5}
\expandafter\def\csname v@exc@GUARDbothS4@MedRankQi\endcsname{4}
\expandafter\def\csname v@exc@GUARDbothS4@MaxRankQi\endcsname{8}
\expandafter\def\csname v@exc@GUARDbothS4@MedLamQo\endcsname{2.9e-12}
\expandafter\def\csname v@exc@GUARDbothS4@MedLamQi\endcsname{7.8e-12}
\expandafter\def\csname v@exc@GUARDbothS4@MaxLamQo\endcsname{1.3\times10^{-10}}
\expandafter\def\csname v@exc@GUARDbothS4@MaxLamQi\endcsname{5.8e-09}
\expandafter\def\csname v@exc@GUARDbothS4@MedDWo\endcsname{1.89}
\expandafter\def\csname v@exc@GUARDbothS4@MedDWi\endcsname{17.51}
\expandafter\def\csname v@exc@GUARDbothS4@MaxDWo\endcsname{7.4}
\expandafter\def\csname v@exc@GUARDbothS4@MaxDWi\endcsname{61.1}
\expandafter\def\csname v@lin@all@rhomax\endcsname{0.99875}
\expandafter\def\csname v@lin@all@nunit\endcsname{93}
\expandafter\def\csname v@lin@Ts1@rho\endcsname{0.99875}
\expandafter\def\csname v@lin@Ts1@rate\endcsname{1.25}
\expandafter\def\csname v@lin@Ts1@rhofrozen\endcsname{0.99859}
\expandafter\def\csname v@lin@Ts1@ratefrozen\endcsname{1.42}
\expandafter\def\csname v@lin@Ts2@rho\endcsname{0.99750}
\expandafter\def\csname v@lin@Ts2@rate\endcsname{1.25}
\expandafter\def\csname v@lin@Ts2@rhofrozen\endcsname{0.99717}
\expandafter\def\csname v@lin@Ts2@ratefrozen\endcsname{1.42}
\expandafter\def\csname v@lin@Ts4@rho\endcsname{0.99500}
\expandafter\def\csname v@lin@Ts4@rate\endcsname{1.25}
\expandafter\def\csname v@lin@Ts4@rhofrozen\endcsname{0.99436}
\expandafter\def\csname v@lin@Ts4@ratefrozen\endcsname{1.42}
\expandafter\def\csname v@lin@all@wnorm\endcsname{60.2}
\expandafter\def\csname v@rIE@b@LPF\endcsname{35.60}
\expandafter\def\csname v@rIE@b@Both\endcsname{35.76}
\expandafter\def\csname v@rIE@b@att\endcsname{46.15}
\expandafter\def\csname v@rIE@b@gap\endcsname{0.16}
\expandafter\def\csname v@rIE@b@LPFhi\endcsname{35.05}
\expandafter\def\csname v@rIE@b@Bothhi\endcsname{35.76}
\expandafter\def\csname v@rIE@b@atthi\endcsname{39.85}
\expandafter\def\csname v@rIE@b@tau\endcsname{20}
\expandafter\def\csname v@rIE@b@go\endcsname{2560}
\expandafter\def\csname v@rIE@tau5@J\endcsname{45.8}
\expandafter\def\csname v@rIE@tau5@go\endcsname{160}
\expandafter\def\csname v@rIE@tau10@J\endcsname{45.4}
\expandafter\def\csname v@rIE@tau10@go\endcsname{160}
\expandafter\def\csname v@rIE@tau20@J\endcsname{35.6}
\expandafter\def\csname v@rIE@tau20@go\endcsname{2560}
\expandafter\def\csname v@rIE@tau40@J\endcsname{39.5}
\expandafter\def\csname v@rIE@tau40@go\endcsname{1280}
\expandafter\def\csname v@rIE@tau60@J\endcsname{43.8}
\expandafter\def\csname v@rIE@tau60@go\endcsname{640}
\expandafter\def\csname v@rIE@tau80@J\endcsname{48.6}
\expandafter\def\csname v@rIE@tau80@go\endcsname{160}
\expandafter\def\csname v@rIE@t20g160@dJ\endcsname{1.15}
\expandafter\def\csname v@rIE@t20g160@dD\endcsname{-0.00}
\expandafter\def\csname v@rIE@t20g160@Jatt\endcsname{46.15}
\expandafter\def\csname v@rIE@t20g160@Jboth\endcsname{45.00}
\expandafter\def\csname v@rIE@t20g160@lagiatt\endcsname{1.67}
\expandafter\def\csname v@rIE@t20g160@lagiboth\endcsname{0.03}
\expandafter\def\csname v@rIE@t20g640@dJ\endcsname{0.43}
\expandafter\def\csname v@rIE@t20g640@dD\endcsname{-0.07}
\expandafter\def\csname v@rIE@t20g640@Jatt\endcsname{39.85}
\expandafter\def\csname v@rIE@t20g640@Jboth\endcsname{39.42}
\expandafter\def\csname v@rIE@t20g640@lagiatt\endcsname{2.02}
\expandafter\def\csname v@rIE@t20g640@lagiboth\endcsname{0.03}
\expandafter\def\csname v@rIE@t20g2560@dJ\endcsname{-0.25}
\expandafter\def\csname v@rIE@t20g2560@dD\endcsname{-0.12}
\expandafter\def\csname v@rIE@t20g2560@Jatt\endcsname{35.51}
\expandafter\def\csname v@rIE@t20g2560@Jboth\endcsname{35.76}
\expandafter\def\csname v@rIE@t20g2560@lagiatt\endcsname{2.92}
\expandafter\def\csname v@rIE@t20g2560@lagiboth\endcsname{0.04}
\expandafter\def\csname v@rIE@t60g160@dJ\endcsname{3.36}
\expandafter\def\csname v@rIE@t60g160@dD\endcsname{0.04}
\expandafter\def\csname v@rIE@t60g160@Jatt\endcsname{49.23}
\expandafter\def\csname v@rIE@t60g160@Jboth\endcsname{45.87}
\expandafter\def\csname v@rIE@t60g160@lagiatt\endcsname{7.12}
\expandafter\def\csname v@rIE@t60g160@lagiboth\endcsname{2.75}
\expandafter\def\csname v@rIE@t60g640@dJ\endcsname{2.29}
\expandafter\def\csname v@rIE@t60g640@dD\endcsname{0.03}
\expandafter\def\csname v@rIE@t60g640@Jatt\endcsname{42.28}
\expandafter\def\csname v@rIE@t60g640@Jboth\endcsname{39.99}
\expandafter\def\csname v@rIE@t60g640@lagiatt\endcsname{8.32}
\expandafter\def\csname v@rIE@t60g640@lagiboth\endcsname{3.35}
\expandafter\def\csname v@rIE@t60g2560@dJ\endcsname{1.56}
\expandafter\def\csname v@rIE@t60g2560@dD\endcsname{0.18}
\expandafter\def\csname v@rIE@t60g2560@Jatt\endcsname{38.16}
\expandafter\def\csname v@rIE@t60g2560@Jboth\endcsname{36.59}
\expandafter\def\csname v@rIE@t60g2560@lagiatt\endcsname{11.31}
\expandafter\def\csname v@rIE@t60g2560@lagiboth\endcsname{4.59}
\expandafter\def\csname v@rIE@t100g160@dJ\endcsname{2.80}
\expandafter\def\csname v@rIE@t100g160@dD\endcsname{0.10}
\expandafter\def\csname v@rIE@t100g160@Jatt\endcsname{52.66}
\expandafter\def\csname v@rIE@t100g160@Jboth\endcsname{49.86}
\expandafter\def\csname v@rIE@t100g160@lagiatt\endcsname{15.17}
\expandafter\def\csname v@rIE@t100g160@lagiboth\endcsname{8.78}
\expandafter\def\csname v@rIE@t100g640@dJ\endcsname{diverged}
\expandafter\def\csname v@rIE@t100g640@dD\endcsname{0.28}
\expandafter\def\csname v@rIE@t100g640@Jatt\endcsname{46.47}
\expandafter\def\csname v@rIE@t100g640@Jboth\endcsname{diverged}
\expandafter\def\csname v@rIE@t100g640@lagiatt\endcsname{17.88}
\expandafter\def\csname v@rIE@t100g640@lagiboth\endcsname{9.10}
\expandafter\def\csname v@rIE@t100g2560@dJ\endcsname{diverged}
\expandafter\def\csname v@rIE@t100g2560@dD\endcsname{1.82}
\expandafter\def\csname v@rIE@t100g2560@Jatt\endcsname{91.33}
\expandafter\def\csname v@rIE@t100g2560@Jboth\endcsname{diverged}
\expandafter\def\csname v@rIE@t100g2560@lagiatt\endcsname{30.21}
\expandafter\def\csname v@rIE@t100g2560@lagiboth\endcsname{21.81}
\expandafter\def\csname v@rIE@c20@J\endcsname{62.14}
\expandafter\def\csname v@rIE@c30@J\endcsname{53.75}
\expandafter\def\csname v@rIE@c40@J\endcsname{48.75}
\expandafter\def\csname v@rIE@c50@J\endcsname{45.31}
\expandafter\def\csname v@rIE@c60@J\endcsname{61.34}
\expandafter\def\csname v@rIE@c80@J\endcsname{93.16}
\expandafter\def\csname v@rIE@c@optratio\endcsname{0.83}
\expandafter\def\csname v@rIE@c@optJ\endcsname{45.31}
\expandafter\def\csname v@rIE@c@optms\endcsname{50}
\expandafter\def\csname v@rIE@g@go\endcsname{1280}
\expandafter\def\csname v@rIE@g640@bound\endcsname{12.82}
\expandafter\def\csname v@rIE@g1280@bound\endcsname{12.96}
\expandafter\def\csname v@rIE@g2560@bound\endcsname{13.16}
\expandafter\def\csname v@rIE@v@pass\endcsname{100}
\expandafter\def\csname v@rIE@v@N\endcsname{100}
\expandafter\def\csname v@rIE@v@paired\endcsname{100}
\expandafter\def\csname v@rIE@v@cilo\endcsname{96.38}
\expandafter\def\csname v@rIE@bench@design\endcsname{37.2}
\expandafter\def\csname v@rIE@bench@eval6\endcsname{45.6}
\expandafter\def\csname v@rIIE@b1m1@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b1m1@J\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1m1@CLLPF\endcsname{73.2}
\expandafter\def\csname v@rIIE@b1m1@GEODOB\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1m1@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1m1p2@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1m1p2@J\endcsname{48.5}
\expandafter\def\csname v@rIIE@b1m1p2@CLBoth\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1m1p2@CLLPF\endcsname{48.5}
\expandafter\def\csname v@rIIE@b1m1p2@GEODOB\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1m1p2@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1m1p2@CLInner\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1m1p5@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1m1p5@J\endcsname{42.9}
\expandafter\def\csname v@rIIE@b1m1p5@CLBoth\endcsname{53.4}
\expandafter\def\csname v@rIIE@b1m1p5@CLLPF\endcsname{42.9}
\expandafter\def\csname v@rIIE@b1m1p5@GEODOB\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1m1p5@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1m1p5@CLInner\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1m2@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1m2@J\endcsname{39.5}
\expandafter\def\csname v@rIIE@b1m2@CLBoth\endcsname{49.7}
\expandafter\def\csname v@rIIE@b1m2@CLLPF\endcsname{39.5}
\expandafter\def\csname v@rIIE@b1m2@GEODOB\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1m2@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1m2@CLInner\endcsname{51.0}
\expandafter\def\csname v@rIIE@b1minf@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1minf@J\endcsname{39.5}
\expandafter\def\csname v@rIIE@b1minf@CLBoth\endcsname{49.7}
\expandafter\def\csname v@rIIE@b1minf@CLLPF\endcsname{39.5}
\expandafter\def\csname v@rIIE@b1minf@GEODOB\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1minf@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1minf@CLInner\endcsname{51.0}
\expandafter\def\csname v@rIIE@b1p05m1@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b1p05m1@J\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1p05m1@CLLPF\endcsname{73.2}
\expandafter\def\csname v@rIIE@b1p05m1@GEODOB\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1p05m1@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1p05m1p2@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p05m1p2@J\endcsname{48.5}
\expandafter\def\csname v@rIIE@b1p05m1p2@CLBoth\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1p05m1p2@CLLPF\endcsname{48.5}
\expandafter\def\csname v@rIIE@b1p05m1p2@GEODOB\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1p05m1p2@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1p05m1p2@CLatt\endcsname{65.0}
\expandafter\def\csname v@rIIE@b1p05m1p2@CLInner\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1p05m1p5@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p05m1p5@J\endcsname{42.9}
\expandafter\def\csname v@rIIE@b1p05m1p5@CLBoth\endcsname{43.5}
\expandafter\def\csname v@rIIE@b1p05m1p5@CLLPF\endcsname{42.9}
\expandafter\def\csname v@rIIE@b1p05m1p5@GEODOB\endcsname{57.0}
\expandafter\def\csname v@rIIE@b1p05m1p5@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1p05m1p5@CLatt\endcsname{46.2}
\expandafter\def\csname v@rIIE@b1p05m1p5@CLInner\endcsname{43.6}
\expandafter\def\csname v@rIIE@b1p05m2@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p05m2@J\endcsname{35.6}
\expandafter\def\csname v@rIIE@b1p05m2@CLBoth\endcsname{35.8}
\expandafter\def\csname v@rIIE@b1p05m2@CLLPF\endcsname{35.6}
\expandafter\def\csname v@rIIE@b1p05m2@GEODOB\endcsname{57.0}
\expandafter\def\csname v@rIIE@b1p05m2@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1p05m2@CLatt\endcsname{46.2}
\expandafter\def\csname v@rIIE@b1p05m2@CLInner\endcsname{37.3}
\expandafter\def\csname v@rIIE@b1p05minf@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p05minf@J\endcsname{35.6}
\expandafter\def\csname v@rIIE@b1p05minf@CLBoth\endcsname{35.8}
\expandafter\def\csname v@rIIE@b1p05minf@CLLPF\endcsname{35.6}
\expandafter\def\csname v@rIIE@b1p05minf@GEODOB\endcsname{57.0}
\expandafter\def\csname v@rIIE@b1p05minf@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1p05minf@CLatt\endcsname{46.2}
\expandafter\def\csname v@rIIE@b1p05minf@CLInner\endcsname{37.3}
\expandafter\def\csname v@rIIE@b1p15m1@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b1p15m1@J\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1p15m1@CLLPF\endcsname{73.2}
\expandafter\def\csname v@rIIE@b1p15m1@GEODOB\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1p15m1@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1p15m1p2@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p15m1p2@J\endcsname{48.5}
\expandafter\def\csname v@rIIE@b1p15m1p2@CLBoth\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1p15m1p2@CLLPF\endcsname{48.5}
\expandafter\def\csname v@rIIE@b1p15m1p2@GEODOB\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1p15m1p2@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1p15m1p2@CLatt\endcsname{65.0}
\expandafter\def\csname v@rIIE@b1p15m1p2@CLInner\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1p15m1p5@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p15m1p5@J\endcsname{42.9}
\expandafter\def\csname v@rIIE@b1p15m1p5@CLBoth\endcsname{43.5}
\expandafter\def\csname v@rIIE@b1p15m1p5@CLLPF\endcsname{42.9}
\expandafter\def\csname v@rIIE@b1p15m1p5@GEODOB\endcsname{57.0}
\expandafter\def\csname v@rIIE@b1p15m1p5@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1p15m1p5@CLatt\endcsname{44.4}
\expandafter\def\csname v@rIIE@b1p15m1p5@CLInner\endcsname{43.6}
\expandafter\def\csname v@rIIE@b1p15m2@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p15m2@J\endcsname{35.6}
\expandafter\def\csname v@rIIE@b1p15m2@CLBoth\endcsname{35.8}
\expandafter\def\csname v@rIIE@b1p15m2@CLLPF\endcsname{35.6}
\expandafter\def\csname v@rIIE@b1p15m2@GEODOB\endcsname{57.0}
\expandafter\def\csname v@rIIE@b1p15m2@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1p15m2@CLatt\endcsname{41.1}
\expandafter\def\csname v@rIIE@b1p15m2@CLInner\endcsname{35.9}
\expandafter\def\csname v@rIIE@b1p15minf@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p15minf@J\endcsname{35.4}
\expandafter\def\csname v@rIIE@b1p15minf@CLBoth\endcsname{35.8}
\expandafter\def\csname v@rIIE@b1p15minf@CLLPF\endcsname{35.4}
\expandafter\def\csname v@rIIE@b1p15minf@GEODOB\endcsname{57.0}
\expandafter\def\csname v@rIIE@b1p15minf@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1p15minf@CLatt\endcsname{41.1}
\expandafter\def\csname v@rIIE@b1p15minf@CLInner\endcsname{35.9}
\expandafter\def\csname v@rIIE@b1p25m1@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b1p25m1@J\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1p25m1@CLLPF\endcsname{73.2}
\expandafter\def\csname v@rIIE@b1p25m1@GEODOB\endcsname{69.6}
\expandafter\def\csname v@rIIE@b1p25m1@INDI\endcsname{101.6}
\expandafter\def\csname v@rIIE@b1p25m1p2@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p25m1p2@J\endcsname{48.5}
\expandafter\def\csname v@rIIE@b1p25m1p2@CLBoth\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1p25m1p2@CLLPF\endcsname{48.5}
\expandafter\def\csname v@rIIE@b1p25m1p2@GEODOB\endcsname{59.1}
\expandafter\def\csname v@rIIE@b1p25m1p2@INDI\endcsname{71.9}
\expandafter\def\csname v@rIIE@b1p25m1p2@CLatt\endcsname{65.0}
\expandafter\def\csname v@rIIE@b1p25m1p2@CLInner\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1p25m1p5@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p25m1p5@J\endcsname{42.9}
\expandafter\def\csname v@rIIE@b1p25m1p5@CLBoth\endcsname{43.5}
\expandafter\def\csname v@rIIE@b1p25m1p5@CLLPF\endcsname{42.9}
\expandafter\def\csname v@rIIE@b1p25m1p5@GEODOB\endcsname{57.0}
\expandafter\def\csname v@rIIE@b1p25m1p5@INDI\endcsname{71.9}
\expandafter\def\csname v@rIIE@b1p25m1p5@CLatt\endcsname{44.4}
\expandafter\def\csname v@rIIE@b1p25m1p5@CLInner\endcsname{43.6}
\expandafter\def\csname v@rIIE@b1p25m2@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p25m2@J\endcsname{35.0}
\expandafter\def\csname v@rIIE@b1p25m2@CLBoth\endcsname{35.8}
\expandafter\def\csname v@rIIE@b1p25m2@CLLPF\endcsname{35.0}
\expandafter\def\csname v@rIIE@b1p25m2@GEODOB\endcsname{57.0}
\expandafter\def\csname v@rIIE@b1p25m2@INDI\endcsname{71.9}
\expandafter\def\csname v@rIIE@b1p25m2@CLatt\endcsname{39.9}
\expandafter\def\csname v@rIIE@b1p25m2@CLInner\endcsname{35.9}
\expandafter\def\csname v@rIIE@b1p25minf@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p25minf@J\endcsname{35.0}
\expandafter\def\csname v@rIIE@b1p25minf@CLBoth\endcsname{35.8}
\expandafter\def\csname v@rIIE@b1p25minf@CLLPF\endcsname{35.0}
\expandafter\def\csname v@rIIE@b1p25minf@GEODOB\endcsname{57.0}
\expandafter\def\csname v@rIIE@b1p25minf@INDI\endcsname{71.9}
\expandafter\def\csname v@rIIE@b1p25minf@CLatt\endcsname{39.9}
\expandafter\def\csname v@rIIE@b1p25minf@CLInner\endcsname{35.9}
\expandafter\def\csname v@rIIE@b1p35m1@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b1p35m1@J\endcsname{58.6}
\expandafter\def\csname v@rIIE@b1p35m1@CLLPF\endcsname{73.2}
\expandafter\def\csname v@rIIE@b1p35m1@GEODOB\endcsname{58.6}
\expandafter\def\csname v@rIIE@b1p35m1@INDI\endcsname{78.7}
\expandafter\def\csname v@rIIE@b1p35m1p2@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p35m1p2@J\endcsname{48.5}
\expandafter\def\csname v@rIIE@b1p35m1p2@CLBoth\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1p35m1p2@CLLPF\endcsname{48.5}
\expandafter\def\csname v@rIIE@b1p35m1p2@GEODOB\endcsname{58.6}
\expandafter\def\csname v@rIIE@b1p35m1p2@INDI\endcsname{65.9}
\expandafter\def\csname v@rIIE@b1p35m1p2@CLatt\endcsname{65.0}
\expandafter\def\csname v@rIIE@b1p35m1p2@CLInner\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1p35m1p5@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p35m1p5@J\endcsname{42.9}
\expandafter\def\csname v@rIIE@b1p35m1p5@CLBoth\endcsname{43.5}
\expandafter\def\csname v@rIIE@b1p35m1p5@CLLPF\endcsname{42.9}
\expandafter\def\csname v@rIIE@b1p35m1p5@GEODOB\endcsname{51.4}
\expandafter\def\csname v@rIIE@b1p35m1p5@INDI\endcsname{65.9}
\expandafter\def\csname v@rIIE@b1p35m1p5@CLatt\endcsname{44.4}
\expandafter\def\csname v@rIIE@b1p35m1p5@CLInner\endcsname{43.6}
\expandafter\def\csname v@rIIE@b1p35m2@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p35m2@J\endcsname{35.0}
\expandafter\def\csname v@rIIE@b1p35m2@CLBoth\endcsname{35.8}
\expandafter\def\csname v@rIIE@b1p35m2@CLLPF\endcsname{35.0}
\expandafter\def\csname v@rIIE@b1p35m2@GEODOB\endcsname{51.4}
\expandafter\def\csname v@rIIE@b1p35m2@INDI\endcsname{65.9}
\expandafter\def\csname v@rIIE@b1p35m2@CLatt\endcsname{37.3}
\expandafter\def\csname v@rIIE@b1p35m2@CLInner\endcsname{35.9}
\expandafter\def\csname v@rIIE@b1p35minf@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p35minf@J\endcsname{34.6}
\expandafter\def\csname v@rIIE@b1p35minf@CLBoth\endcsname{35.8}
\expandafter\def\csname v@rIIE@b1p35minf@CLLPF\endcsname{34.6}
\expandafter\def\csname v@rIIE@b1p35minf@GEODOB\endcsname{51.4}
\expandafter\def\csname v@rIIE@b1p35minf@INDI\endcsname{65.9}
\expandafter\def\csname v@rIIE@b1p35minf@CLatt\endcsname{37.3}
\expandafter\def\csname v@rIIE@b1p35minf@CLInner\endcsname{35.9}
\expandafter\def\csname v@rIIE@b1p5m1@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b1p5m1@J\endcsname{58.6}
\expandafter\def\csname v@rIIE@b1p5m1@CLLPF\endcsname{73.2}
\expandafter\def\csname v@rIIE@b1p5m1@GEODOB\endcsname{58.6}
\expandafter\def\csname v@rIIE@b1p5m1@INDI\endcsname{78.7}
\expandafter\def\csname v@rIIE@b1p5m1p2@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b1p5m1p2@J\endcsname{45.2}
\expandafter\def\csname v@rIIE@b1p5m1p2@CLBoth\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1p5m1p2@CLLPF\endcsname{48.5}
\expandafter\def\csname v@rIIE@b1p5m1p2@GEODOB\endcsname{45.2}
\expandafter\def\csname v@rIIE@b1p5m1p2@INDI\endcsname{59.1}
\expandafter\def\csname v@rIIE@b1p5m1p2@CLatt\endcsname{65.0}
\expandafter\def\csname v@rIIE@b1p5m1p2@CLInner\endcsname{60.0}
\expandafter\def\csname v@rIIE@b1p5m1p5@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b1p5m1p5@J\endcsname{38.8}
\expandafter\def\csname v@rIIE@b1p5m1p5@CLBoth\endcsname{43.5}
\expandafter\def\csname v@rIIE@b1p5m1p5@CLLPF\endcsname{42.9}
\expandafter\def\csname v@rIIE@b1p5m1p5@GEODOB\endcsname{38.8}
\expandafter\def\csname v@rIIE@b1p5m1p5@INDI\endcsname{59.1}
\expandafter\def\csname v@rIIE@b1p5m1p5@CLatt\endcsname{44.4}
\expandafter\def\csname v@rIIE@b1p5m1p5@CLInner\endcsname{43.6}
\expandafter\def\csname v@rIIE@b1p5m2@win\endcsname{CL-LPF}
\expandafter\def\csname v@rIIE@b1p5m2@J\endcsname{35.0}
\expandafter\def\csname v@rIIE@b1p5m2@CLBoth\endcsname{35.8}
\expandafter\def\csname v@rIIE@b1p5m2@CLLPF\endcsname{35.0}
\expandafter\def\csname v@rIIE@b1p5m2@GEODOB\endcsname{38.8}
\expandafter\def\csname v@rIIE@b1p5m2@INDI\endcsname{59.1}
\expandafter\def\csname v@rIIE@b1p5m2@CLatt\endcsname{37.3}
\expandafter\def\csname v@rIIE@b1p5m2@CLInner\endcsname{35.9}
\expandafter\def\csname v@rIIE@b1p5minf@win\endcsname{CL-att}
\expandafter\def\csname v@rIIE@b1p5minf@J\endcsname{34.2}
\expandafter\def\csname v@rIIE@b1p5minf@CLBoth\endcsname{35.8}
\expandafter\def\csname v@rIIE@b1p5minf@CLLPF\endcsname{34.3}
\expandafter\def\csname v@rIIE@b1p5minf@GEODOB\endcsname{38.8}
\expandafter\def\csname v@rIIE@b1p5minf@INDI\endcsname{59.1}
\expandafter\def\csname v@rIIE@b1p5minf@CLatt\endcsname{34.2}
\expandafter\def\csname v@rIIE@b1p5minf@CLInner\endcsname{35.9}
\expandafter\def\csname v@rIIE@b2m1@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b2m1@J\endcsname{58.6}
\expandafter\def\csname v@rIIE@b2m1@CLLPF\endcsname{73.2}
\expandafter\def\csname v@rIIE@b2m1@GEODOB\endcsname{58.6}
\expandafter\def\csname v@rIIE@b2m1@INDI\endcsname{78.7}
\expandafter\def\csname v@rIIE@b2m1p2@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b2m1p2@J\endcsname{39.9}
\expandafter\def\csname v@rIIE@b2m1p2@CLBoth\endcsname{60.0}
\expandafter\def\csname v@rIIE@b2m1p2@CLLPF\endcsname{48.5}
\expandafter\def\csname v@rIIE@b2m1p2@GEODOB\endcsname{39.9}
\expandafter\def\csname v@rIIE@b2m1p2@INDI\endcsname{51.4}
\expandafter\def\csname v@rIIE@b2m1p2@CLatt\endcsname{65.0}
\expandafter\def\csname v@rIIE@b2m1p2@CLInner\endcsname{60.0}
\expandafter\def\csname v@rIIE@b2m1p5@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b2m1p5@J\endcsname{31.3}
\expandafter\def\csname v@rIIE@b2m1p5@CLBoth\endcsname{43.5}
\expandafter\def\csname v@rIIE@b2m1p5@CLLPF\endcsname{42.9}
\expandafter\def\csname v@rIIE@b2m1p5@GEODOB\endcsname{31.3}
\expandafter\def\csname v@rIIE@b2m1p5@INDI\endcsname{51.4}
\expandafter\def\csname v@rIIE@b2m1p5@CLatt\endcsname{44.4}
\expandafter\def\csname v@rIIE@b2m1p5@CLInner\endcsname{43.6}
\expandafter\def\csname v@rIIE@b2m2@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b2m2@J\endcsname{31.3}
\expandafter\def\csname v@rIIE@b2m2@CLBoth\endcsname{35.8}
\expandafter\def\csname v@rIIE@b2m2@CLLPF\endcsname{35.0}
\expandafter\def\csname v@rIIE@b2m2@GEODOB\endcsname{31.3}
\expandafter\def\csname v@rIIE@b2m2@INDI\endcsname{51.4}
\expandafter\def\csname v@rIIE@b2m2@CLatt\endcsname{37.3}
\expandafter\def\csname v@rIIE@b2m2@CLInner\endcsname{35.9}
\expandafter\def\csname v@rIIE@b2minf@win\endcsname{GEO-DOB}
\expandafter\def\csname v@rIIE@b2minf@J\endcsname{31.3}
\expandafter\def\csname v@rIIE@b2minf@CLBoth\endcsname{35.8}
\expandafter\def\csname v@rIIE@b2minf@CLLPF\endcsname{34.3}
\expandafter\def\csname v@rIIE@b2minf@GEODOB\endcsname{31.3}
\expandafter\def\csname v@rIIE@b2minf@INDI\endcsname{51.4}
\expandafter\def\csname v@rIIE@b2minf@CLatt\endcsname{34.2}
\expandafter\def\csname v@rIIE@b2minf@CLInner\endcsname{35.9}
\expandafter\def\csname v@rIIE@psd@fcmin\endcsname{95}
\expandafter\def\csname v@rIIE@psd@fcmax\endcsname{98}
\expandafter\def\csname v@rIIE@psd@fiftymin\endcsname{86}
\expandafter\def\csname v@rIIE@psd@fiftymax\endcsname{90}
\expandafter\def\csname v@rIIE@act@spearmin\endcsname{0.90}
\expandafter\def\csname v@rIIE@act@bothLPF\endcsname{1.11}
\expandafter\def\csname v@rIIE@act@bothDW\endcsname{1.03}
\expandafter\def\csname v@rIIIE@indi@J\endcsname{101.6}
\expandafter\def\csname v@rIIIE@indi@DW\endcsname{11.79}
\expandafter\def\csname v@rIIIE@ka1@J\endcsname{59.1}
\expandafter\def\csname v@rIIIE@ka1@DW\endcsname{17.19}
\expandafter\def\csname v@rIIIE@tau01@J\endcsname{78.7}
\expandafter\def\csname v@rIIIE@tau01@DW\endcsname{16.24}
\expandafter\def\csname v@rIIIE@kp4@J\endcsname{415.2}
\expandafter\def\csname v@rIIIE@kp4@DW\endcsname{15.04}
\expandafter\def\csname v@rIIIE@INDI@ncand\endcsname{10}
\expandafter\def\csname v@rIIIE@INDI@npass\endcsname{8}
\expandafter\def\csname v@rIIIE@INDI@gJ\endcsname{101.6}
\expandafter\def\csname v@rIIIE@INDI@gbound\endcsname{11.95}
\expandafter\def\csname v@rIIIE@INDI@gcfg\endcsname{[2 0.5 0.2]}
\expandafter\def\csname v@rIIIE@INDI@sJ\endcsname{101.6}
\expandafter\def\csname v@rIIIE@INDI@sbound\endcsname{11.95}
\expandafter\def\csname v@rIIIE@INDI@spass\endcsname{passes}
\expandafter\def\csname v@rIIIE@L1@ncand\endcsname{10}
\expandafter\def\csname v@rIIIE@L1@npass\endcsname{0}
\expandafter\def\csname v@rIIIE@L1@gJ\endcsname{--}
\expandafter\def\csname v@rIIIE@L1@gbound\endcsname{--}
\expandafter\def\csname v@rIIIE@L1@gcfg\endcsname{none}
\expandafter\def\csname v@rIIIE@L1@minbound\endcsname{13.08}
\expandafter\def\csname v@rIIIE@L1@sJ\endcsname{100.8}
\expandafter\def\csname v@rIIIE@L1@sbound\endcsname{13.12}
\expandafter\def\csname v@rIIIE@L1@spass\endcsname{fails}
\expandafter\def\csname v@rIIIE@GEODOB@ncand\endcsname{10}
\expandafter\def\csname v@rIIIE@GEODOB@npass\endcsname{9}
\expandafter\def\csname v@rIIIE@GEODOB@gJ\endcsname{69.6}
\expandafter\def\csname v@rIIIE@GEODOB@gbound\endcsname{11.37}
\expandafter\def\csname v@rIIIE@GEODOB@gcfg\endcsname{[1 0.5 0.2 1 0.4]}
\expandafter\def\csname v@rIIIE@GEODOB@sJ\endcsname{57.0}
\expandafter\def\csname v@rIIIE@GEODOB@sbound\endcsname{13.15}
\expandafter\def\csname v@rIIIE@GEODOB@spass\endcsname{fails}
\expandafter\def\csname v@rIIIE@INDIRPM@ncand\endcsname{10}
\expandafter\def\csname v@rIIIE@INDIRPM@npass\endcsname{8}
\expandafter\def\csname v@rIIIE@INDIRPM@gJ\endcsname{102.5}
\expandafter\def\csname v@rIIIE@INDIRPM@gbound\endcsname{11.95}
\expandafter\def\csname v@rIIIE@INDIRPM@gcfg\endcsname{[2 0.5 0.2]}
\expandafter\def\csname v@rIIIE@INDIRPM@sJ\endcsname{102.5}
\expandafter\def\csname v@rIIIE@INDIRPM@sbound\endcsname{11.95}
\expandafter\def\csname v@rIIIE@INDIRPM@spass\endcsname{passes}
\expandafter\def\csname v@rIIIE@diag@sat\endcsname{0.0}
\expandafter\def\csname v@rIIIE@diag@tiltmax\endcsname{57.0}
\expandafter\def\csname v@rIIIE@diag@tiltlim\endcsname{35}
\expandafter\def\csname v@rIIIE@diag@atlim\endcsname{58.5}
\expandafter\def\csname v@rIIIE@diag@emax\endcsname{1.19}
\expandafter\def\csname v@rIIIE@diag@efirst\endcsname{968}
\expandafter\def\csname v@rIIIE@diag@elast\endcsname{648}
\expandafter\def\csname v@rIIIE@diagB@tiltmax\endcsname{30.7}
\expandafter\def\csname v@rIIIE@diagB@atlim\endcsname{0.0}
\expandafter\def\csname v@rIIIE@INDI@pass\endcsname{100}
\expandafter\def\csname v@rIIIE@INDI@paired\endcsname{100}
\expandafter\def\csname v@rIIIE@GEODOB@pass\endcsname{100}
\expandafter\def\csname v@rIIIE@GEODOB@paired\endcsname{100}
\expandafter\def\csname v@rIIIE@INDIRPM@pass\endcsname{100}
\expandafter\def\csname v@rIIIE@INDIRPM@paired\endcsname{100}
\expandafter\def\csname v@rIIIE@GEODOB@design\endcsname{69.6}
\expandafter\def\csname v@rIIIE@GEODOB@eval6\endcsname{120.5}
\expandafter\def\csname v@rIIIE@GEODOB@Sten\endcsname{202.0}
\expandafter\def\csname v@rIIIE@GEODOB@Sone\endcsname{16.2}
\expandafter\def\csname v@rIIIE@INDI@design\endcsname{101.6}
\expandafter\def\csname v@rIIIE@INDI@eval6\endcsname{235.2}
\expandafter\def\csname v@rIIIE@INDI@Sten\endcsname{845.2}
\expandafter\def\csname v@rIIIE@INDIRPM@design\endcsname{102.5}
\expandafter\def\csname v@rIIIE@INDIRPM@eval6\endcsname{238.0}
\expandafter\def\csname v@rIIIE@INDIRPM@Sten\endcsname{861.2}
\expandafter\def\csname v@rIIIE@best@eval6\endcsname{120.5}
\expandafter\def\csname v@rIIIE@best@name\endcsname{GEO-DOB}
\expandafter\def\csname v@rIVE@S2CLBothG@mean\endcsname{31.6}
\expandafter\def\csname v@rIVE@S2CLBothG@median\endcsname{31.1}
\expandafter\def\csname v@rIVE@S2CLBothG@p95\endcsname{36.2}
\expandafter\def\csname v@rIVE@S2CLBothG@meandw\endcsname{18.81}
\expandafter\def\csname v@rIVE@S2CLBothG@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S2CLBothG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S2CLInnerG@mean\endcsname{38.1}
\expandafter\def\csname v@rIVE@S2CLInnerG@median\endcsname{37.5}
\expandafter\def\csname v@rIVE@S2CLInnerG@p95\endcsname{43.8}
\expandafter\def\csname v@rIVE@S2CLInnerG@meandw\endcsname{17.84}
\expandafter\def\csname v@rIVE@S2CLInnerG@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S2CLInnerG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S2CLLPFG@mean\endcsname{31.3}
\expandafter\def\csname v@rIVE@S2CLLPFG@median\endcsname{30.9}
\expandafter\def\csname v@rIVE@S2CLLPFG@p95\endcsname{35.6}
\expandafter\def\csname v@rIVE@S2CLLPFG@meandw\endcsname{18.71}
\expandafter\def\csname v@rIVE@S2CLLPFG@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S2CLLPFG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S2CLattG@mean\endcsname{50.6}
\expandafter\def\csname v@rIVE@S2CLattG@median\endcsname{49.2}
\expandafter\def\csname v@rIVE@S2CLattG@p95\endcsname{60.7}
\expandafter\def\csname v@rIVE@S2CLattG@meandw\endcsname{16.06}
\expandafter\def\csname v@rIVE@S2CLattG@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S2CLattG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S2GEODOBG@mean\endcsname{184.2}
\expandafter\def\csname v@rIVE@S2GEODOBG@median\endcsname{76.8}
\expandafter\def\csname v@rIVE@S2GEODOBG@p95\endcsname{739.8}
\expandafter\def\csname v@rIVE@S2GEODOBG@meandw\endcsname{11.81}
\expandafter\def\csname v@rIVE@S2GEODOBG@inc\endcsname{1}
\expandafter\def\csname v@rIVE@S2GEODOBG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S2INDIG@mean\endcsname{118.2}
\expandafter\def\csname v@rIVE@S2INDIG@median\endcsname{94.6}
\expandafter\def\csname v@rIVE@S2INDIG@p95\endcsname{326.8}
\expandafter\def\csname v@rIVE@S2INDIG@meandw\endcsname{12.37}
\expandafter\def\csname v@rIVE@S2INDIG@inc\endcsname{2}
\expandafter\def\csname v@rIVE@S2INDIG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S2INDIRPMG@mean\endcsname{219.9}
\expandafter\def\csname v@rIVE@S2INDIRPMG@median\endcsname{101.7}
\expandafter\def\csname v@rIVE@S2INDIRPMG@p95\endcsname{1091.4}
\expandafter\def\csname v@rIVE@S2INDIRPMG@meandw\endcsname{12.38}
\expandafter\def\csname v@rIVE@S2INDIRPMG@inc\endcsname{2}
\expandafter\def\csname v@rIVE@S2INDIRPMG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S2LQR@mean\endcsname{348.3}
\expandafter\def\csname v@rIVE@S2LQR@median\endcsname{336.8}
\expandafter\def\csname v@rIVE@S2LQR@p95\endcsname{560.7}
\expandafter\def\csname v@rIVE@S2LQR@meandw\endcsname{12.25}
\expandafter\def\csname v@rIVE@S2LQR@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S2LQR@over\endcsname{0}
\expandafter\def\csname v@rIVE@S2MRAC@mean\endcsname{89.1}
\expandafter\def\csname v@rIVE@S2MRAC@median\endcsname{82.5}
\expandafter\def\csname v@rIVE@S2MRAC@p95\endcsname{134.0}
\expandafter\def\csname v@rIVE@S2MRAC@meandw\endcsname{20.57}
\expandafter\def\csname v@rIVE@S2MRAC@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S2MRAC@over\endcsname{0}
\expandafter\def\csname v@rIVE@S2NNMRAC@mean\endcsname{66.8}
\expandafter\def\csname v@rIVE@S2NNMRAC@median\endcsname{66.6}
\expandafter\def\csname v@rIVE@S2NNMRAC@p95\endcsname{91.1}
\expandafter\def\csname v@rIVE@S2NNMRAC@meandw\endcsname{13.69}
\expandafter\def\csname v@rIVE@S2NNMRAC@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S2NNMRAC@over\endcsname{0}
\expandafter\def\csname v@rIVE@S4CLBothG@mean\endcsname{48.0}
\expandafter\def\csname v@rIVE@S4CLBothG@median\endcsname{46.6}
\expandafter\def\csname v@rIVE@S4CLBothG@p95\endcsname{64.3}
\expandafter\def\csname v@rIVE@S4CLBothG@meandw\endcsname{23.22}
\expandafter\def\csname v@rIVE@S4CLBothG@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S4CLBothG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S4CLInnerG@mean\endcsname{49.9}
\expandafter\def\csname v@rIVE@S4CLInnerG@median\endcsname{47.7}
\expandafter\def\csname v@rIVE@S4CLInnerG@p95\endcsname{64.7}
\expandafter\def\csname v@rIVE@S4CLInnerG@meandw\endcsname{21.98}
\expandafter\def\csname v@rIVE@S4CLInnerG@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S4CLInnerG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S4CLLPFG@mean\endcsname{48.0}
\expandafter\def\csname v@rIVE@S4CLLPFG@median\endcsname{46.0}
\expandafter\def\csname v@rIVE@S4CLLPFG@p95\endcsname{65.8}
\expandafter\def\csname v@rIVE@S4CLLPFG@meandw\endcsname{23.47}
\expandafter\def\csname v@rIVE@S4CLLPFG@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S4CLLPFG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S4CLattG@mean\endcsname{59.0}
\expandafter\def\csname v@rIVE@S4CLattG@median\endcsname{57.4}
\expandafter\def\csname v@rIVE@S4CLattG@p95\endcsname{76.4}
\expandafter\def\csname v@rIVE@S4CLattG@meandw\endcsname{19.48}
\expandafter\def\csname v@rIVE@S4CLattG@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S4CLattG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S4GEODOBG@mean\endcsname{197.9}
\expandafter\def\csname v@rIVE@S4GEODOBG@median\endcsname{113.5}
\expandafter\def\csname v@rIVE@S4GEODOBG@p95\endcsname{842.1}
\expandafter\def\csname v@rIVE@S4GEODOBG@meandw\endcsname{12.09}
\expandafter\def\csname v@rIVE@S4GEODOBG@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S4GEODOBG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S4INDIG@mean\endcsname{199.5}
\expandafter\def\csname v@rIVE@S4INDIG@median\endcsname{122.0}
\expandafter\def\csname v@rIVE@S4INDIG@p95\endcsname{702.8}
\expandafter\def\csname v@rIVE@S4INDIG@meandw\endcsname{11.97}
\expandafter\def\csname v@rIVE@S4INDIG@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S4INDIG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S4INDIRPMG@mean\endcsname{330.7}
\expandafter\def\csname v@rIVE@S4INDIRPMG@median\endcsname{127.9}
\expandafter\def\csname v@rIVE@S4INDIRPMG@p95\endcsname{1442.2}
\expandafter\def\csname v@rIVE@S4INDIRPMG@meandw\endcsname{11.93}
\expandafter\def\csname v@rIVE@S4INDIRPMG@inc\endcsname{1}
\expandafter\def\csname v@rIVE@S4INDIRPMG@over\endcsname{0}
\expandafter\def\csname v@rIVE@S4LQR@mean\endcsname{392.9}
\expandafter\def\csname v@rIVE@S4LQR@median\endcsname{373.4}
\expandafter\def\csname v@rIVE@S4LQR@p95\endcsname{529.5}
\expandafter\def\csname v@rIVE@S4LQR@meandw\endcsname{12.33}
\expandafter\def\csname v@rIVE@S4LQR@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S4LQR@over\endcsname{0}
\expandafter\def\csname v@rIVE@S4MRAC@mean\endcsname{107.8}
\expandafter\def\csname v@rIVE@S4MRAC@median\endcsname{102.5}
\expandafter\def\csname v@rIVE@S4MRAC@p95\endcsname{148.7}
\expandafter\def\csname v@rIVE@S4MRAC@meandw\endcsname{24.42}
\expandafter\def\csname v@rIVE@S4MRAC@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S4MRAC@over\endcsname{0}
\expandafter\def\csname v@rIVE@S4NNMRAC@mean\endcsname{85.5}
\expandafter\def\csname v@rIVE@S4NNMRAC@median\endcsname{84.2}
\expandafter\def\csname v@rIVE@S4NNMRAC@p95\endcsname{108.5}
\expandafter\def\csname v@rIVE@S4NNMRAC@meandw\endcsname{14.59}
\expandafter\def\csname v@rIVE@S4NNMRAC@inc\endcsname{0}
\expandafter\def\csname v@rIVE@S4NNMRAC@over\endcsname{0}
\expandafter\def\csname v@rIVE@S2CLInnerG@wins\endcsname{50}
\expandafter\def\csname v@rIVE@S2CLInnerG@n\endcsname{50}
\expandafter\def\csname v@rIVE@S2CLInnerG@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S2CLInnerG@mdiff\endcsname{6.52}
\expandafter\def\csname v@rIVE@S2CLLPFG@wins\endcsname{0}
\expandafter\def\csname v@rIVE@S2CLLPFG@n\endcsname{50}
\expandafter\def\csname v@rIVE@S2CLLPFG@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S2CLLPFG@mdiff\endcsname{0.30}
\expandafter\def\csname v@rIVE@S2CLattG@wins\endcsname{50}
\expandafter\def\csname v@rIVE@S2CLattG@n\endcsname{50}
\expandafter\def\csname v@rIVE@S2CLattG@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S2CLattG@mdiff\endcsname{19.03}
\expandafter\def\csname v@rIVE@S2GEODOBG@wins\endcsname{49}
\expandafter\def\csname v@rIVE@S2GEODOBG@n\endcsname{49}
\expandafter\def\csname v@rIVE@S2GEODOBG@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S2GEODOBG@mdiff\endcsname{152.65}
\expandafter\def\csname v@rIVE@S2INDIG@wins\endcsname{48}
\expandafter\def\csname v@rIVE@S2INDIG@n\endcsname{48}
\expandafter\def\csname v@rIVE@S2INDIG@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S2INDIG@mdiff\endcsname{86.68}
\expandafter\def\csname v@rIVE@S2INDIRPMG@wins\endcsname{48}
\expandafter\def\csname v@rIVE@S2INDIRPMG@n\endcsname{48}
\expandafter\def\csname v@rIVE@S2INDIRPMG@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S2INDIRPMG@mdiff\endcsname{188.37}
\expandafter\def\csname v@rIVE@S2LQR@wins\endcsname{50}
\expandafter\def\csname v@rIVE@S2LQR@n\endcsname{50}
\expandafter\def\csname v@rIVE@S2LQR@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S2LQR@mdiff\endcsname{316.76}
\expandafter\def\csname v@rIVE@S2MRAC@wins\endcsname{50}
\expandafter\def\csname v@rIVE@S2MRAC@n\endcsname{50}
\expandafter\def\csname v@rIVE@S2MRAC@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S2MRAC@mdiff\endcsname{57.56}
\expandafter\def\csname v@rIVE@S2NNMRAC@wins\endcsname{50}
\expandafter\def\csname v@rIVE@S2NNMRAC@n\endcsname{50}
\expandafter\def\csname v@rIVE@S2NNMRAC@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S2NNMRAC@mdiff\endcsname{35.24}
\expandafter\def\csname v@rIVE@S4CLInnerG@wins\endcsname{41}
\expandafter\def\csname v@rIVE@S4CLInnerG@n\endcsname{50}
\expandafter\def\csname v@rIVE@S4CLInnerG@pholm\endcsname{\ensuremath{5.6\times10^{-6}}}
\expandafter\def\csname v@rIVE@S4CLInnerG@mdiff\endcsname{1.82}
\expandafter\def\csname v@rIVE@S4CLLPFG@wins\endcsname{7}
\expandafter\def\csname v@rIVE@S4CLLPFG@n\endcsname{50}
\expandafter\def\csname v@rIVE@S4CLLPFG@pholm\endcsname{\ensuremath{4.2\times10^{-7}}}
\expandafter\def\csname v@rIVE@S4CLLPFG@mdiff\endcsname{0.04}
\expandafter\def\csname v@rIVE@S4CLattG@wins\endcsname{49}
\expandafter\def\csname v@rIVE@S4CLattG@n\endcsname{50}
\expandafter\def\csname v@rIVE@S4CLattG@pholm\endcsname{\ensuremath{2.7\times10^{-13}}}
\expandafter\def\csname v@rIVE@S4CLattG@mdiff\endcsname{10.96}
\expandafter\def\csname v@rIVE@S4GEODOBG@wins\endcsname{50}
\expandafter\def\csname v@rIVE@S4GEODOBG@n\endcsname{50}
\expandafter\def\csname v@rIVE@S4GEODOBG@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S4GEODOBG@mdiff\endcsname{149.81}
\expandafter\def\csname v@rIVE@S4INDIG@wins\endcsname{50}
\expandafter\def\csname v@rIVE@S4INDIG@n\endcsname{50}
\expandafter\def\csname v@rIVE@S4INDIG@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S4INDIG@mdiff\endcsname{151.44}
\expandafter\def\csname v@rIVE@S4INDIRPMG@wins\endcsname{49}
\expandafter\def\csname v@rIVE@S4INDIRPMG@n\endcsname{49}
\expandafter\def\csname v@rIVE@S4INDIRPMG@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S4INDIRPMG@mdiff\endcsname{282.77}
\expandafter\def\csname v@rIVE@S4LQR@wins\endcsname{50}
\expandafter\def\csname v@rIVE@S4LQR@n\endcsname{50}
\expandafter\def\csname v@rIVE@S4LQR@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S4LQR@mdiff\endcsname{344.84}
\expandafter\def\csname v@rIVE@S4MRAC@wins\endcsname{50}
\expandafter\def\csname v@rIVE@S4MRAC@n\endcsname{50}
\expandafter\def\csname v@rIVE@S4MRAC@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S4MRAC@mdiff\endcsname{59.77}
\expandafter\def\csname v@rIVE@S4NNMRAC@wins\endcsname{50}
\expandafter\def\csname v@rIVE@S4NNMRAC@n\endcsname{50}
\expandafter\def\csname v@rIVE@S4NNMRAC@pholm\endcsname{\ensuremath{1.6\times10^{-14}}}
\expandafter\def\csname v@rIVE@S4NNMRAC@mdiff\endcsname{37.46}
\expandafter\def\csname v@rIVE@all@pmax\endcsname{\ensuremath{6\times10^{-6}}}
\expandafter\def\csname v@rIVE@S2CLInnerG@med\endcsname{6.91}
\expandafter\def\csname v@rIVE@S2CLInnerG@cilo\endcsname{5.77}
\expandafter\def\csname v@rIVE@S2CLInnerG@cihi\endcsname{7.48}
\expandafter\def\csname v@rIVE@S2CLLPFG@med\endcsname{0.25}
\expandafter\def\csname v@rIVE@S2CLLPFG@cilo\endcsname{0.20}
\expandafter\def\csname v@rIVE@S2CLLPFG@cihi\endcsname{0.33}
\expandafter\def\csname v@rIVE@S2CLattG@med\endcsname{18.45}
\expandafter\def\csname v@rIVE@S2CLattG@cilo\endcsname{16.70}
\expandafter\def\csname v@rIVE@S2CLattG@cihi\endcsname{20.37}
\expandafter\def\csname v@rIVE@S2GEODOBG@med\endcsname{44.29}
\expandafter\def\csname v@rIVE@S2GEODOBG@cilo\endcsname{38.43}
\expandafter\def\csname v@rIVE@S2GEODOBG@cihi\endcsname{57.86}
\expandafter\def\csname v@rIVE@S2INDIG@med\endcsname{62.90}
\expandafter\def\csname v@rIVE@S2INDIG@cilo\endcsname{57.55}
\expandafter\def\csname v@rIVE@S2INDIG@cihi\endcsname{67.01}
\expandafter\def\csname v@rIVE@S2INDIRPMG@med\endcsname{67.73}
\expandafter\def\csname v@rIVE@S2INDIRPMG@cilo\endcsname{60.90}
\expandafter\def\csname v@rIVE@S2INDIRPMG@cihi\endcsname{77.91}
\expandafter\def\csname v@rIVE@S2LQR@med\endcsname{306.39}
\expandafter\def\csname v@rIVE@S2LQR@cilo\endcsname{259.86}
\expandafter\def\csname v@rIVE@S2LQR@cihi\endcsname{357.81}
\expandafter\def\csname v@rIVE@S2MRAC@med\endcsname{52.03}
\expandafter\def\csname v@rIVE@S2MRAC@cilo\endcsname{46.96}
\expandafter\def\csname v@rIVE@S2MRAC@cihi\endcsname{57.05}
\expandafter\def\csname v@rIVE@S2NNMRAC@med\endcsname{33.22}
\expandafter\def\csname v@rIVE@S2NNMRAC@cilo\endcsname{31.93}
\expandafter\def\csname v@rIVE@S2NNMRAC@cihi\endcsname{36.83}
\expandafter\def\csname v@rIVE@S4CLInnerG@med\endcsname{2.06}
\expandafter\def\csname v@rIVE@S4CLInnerG@cilo\endcsname{1.29}
\expandafter\def\csname v@rIVE@S4CLInnerG@cihi\endcsname{2.78}
\expandafter\def\csname v@rIVE@S4CLLPFG@med\endcsname{0.66}
\expandafter\def\csname v@rIVE@S4CLLPFG@cilo\endcsname{0.54}
\expandafter\def\csname v@rIVE@S4CLLPFG@cihi\endcsname{0.81}
\expandafter\def\csname v@rIVE@S4CLattG@med\endcsname{11.08}
\expandafter\def\csname v@rIVE@S4CLattG@cilo\endcsname{9.64}
\expandafter\def\csname v@rIVE@S4CLattG@cihi\endcsname{12.00}
\expandafter\def\csname v@rIVE@S4GEODOBG@med\endcsname{57.43}
\expandafter\def\csname v@rIVE@S4GEODOBG@cilo\endcsname{47.69}
\expandafter\def\csname v@rIVE@S4GEODOBG@cihi\endcsname{84.74}
\expandafter\def\csname v@rIVE@S4INDIG@med\endcsname{71.87}
\expandafter\def\csname v@rIVE@S4INDIG@cilo\endcsname{62.73}
\expandafter\def\csname v@rIVE@S4INDIG@cihi\endcsname{96.58}
\expandafter\def\csname v@rIVE@S4INDIRPMG@med\endcsname{81.16}
\expandafter\def\csname v@rIVE@S4INDIRPMG@cilo\endcsname{69.20}
\expandafter\def\csname v@rIVE@S4INDIRPMG@cihi\endcsname{113.91}
\expandafter\def\csname v@rIVE@S4LQR@med\endcsname{326.56}
\expandafter\def\csname v@rIVE@S4LQR@cilo\endcsname{299.49}
\expandafter\def\csname v@rIVE@S4LQR@cihi\endcsname{364.84}
\expandafter\def\csname v@rIVE@S4MRAC@med\endcsname{55.10}
\expandafter\def\csname v@rIVE@S4MRAC@cilo\endcsname{48.98}
\expandafter\def\csname v@rIVE@S4MRAC@cihi\endcsname{71.63}
\expandafter\def\csname v@rIVE@S4NNMRAC@med\endcsname{36.47}
\expandafter\def\csname v@rIVE@S4NNMRAC@cilo\endcsname{31.85}
\expandafter\def\csname v@rIVE@S4NNMRAC@cihi\endcsname{40.34}
\expandafter\def\csname v@rV@six@Jsym\endcsname{43.79}
\expandafter\def\csname v@rV@six@tauf\endcsname{150}
\expandafter\def\csname v@rV@six@go\endcsname{160}
\expandafter\def\csname v@rV@six@gap\endcsname{8.2}
\expandafter\def\csname v@rV@six50@J\endcsname{46.15}
\expandafter\def\csname v@rV@six50@DW\endcsname{12.93}
\expandafter\def\csname v@rV@six70@J\endcsname{45.52}
\expandafter\def\csname v@rV@six70@DW\endcsname{12.89}
\expandafter\def\csname v@rV@six100@J\endcsname{44.74}
\expandafter\def\csname v@rV@six100@DW\endcsname{12.93}
\expandafter\def\csname v@rV@six150@J\endcsname{43.79}
\expandafter\def\csname v@rV@six150@DW\endcsname{13.00}
\expandafter\def\csname v@rV@six200@J\endcsname{46.73}
\expandafter\def\csname v@rV@six200@DW\endcsname{12.57}
\expandafter\def\csname v@rV@act@lpfLPF\endcsname{1.11}
\expandafter\def\csname v@rV@act@lpfDW\endcsname{1.03}
\expandafter\def\csname v@rV@act@bothLPF\endcsname{1.11}
\expandafter\def\csname v@rV@act@inLPF\endcsname{1.06}
\expandafter\def\csname v@rV@act@geoLPF\endcsname{1.05}
\expandafter\def\csname v@rV@act@indiLPF\endcsname{0.97}
\expandafter\def\csname v@rV@CLLPFG@esmean\endcsname{45.6}
\expandafter\def\csname v@rV@CLLPFG@essd\endcsname{0.08}
\expandafter\def\csname v@rV@CLLPFG@esbest\endcsname{10}
\expandafter\def\csname v@rV@CLLPFG@esinc\endcsname{0}
\expandafter\def\csname v@rV@CLBothG@esmean\endcsname{46.4}
\expandafter\def\csname v@rV@CLBothG@essd\endcsname{0.08}
\expandafter\def\csname v@rV@CLBothG@esbest\endcsname{0}
\expandafter\def\csname v@rV@CLBothG@esinc\endcsname{0}
\expandafter\def\csname v@rV@CLInnerG@esmean\endcsname{51.9}
\expandafter\def\csname v@rV@CLInnerG@essd\endcsname{0.04}
\expandafter\def\csname v@rV@CLInnerG@esbest\endcsname{0}
\expandafter\def\csname v@rV@CLInnerG@esinc\endcsname{0}
\expandafter\def\csname v@rV@CLattG@esmean\endcsname{60.5}
\expandafter\def\csname v@rV@CLattG@essd\endcsname{0.06}
\expandafter\def\csname v@rV@CLattG@esbest\endcsname{0}
\expandafter\def\csname v@rV@CLattG@esinc\endcsname{0}
\expandafter\def\csname v@rV@MRAC@esmean\endcsname{83.9}
\expandafter\def\csname v@rV@MRAC@essd\endcsname{0.06}
\expandafter\def\csname v@rV@MRAC@esbest\endcsname{0}
\expandafter\def\csname v@rV@MRAC@esinc\endcsname{0}
\expandafter\def\csname v@rV@NNMRAC@esmean\endcsname{84.6}
\expandafter\def\csname v@rV@NNMRAC@essd\endcsname{0.06}
\expandafter\def\csname v@rV@NNMRAC@esbest\endcsname{0}
\expandafter\def\csname v@rV@NNMRAC@esinc\endcsname{0}
\expandafter\def\csname v@rV@GEODOBG@esmean\endcsname{122.1}
\expandafter\def\csname v@rV@GEODOBG@essd\endcsname{0.77}
\expandafter\def\csname v@rV@GEODOBG@esbest\endcsname{0}
\expandafter\def\csname v@rV@GEODOBG@esinc\endcsname{0}
\expandafter\def\csname v@rV@INDIG@esmean\endcsname{235.0}
\expandafter\def\csname v@rV@INDIG@essd\endcsname{0.55}
\expandafter\def\csname v@rV@INDIG@esbest\endcsname{0}
\expandafter\def\csname v@rV@INDIG@esinc\endcsname{0}
\expandafter\def\csname v@rV@INDIRPMG@esmean\endcsname{238.8}
\expandafter\def\csname v@rV@INDIRPMG@essd\endcsname{1.25}
\expandafter\def\csname v@rV@INDIRPMG@esbest\endcsname{0}
\expandafter\def\csname v@rV@INDIRPMG@esinc\endcsname{0}
\expandafter\def\csname v@rV@LQR@esmean\endcsname{482.9}
\expandafter\def\csname v@rV@LQR@essd\endcsname{0.05}
\expandafter\def\csname v@rV@LQR@esbest\endcsname{0}
\expandafter\def\csname v@rV@LQR@esinc\endcsname{0}
\expandafter\def\csname v@rV@sitl@lqrmed\endcsname{0.61}
\expandafter\def\csname v@rV@sitl@nto\endcsname{16}
\expandafter\def\csname v@rV@sitl@nruns\endcsname{20}
\expandafter\def\csname v@rV@sitl160@medratio\endcsname{1.09}
\expandafter\def\csname v@rV@sitl160@maxratio\endcsname{2.36}
\expandafter\def\csname v@rV@sitl160@med\endcsname{0.64}
\expandafter\def\csname v@rV@sitl160@npass\endcsname{2}
\expandafter\def\csname v@rV@sitl320@medratio\endcsname{1.07}
\expandafter\def\csname v@rV@sitl320@maxratio\endcsname{1.67}
\expandafter\def\csname v@rV@sitl320@med\endcsname{0.75}
\expandafter\def\csname v@rV@sitl320@npass\endcsname{2}
\expandafter\def\csname v@rV@sitl640@medratio\endcsname{1.04}
\expandafter\def\csname v@rV@sitl640@maxratio\endcsname{1.76}
\expandafter\def\csname v@rV@sitl640@med\endcsname{0.65}
\expandafter\def\csname v@rV@sitl640@npass\endcsname{3}
\makeatother

